Quantum Methods for Managing Ambiguity in Natural Language Processing

The Categorical Compositional Distributional (DisCoCat) framework models meaning in natural language using the mathematical framework of quantum theory, expressed as formal diagrams. DisCoCat diagrams can be associated with tensor networks and quantum circuits. DisCoCat diagrams have been connected to density matrices in various contexts in Quantum Natural Language Processing (QNLP). Previous use of density matrices in QNLP entails modelling ambiguous words as probability distributions over more basic words (the word \texttt{queen}, e.g., might mean the reigning queen or the chess piece). In this article, we investigate using probability distributions over processes to account for syntactic ambiguity in sentences. The meanings of these sentences are represented by density matrices. We show how to create probability distributions on quantum circuits that represent the meanings of sentences and explain how this approach generalises tasks from the literature. We conduct an experiment to validate the proposed theory.

==> Definitions/journalnames.tex <==
% Updated 4 September 2024
%% --------------------------------------------------------------------
%\DeclareOption{}{%
%	\gdef\@journal{}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalfull: Journal full name
%% - @journalshort: Short Name (ISO4)
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.3390/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @continuouspages: use \gdef\@continuouspages{yes} for journals that use pagination
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{acoustics}{%
	\gdef\@journal{acoustics}
	\gdef\@journalfull{Acoustics}
	\gdef\@journalshort{Acoustics}
	\gdef\@doiabbr{acoustics}
	\gdef\@ISSN{2624-599X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{actuators}{%
	\gdef\@journal{actuators}
	\gdef\@journalfull{Actuators}
	\gdef\@journalshort{Actuators}
	\gdef\@doiabbr{act}
	\gdef\@ISSN{2076-0825}
	\gdef\@societyowner{}
}
\DeclareOption{addictions}{%
	\gdef\@journal{addictions}
	\gdef\@journalfull{Addictions}
	\gdef\@journalshort{Addictions}
	\gdef\@doiabbr{addictions}
	\gdef\@ISSN{0006-0006}
	\gdef\@societyowner{}
}
\DeclareOption{adhesives}{%
	\gdef\@journal{adhesives}
	\gdef\@journalfull{Adhesives}
	\gdef\@journalshort{Adhesives}
	\gdef\@doiabbr{adhesives}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{admsci}{%
	\gdef\@journal{admsci}
	\gdef\@journalfull{Administrative Sciences}
	\gdef\@journalshort{Adm. Sci.}
	\gdef\@doiabbr{admsci}
	\gdef\@ISSN{2076-3387}
	\gdef\@societyowner{}
}
\DeclareOption{adolescents}{%
	\gdef\@journal{adolescents}
	\gdef\@journalfull{Adolescents}
	\gdef\@journalshort{Adolescents}
	\gdef\@doiabbr{adolescents}
	\gdef\@ISSN{2673-7051}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{aerobiology}{%
	\gdef\@journal{aerobiology}
	\gdef\@journalfull{Aerobiology}
	\gdef\@journalshort{Aerobiology}
	\gdef\@doiabbr{aerobiology}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{aerospace}{%
	\gdef\@journal{aerospace}
	\gdef\@journalfull{Aerospace}
	\gdef\@journalshort{Aerospace}
	\gdef\@doiabbr{aerospace}
	\gdef\@ISSN{2226-4310}
	\gdef\@societyowner{}
}
\DeclareOption{agriculture}{%
	\gdef\@journal{agriculture}
	\gdef\@journalfull{Agriculture}
	\gdef\@journalshort{Agriculture}
	\gdef\@doiabbr{agriculture}
	\gdef\@ISSN{2077-0472}
	\gdef\@societyowner{}
}
\DeclareOption{agriengineering}{%
	\gdef\@journal{agriengineering}
	\gdef\@journalfull{AgriEngineering}
	\gdef\@journalshort{AgriEngineering}
	\gdef\@doiabbr{agriengineering}
	\gdef\@ISSN{2624-7402}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{agrochemicals}{%
	\gdef\@journal{agrochemicals}
	\gdef\@journalfull{Agrochemicals}
	\gdef\@journalshort{Agrochemicals}
	\gdef\@doiabbr{agrochemicals}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{agronomy}{%
	\gdef\@journal{agronomy}
	\gdef\@journalfull{Agronomy}
	\gdef\@journalshort{Agronomy}
	\gdef\@doiabbr{agronomy}
	\gdef\@ISSN{2073-4395}
	\gdef\@societyowner{}
}
\DeclareOption{ai}{%
	\gdef\@journal{ai}
	\gdef\@journalfull{AI}
	\gdef\@journalshort{AI}
	\gdef\@doiabbr{ai}
	\gdef\@ISSN{2673-2688}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{air}{%
	\gdef\@journal{air}
	\gdef\@journalfull{Air}
	\gdef\@journalshort{Air}
	\gdef\@doiabbr{air}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{algorithms}{%
	\gdef\@journal{algorithms}
	\gdef\@journalfull{Algorithms}
	\gdef\@journalshort{Algorithms}
	\gdef\@doiabbr{a}
	\gdef\@ISSN{1999-4893}
	\gdef\@societyowner{}
}
\DeclareOption{allergies}{%
	\gdef\@journal{allergies}
	\gdef\@journalfull{Allergies}
	\gdef\@journalshort{Allergies}
	\gdef\@doiabbr{allergies}
	\gdef\@ISSN{2313-5786}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{alloys}{%
	\gdef\@journal{alloys}
	\gdef\@journalfull{Alloys}
	\gdef\@journalshort{Alloys}
	\gdef\@doiabbr{alloys}
	\gdef\@ISSN{2674-063X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{amh}{%
	\gdef\@journal{amh}
	\gdef\@journalfull{Acta Microbiologica Hellenica}
	\gdef\@journalshort{Acta Microbiol. Hell.}
	\gdef\@doiabbr{amh}
	\gdef\@ISSN{0438-9573}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{Hellenic Society for Microbiology}
}
\DeclareOption{analytica}{%
	\gdef\@journal{analytica}
	\gdef\@journalfull{Analytica}
	\gdef\@journalshort{Analytica}
	\gdef\@doiabbr{analytica}
	\gdef\@ISSN{2673-4532}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{analytics}{%
	\gdef\@journal{analytics}
	\gdef\@journalfull{Analytics}
	\gdef\@journalshort{Analytics}
	\gdef\@doiabbr{analytics}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{anatomia}{%
	\gdef\@journal{anatomia}
	\gdef\@journalfull{Anatomia}
	\gdef\@journalshort{Anatomia}
	\gdef\@doiabbr{anatomia}
	\gdef\@ISSN{2813-0545}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{anesthres}{%
	\gdef\@journal{anesthres}
	\gdef\@journalfull{Anesthesia Research}
	\gdef\@journalshort{Anesth. Res.}
	\gdef\@doiabbr{anesthres}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{animals}{%
	\gdef\@journal{animals}
	\gdef\@journalfull{Animals}
	\gdef\@journalshort{Animals}
	\gdef\@doiabbr{ani}
	\gdef\@ISSN{2076-2615}
	\gdef\@societyowner{}
}
\DeclareOption{antibiotics}{%
	\gdef\@journal{antibiotics}
	\gdef\@journalfull{Antibiotics}
	\gdef\@journalshort{Antibiotics}
	\gdef\@doiabbr{antibiotics}
	\gdef\@ISSN{2079-6382}
	\gdef\@societyowner{}
}
\DeclareOption{antibodies}{%
	\gdef\@journal{antibodies}
	\gdef\@journalfull{Antibodies}
	\gdef\@journalshort{Antibodies}
	\gdef\@doiabbr{antib}
	\gdef\@ISSN{2073-4468}
	\gdef\@societyowner{}
}
\DeclareOption{antioxidants}{%
	\gdef\@journal{antioxidants}
	\gdef\@journalfull{Antioxidants}
	\gdef\@journalshort{Antioxidants}
	\gdef\@doiabbr{antiox}
	\gdef\@ISSN{2076-3921}
	\gdef\@societyowner{}
}
\DeclareOption{applbiosci}{%
	\gdef\@journal{applbiosci}
	\gdef\@journalfull{Applied Biosciences}
	\gdef\@journalshort{Appl. Biosci.}
	\gdef\@doiabbr{applbiosci}
	\gdef\@ISSN{2813-0464}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{appliedchem}{%
	\gdef\@journal{appliedchem}
	\gdef\@journalfull{AppliedChem}
	\gdef\@journalshort{AppliedChem}
	\gdef\@doiabbr{appliedchem}
	\gdef\@ISSN{2673-9623}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{appliedmath}{%
	\gdef\@journal{appliedmath}
	\gdef\@journalfull{AppliedMath}
	\gdef\@journalshort{AppliedMath}
	\gdef\@doiabbr{appliedmath}
	\gdef\@ISSN{2673-9909}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{appliedphys}{%
	\gdef\@journal{appliedphys}
	\gdef\@journalfull{AppliedPhys}
	\gdef\@journalshort{AppliedPhys}
	\gdef\@doiabbr{appliedphys}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{applmech}{%
	\gdef\@journal{applmech}
	\gdef\@journalfull{Applied Mechanics}
	\gdef\@journalshort{Appl. Mech.}
	\gdef\@doiabbr{applmech}
	\gdef\@ISSN{2673-3161}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{applmicrobiol}{%
	\gdef\@journal{applmicrobiol}
	\gdef\@journalfull{Applied Microbiology}
	\gdef\@journalshort{Appl. Microbiol.}
	\gdef\@doiabbr{applmicrobiol}
	\gdef\@ISSN{2673-8007}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{applnano}{%
	\gdef\@journal{applnano}
	\gdef\@journalfull{Applied Nano}
	\gdef\@journalshort{Appl. Nano}
	\gdef\@doiabbr{applnano}
	\gdef\@ISSN{2673-3501}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{applsci}{%
	\gdef\@journal{applsci}
	\gdef\@journalfull{Applied Sciences}
	\gdef\@journalshort{Appl. Sci.}
	\gdef\@doiabbr{app}
	\gdef\@ISSN{2076-3417}
	\gdef\@societyowner{}
}
\DeclareOption{aquacj}{%
	\gdef\@journal{aquacj}
	\gdef\@journalfull{Aquaculture Journal}
	\gdef\@journalshort{Aquac. J.}
	\gdef\@doiabbr{aquacj}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{architecture}{%
	\gdef\@journal{architecture}
	\gdef\@journalfull{Architecture}
	\gdef\@journalshort{Architecture}
	\gdef\@doiabbr{architecture}
	\gdef\@ISSN{2673-8945}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{arm}{%
	\gdef\@journal{arm}
	\gdef\@journalfull{Advances in Respiratory Medicine}
	\gdef\@journalshort{Adv. Respir. Med.}
	\gdef\@doiabbr{arm}
	\gdef\@ISSN{2543-6031}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{Polish Respiratory Society}
}
\DeclareOption{arthropoda}{%
	\gdef\@journal{arthropoda}
	\gdef\@journalfull{Arthropoda}
	\gdef\@journalshort{Arthropoda}
	\gdef\@doiabbr{arthropoda}
	\gdef\@ISSN{2813-3323}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{arts}{%
	\gdef\@journal{arts}
	\gdef\@journalfull{Arts}
	\gdef\@journalshort{Arts}
	\gdef\@doiabbr{arts}
	\gdef\@ISSN{2076-0752}
	\gdef\@societyowner{}
}
\DeclareOption{asc}{%
	\gdef\@journal{asc}
	\gdef\@journalfull{Automatic Systems and Control}
	\gdef\@journalshort{Autom. Syst. Control}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{asi}{%
	\gdef\@journal{asi}
	\gdef\@journalfull{Applied System Innovation}
	\gdef\@journalshort{Appl. Syst. Innov.}
	\gdef\@doiabbr{asi}
	\gdef\@ISSN{2571-5577}
	\gdef\@societyowner{International Institute of Knowledge Innovation and Invention}
}
\DeclareOption{astronomy}{%
	\gdef\@journal{astronomy}
	\gdef\@journalfull{Astronomy}
	\gdef\@journalshort{Astronomy}
	\gdef\@doiabbr{astronomy}
	\gdef\@ISSN{2674-0346}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{atmosphere}{%
	\gdef\@journal{atmosphere}
	\gdef\@journalfull{Atmosphere}
	\gdef\@journalshort{Atmosphere}
	\gdef\@doiabbr{atmos}
	\gdef\@ISSN{2073-4433}
	\gdef\@societyowner{}
}
\DeclareOption{atoms}{%
	\gdef\@journal{atoms}
	\gdef\@journalfull{Atoms}
	\gdef\@journalshort{Atoms}
	\gdef\@doiabbr{atoms}
	\gdef\@ISSN{2218-2004}
	\gdef\@societyowner{}
}
\DeclareOption{audiolres}{%
	\gdef\@journal{audiolres}
	\gdef\@journalfull{Audiology Research}
	\gdef\@journalshort{Audiol. Res.}
	\gdef\@doiabbr{audiolres}
	\gdef\@ISSN{2039-4349}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{automation}{%
	\gdef\@journal{automation}
	\gdef\@journalfull{Automation}
	\gdef\@journalshort{Automation}
	\gdef\@doiabbr{automation}
	\gdef\@ISSN{2673-4052}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{axioms}{%
	\gdef\@journal{axioms}
	\gdef\@journalfull{Axioms}
	\gdef\@journalshort{Axioms}
	\gdef\@doiabbr{axioms}
	\gdef\@ISSN{2075-1680}
	\gdef\@societyowner{}
}
\DeclareOption{bacteria}{%
	\gdef\@journal{bacteria}
	\gdef\@journalfull{Bacteria}
	\gdef\@journalshort{Bacteria}
	\gdef\@doiabbr{bacteria}
	\gdef\@ISSN{2674-1334}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{batteries}{%
	\gdef\@journal{batteries}
	\gdef\@journalfull{Batteries}
	\gdef\@journalshort{Batteries}
	\gdef\@doiabbr{batteries}
	\gdef\@ISSN{2313-0105}
	\gdef\@societyowner{}
}
\DeclareOption{bdcc}{%
	\gdef\@journal{bdcc}
	\gdef\@journalfull{Big Data and Cognitive Computing}
	\gdef\@journalshort{Big Data Cogn. Comput.}
	\gdef\@doiabbr{bdcc}
	\gdef\@ISSN{2504-2289}
	\gdef\@societyowner{}
}
\DeclareOption{behavsci}{%
	\gdef\@journal{behavsci}
	\gdef\@journalfull{Behavioral Sciences}
	\gdef\@journalshort{Behav. Sci.}
	\gdef\@doiabbr{bs}
	\gdef\@ISSN{2076-328X}
	\gdef\@societyowner{}
}
\DeclareOption{beverages}{%
	\gdef\@journal{beverages}
	\gdef\@journalfull{Beverages}
	\gdef\@journalshort{Beverages}
	\gdef\@doiabbr{beverages}
	\gdef\@ISSN{2306-5710}
	\gdef\@societyowner{}
}
\DeclareOption{biochem}{%
	\gdef\@journal{biochem}
	\gdef\@journalfull{BioChem}
	\gdef\@journalshort{BioChem}
	\gdef\@doiabbr{biochem}
	\gdef\@ISSN{2673-6411}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{bioengineering}{%
	\gdef\@journal{bioengineering}
	\gdef\@journalfull{Bioengineering}
	\gdef\@journalshort{Bioengineering}
	\gdef\@doiabbr{bioengineering}
	\gdef\@ISSN{2306-5354}
	\gdef\@societyowner{}
}
\DeclareOption{biologics}{%
	\gdef\@journal{biologics}
	\gdef\@journalfull{Biologics}
	\gdef\@journalshort{Biologics}
	\gdef\@doiabbr{biologics}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{biology}{%
	\gdef\@journal{biology}
	\gdef\@journalfull{Biology}
	\gdef\@journalshort{Biology}
	\gdef\@doiabbr{biology}
	\gdef\@ISSN{2079-7737}
	\gdef\@societyowner{}
}
\DeclareOption{biomass}{%
	\gdef\@journal{biomass}
	\gdef\@journalfull{Biomass}
	\gdef\@journalshort{Biomass}
	\gdef\@doiabbr{biomass}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{biomechanics}{%
	\gdef\@journal{biomechanics}
	\gdef\@journalfull{Biomechanics}
	\gdef\@journalshort{Biomechanics}
	\gdef\@doiabbr{biomechanics}
	\gdef\@ISSN{2673-7078}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{biomed}{%
	\gdef\@journal{biomed}
	\gdef\@journalfull{BioMed}
	\gdef\@journalshort{BioMed}
	\gdef\@doiabbr{biomed}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{biomedicines}{%
	\gdef\@journal{biomedicines}
	\gdef\@journalfull{Biomedicines}
	\gdef\@journalshort{Biomedicines}
	\gdef\@doiabbr{biomedicines}
	\gdef\@ISSN{2227-9059}
	\gdef\@societyowner{}
}
\DeclareOption{biomedinformatics}{%
	\gdef\@journal{biomedinformatics}
	\gdef\@journalfull{BioMedInformatics}
	\gdef\@journalshort{BioMedInformatics}
	\gdef\@doiabbr{biomedinformatics}
	\gdef\@ISSN{2673-7426}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{biomimetics}{%
	\gdef\@journal{biomimetics}
	\gdef\@journalfull{Biomimetics}
	\gdef\@journalshort{Biomimetics}
	\gdef\@doiabbr{biomimetics}
	\gdef\@ISSN{2313-7673}
	\gdef\@societyowner{}
}
\DeclareOption{biomolecules}{%
	\gdef\@journal{biomolecules}
	\gdef\@journalfull{Biomolecules}
	\gdef\@journalshort{Biomolecules}
	\gdef\@doiabbr{biom}
	\gdef\@ISSN{2218-273X}
	\gdef\@societyowner{}
}
\DeclareOption{biophysica}{%
	\gdef\@journal{biophysica}
	\gdef\@journalfull{Biophysica}
	\gdef\@journalshort{Biophysica}
	\gdef\@doiabbr{biophysica}
	\gdef\@ISSN{2673-4125}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{biosensors}{%
	\gdef\@journal{biosensors}
	\gdef\@journalfull{Biosensors}
	\gdef\@journalshort{Biosensors}
	\gdef\@doiabbr{bios}
	\gdef\@ISSN{2079-6374}
	\gdef\@societyowner{}
}
\DeclareOption{biotech}{%
	\gdef\@journal{biotech}
	\gdef\@journalfull{BioTech}
	\gdef\@journalshort{BioTech}
	\gdef\@doiabbr{biotech}
	\gdef\@ISSN{2673-6284}
	\gdef\@societyowner{}
}
\DeclareOption{birds}{%
	\gdef\@journal{birds}
	\gdef\@journalfull{Birds}
	\gdef\@journalshort{Birds}
	\gdef\@doiabbr{birds}
	\gdef\@ISSN{2673-6004}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{blockchains}{%
	\gdef\@journal{blockchains}
	\gdef\@journalfull{Blockchains}
	\gdef\@journalshort{Blockchains}
	\gdef\@doiabbr{blockchains}
	\gdef\@ISSN{2813-5288}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{bloods}{%
	\gdef\@journal{bloods}
	\gdef\@journalfull{Bloods}
	\gdef\@journalshort{Bloods}
	\gdef\@doiabbr{bloods}
	\gdef\@ISSN{2673-415X}
	\gdef\@societyowner{}
}
\DeclareOption{blsf}{%
	\gdef\@journal{blsf}
	\gdef\@journalfull{Biology and Life Sciences Forum}
	\gdef\@journalshort{Biol. Life Sci. Forum}
	\gdef\@doiabbr{blsf}
	\gdef\@ISSN{2673-9976}
	\gdef\@societyowner{}
}
\DeclareOption{brainsci}{%
	\gdef\@journal{brainsci}
	\gdef\@journalfull{Brain Sciences}
	\gdef\@journalshort{Brain Sci.}
	\gdef\@doiabbr{brainsci}
	\gdef\@ISSN{2076-3425}
	\gdef\@societyowner{}
}
\DeclareOption{breath}{%
	\gdef\@journal{breath}
	\gdef\@journalfull{Breath}
	\gdef\@journalshort{Breath}
	\gdef\@doiabbr{breath}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{buildings}{%
	\gdef\@journal{buildings}
	\gdef\@journalfull{Buildings}
	\gdef\@journalshort{Buildings}
	\gdef\@doiabbr{buildings}
	\gdef\@ISSN{2075-5309}
	\gdef\@societyowner{}
}
\DeclareOption{businesses}{%
	\gdef\@journal{businesses}
	\gdef\@journalfull{Businesses}
	\gdef\@journalshort{Businesses}
	\gdef\@doiabbr{businesses}
	\gdef\@ISSN{2673-7116}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cancers}{%
	\gdef\@journal{cancers}
	\gdef\@journalfull{Cancers}
	\gdef\@journalshort{Cancers}
	\gdef\@doiabbr{cancers}
	\gdef\@ISSN{2072-6694}
	\gdef\@societyowner{}
}
\DeclareOption{carbon}{%
	\gdef\@journal{carbon}
	\gdef\@journalfull{C}
	\gdef\@journalshort{C}
	\gdef\@doiabbr{c}
	\gdef\@ISSN{2311-5629}
	\gdef\@societyowner{}
}
\DeclareOption{cardiogenetics}{%
	\gdef\@journal{cardiogenetics}
	\gdef\@journalfull{Cardiogenetics}
	\gdef\@journalshort{Cardiogenetics}
	\gdef\@doiabbr{cardiogenetics}
	\gdef\@ISSN{2035-8148}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{catalysts}{%
	\gdef\@journal{catalysts}
	\gdef\@journalfull{Catalysts}
	\gdef\@journalshort{Catalysts}
	\gdef\@doiabbr{catal}
	\gdef\@ISSN{2073-4344}
	\gdef\@societyowner{}
}
\DeclareOption{cells}{%
	\gdef\@journal{cells}
	\gdef\@journalfull{Cells}
	\gdef\@journalshort{Cells}
	\gdef\@doiabbr{cells}
	\gdef\@ISSN{2073-4409}
	\gdef\@societyowner{}
}
\DeclareOption{ceramics}{%
	\gdef\@journal{ceramics}
	\gdef\@journalfull{Ceramics}
	\gdef\@journalshort{Ceramics}
	\gdef\@doiabbr{ceramics}
	\gdef\@ISSN{2571-6131}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{challenges}{%
	\gdef\@journal{challenges}
	\gdef\@journalfull{Challenges}
	\gdef\@journalshort{Challenges}
	\gdef\@doiabbr{challe}
	\gdef\@ISSN{2078-1547}
	\gdef\@societyowner{}
}
\DeclareOption{chemengineering}{%
	\gdef\@journal{chemengineering}
	\gdef\@journalfull{ChemEngineering}
	\gdef\@journalshort{ChemEngineering}
	\gdef\@doiabbr{chemengineering}
	\gdef\@ISSN{2305-7084}
	\gdef\@societyowner{}
}
\DeclareOption{chemistry}{%
	\gdef\@journal{chemistry}
	\gdef\@journalfull{Chemistry}
	\gdef\@journalshort{Chemistry}
	\gdef\@doiabbr{chemistry}
	\gdef\@ISSN{2624-8549}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{chemosensors}{%
	\gdef\@journal{chemosensors}
	\gdef\@journalfull{Chemosensors}
	\gdef\@journalshort{Chemosensors}
	\gdef\@doiabbr{chemosensors}
	\gdef\@ISSN{2227-9040}
	\gdef\@societyowner{}
}
\DeclareOption{chemproc}{%
	\gdef\@journal{chemproc}
	\gdef\@journalfull{Chemistry Proceedings}
	\gdef\@journalshort{Chem. Proc.}
	\gdef\@doiabbr{chemproc}
	\gdef\@ISSN{2673-4583}
	\gdef\@societyowner{}
}
\DeclareOption{children}{%
	\gdef\@journal{children}
	\gdef\@journalfull{Children}
	\gdef\@journalshort{Children}
	\gdef\@doiabbr{children}
	\gdef\@ISSN{2227-9067}
	\gdef\@societyowner{}
}
\DeclareOption{chips}{%
	\gdef\@journal{chips}
	\gdef\@journalfull{Chips}
	\gdef\@journalshort{Chips}
	\gdef\@doiabbr{chips}
	\gdef\@ISSN{2674-0729}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cimb}{%
	\gdef\@journal{cimb}
	\gdef\@journalfull{Current Issues in Molecular Biology}
	\gdef\@journalshort{Curr. Issues Mol. Biol.}
	\gdef\@doiabbr{cimb}
	\gdef\@ISSN{1467-3045}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{civileng}{%
	\gdef\@journal{civileng}
	\gdef\@journalfull{CivilEng}
	\gdef\@journalshort{CivilEng}
	\gdef\@doiabbr{civileng}
	\gdef\@ISSN{2673-4109}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cleantechnol}{%
	\gdef\@journal{cleantechnol}
	\gdef\@journalfull{Clean Technologies}
	\gdef\@journalshort{Clean Technol.}
	\gdef\@doiabbr{cleantechnol}
	\gdef\@ISSN{2571-8797}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{climate}{%
	\gdef\@journal{climate}
	\gdef\@journalfull{Climate}
	\gdef\@journalshort{Climate}
	\gdef\@doiabbr{cli}
	\gdef\@ISSN{2225-1154}
	\gdef\@societyowner{}
}
\DeclareOption{clinpract}{%
	\gdef\@journal{clinpract}
	\gdef\@journalfull{Clinics and Practice}
	\gdef\@journalshort{Clin. Pract.}
	\gdef\@doiabbr{clinpract}
	\gdef\@ISSN{2039-7283}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{clockssleep}{%
	\gdef\@journal{clockssleep}
	\gdef\@journalfull{Clocks \& Sleep}
	\gdef\@journalshort{Clocks\&Sleep}
	\gdef\@doiabbr{clockssleep}
	\gdef\@ISSN{2624-5175}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cmd}{%
	\gdef\@journal{cmd}
	\gdef\@journalfull{Corrosion and Materials Degradation}
	\gdef\@journalshort{Corros. Mater. Degrad.}
	\gdef\@doiabbr{cmd}
	\gdef\@ISSN{2624-5558}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{coasts}{%
	\gdef\@journal{coasts}
	\gdef\@journalfull{Coasts}
	\gdef\@journalshort{Coasts}
	\gdef\@doiabbr{coasts}
	\gdef\@ISSN{2673-964X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{coatings}{%
	\gdef\@journal{coatings}
	\gdef\@journalfull{Coatings}
	\gdef\@journalshort{Coatings}
	\gdef\@doiabbr{coatings}
	\gdef\@ISSN{2079-6412}
	\gdef\@societyowner{}
}
\DeclareOption{colloids}{%
	\gdef\@journal{colloids}
	\gdef\@journalfull{Colloids and Interfaces}
	\gdef\@journalshort{Colloids Interfaces}
	\gdef\@doiabbr{colloids}
	\gdef\@ISSN{2504-5377}
	\gdef\@societyowner{}
}
\DeclareOption{colorants}{%
	\gdef\@journal{colorants}
	\gdef\@journalfull{Colorants}
	\gdef\@journalshort{Colorants}
	\gdef\@doiabbr{colorants}
	\gdef\@ISSN{2079-6447}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{commodities}{%
	\gdef\@journal{commodities}
	\gdef\@journalfull{Commodities}
	\gdef\@journalshort{Commodities}
	\gdef\@doiabbr{commodities}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{complications}{%
       \gdef\@journal{complications}
       \gdef\@journalfull{Complications}
       \gdef\@journalshort{Complications}
       \gdef\@doiabbr{complications}
       \gdef\@ISSN{}
       \gdef\@continuouspages{yes}
       \gdef\@societyowner{}
}
\DeclareOption{compounds}{%
	\gdef\@journal{compounds}
	\gdef\@journalfull{Compounds}
	\gdef\@journalshort{Compounds}
	\gdef\@doiabbr{compounds}
	\gdef\@ISSN{2673-6918}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{computation}{%
	\gdef\@journal{computation}
	\gdef\@journalfull{Computation}
	\gdef\@journalshort{Computation}
	\gdef\@doiabbr{computation}
	\gdef\@ISSN{2079-3197}
	\gdef\@societyowner{}
}
\DeclareOption{computers}{%
	\gdef\@journal{computers}
	\gdef\@journalfull{Computers}
	\gdef\@journalshort{Computers}
	\gdef\@doiabbr{computers}
	\gdef\@ISSN{2073-431X}
	\gdef\@societyowner{}
}
\DeclareOption{condensedmatter}{%
	\gdef\@journal{condensedmatter}
	\gdef\@journalfull{Condensed Matter}
	\gdef\@journalshort{Condens. Matter}
	\gdef\@doiabbr{condmat}
	\gdef\@ISSN{2410-3896}
	\gdef\@societyowner{}
}
\DeclareOption{conservation}{%
	\gdef\@journal{conservation}
	\gdef\@journalfull{Conservation}
	\gdef\@journalshort{Conservation}
	\gdef\@doiabbr{conservation}
	\gdef\@ISSN{2673-7159}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{constrmater}{%
	\gdef\@journal{constrmater}
	\gdef\@journalfull{Construction Materials}
	\gdef\@journalshort{Constr. Mater.}
	\gdef\@doiabbr{constrmater}
	\gdef\@ISSN{2673-7108}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cosmetics}{%
	\gdef\@journal{cosmetics}
	\gdef\@journalfull{Cosmetics}
	\gdef\@journalshort{Cosmetics}
	\gdef\@doiabbr{cosmetics}
	\gdef\@ISSN{2079-9284}
	\gdef\@societyowner{}
}
\DeclareOption{covid}{%
	\gdef\@journal{covid}
	\gdef\@journalfull{COVID}
	\gdef\@journalshort{COVID}
	\gdef\@doiabbr{covid}
	\gdef\@ISSN{2673-8112}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{crops}{%
	\gdef\@journal{crops}
	\gdef\@journalfull{Crops}
	\gdef\@journalshort{Crops}
	\gdef\@doiabbr{crops}
	\gdef\@ISSN{2673-7655}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cryo}{%
	\gdef\@journal{cryo}
	\gdef\@journalfull{Cryo}
	\gdef\@journalshort{Cryo}
	\gdef\@doiabbr{cryo}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cryptography}{%
	\gdef\@journal{cryptography}
	\gdef\@journalfull{Cryptography}
	\gdef\@journalshort{Cryptography}
	\gdef\@doiabbr{cryptography}
	\gdef\@ISSN{2410-387X}
	\gdef\@societyowner{}
}
\DeclareOption{crystals}{%
	\gdef\@journal{crystals}
	\gdef\@journalfull{Crystals}
	\gdef\@journalshort{Crystals}
	\gdef\@doiabbr{cryst}
	\gdef\@ISSN{2073-4352}
	\gdef\@societyowner{}
}
\DeclareOption{csmf}{%
	\gdef\@journal{csmf}
	\gdef\@journalfull{Computer Sciences \& Mathematics Forum}
	\gdef\@journalshort{Comput. Sci. Math. Forum}
	\gdef\@doiabbr{csmf}
	\gdef\@ISSN{2813-0324}
	\gdef\@societyowner{}
}
\DeclareOption{ctn}{%
	\gdef\@journal{ctn}
	\gdef\@journalfull{Clinical and Translational Neuroscience}
	\gdef\@journalshort{Clin. Transl. Neurosci.}
	\gdef\@doiabbr{ctn}
	\gdef\@ISSN{2514-183X}
	\gdef\@societyowner{Swiss Federation of Clinical Neuro-Societies}
}
\DeclareOption{curroncol}{%
	\gdef\@journal{curroncol}
	\gdef\@journalfull{Current Oncology}
	\gdef\@journalshort{Curr. Oncol.}
	\gdef\@doiabbr{curroncol}
	\gdef\@ISSN{1718-7729}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cyber}{%
	\gdef\@journal{cyber}
	\gdef\@journalfull{Cyber}
	\gdef\@journalshort{Cyber}
	\gdef\@doiabbr{cyber}
	\gdef\@ISSN{2624-800X}
	\gdef\@societyowner{}
}
\DeclareOption{dairy}{%
	\gdef\@journal{dairy}
	\gdef\@journalfull{Dairy}
	\gdef\@journalshort{Dairy}
	\gdef\@doiabbr{dairy}
	\gdef\@ISSN{2624-862X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{data}{%
	\gdef\@journal{data}
	\gdef\@journalfull{Data}
	\gdef\@journalshort{Data}
	\gdef\@doiabbr{data}
	\gdef\@ISSN{2306-5729}
	\gdef\@societyowner{}
}
\DeclareOption{ddc}{%
	\gdef\@journal{ddc}
	\gdef\@journalfull{Drugs and Drug Candidates}
	\gdef\@journalshort{Drugs Drug Candidates}
	\gdef\@doiabbr{ddc}
	\gdef\@ISSN{2813-2998}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{dentistry}{%
	\gdef\@journal{dentistry}
	\gdef\@journalfull{Dentistry Journal}
	\gdef\@journalshort{Dent. J.}
	\gdef\@doiabbr{dj}
	\gdef\@ISSN{2304-6767}
	\gdef\@societyowner{}
}
\DeclareOption{dermato}{%
	\gdef\@journal{dermato}
	\gdef\@journalfull{Dermato}
	\gdef\@journalshort{Dermato}
	\gdef\@doiabbr{dermato}
	\gdef\@ISSN{2673-6179}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{dermatopathology}{%
	\gdef\@journal{dermatopathology}
	\gdef\@journalfull{Dermatopathology}
	\gdef\@journalshort{Dermatopathology}
	\gdef\@doiabbr{dermatopathology}
	\gdef\@ISSN{2296-3529}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{European Society of Dermatopathology}
}
\DeclareOption{designs}{%
	\gdef\@journal{designs}
	\gdef\@journalfull{Designs}
	\gdef\@journalshort{Designs}
	\gdef\@doiabbr{designs}
	\gdef\@ISSN{2411-9660}
	\gdef\@societyowner{}
}
\DeclareOption{devices}{%
	\gdef\@journal{devices}
	\gdef\@journalfull{Devices}
	\gdef\@journalshort{Devices}
	\gdef\@doiabbr{devices}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{diabetology}{%
	\gdef\@journal{diabetology}
	\gdef\@journalfull{Diabetology}
	\gdef\@journalshort{Diabetology}
	\gdef\@doiabbr{diabetology}
	\gdef\@ISSN{2673-4540}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{diagnostics}{%
	\gdef\@journal{diagnostics}
	\gdef\@journalfull{Diagnostics}
	\gdef\@journalshort{Diagnostics}
	\gdef\@doiabbr{diagnostics}
	\gdef\@ISSN{2075-4418}
	\gdef\@societyowner{}
}
\DeclareOption{dietetics}{%
	\gdef\@journal{dietetics}
	\gdef\@journalfull{Dietetics}
	\gdef\@journalshort{Dietetics}
	\gdef\@doiabbr{dietetics}
	\gdef\@ISSN{2674-0311}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{digital}{%
	\gdef\@journal{digital}
	\gdef\@journalfull{Digital}
	\gdef\@journalshort{Digital}
	\gdef\@doiabbr{digital}
	\gdef\@ISSN{2673-6470}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{disabilities}{%
	\gdef\@journal{disabilities}
	\gdef\@journalfull{Disabilities}
	\gdef\@journalshort{Disabilities}
	\gdef\@doiabbr{disabilities}
	\gdef\@ISSN{2673-7272}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{diseases}{%
	\gdef\@journal{diseases}
	\gdef\@journalfull{Diseases}
	\gdef\@journalshort{Diseases}
	\gdef\@doiabbr{diseases}
	\gdef\@ISSN{2079-9721}
	\gdef\@societyowner{}
}
\DeclareOption{diversity}{%
	\gdef\@journal{diversity}
	\gdef\@journalfull{Diversity}
	\gdef\@journalshort{Diversity}
	\gdef\@doiabbr{d}
	\gdef\@ISSN{1424-2818}
	\gdef\@societyowner{}
}
\DeclareOption{dna}{%
	\gdef\@journal{dna}
	\gdef\@journalfull{DNA}
	\gdef\@journalshort{DNA}
	\gdef\@doiabbr{dna}
	\gdef\@ISSN{2673-8856}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{drones}{%
	\gdef\@journal{drones}
	\gdef\@journalfull{Drones}
	\gdef\@journalshort{Drones}
	\gdef\@doiabbr{drones}
	\gdef\@ISSN{2504-446X}
	\gdef\@societyowner{}
}
\DeclareOption{dynamics}{%
	\gdef\@journal{dynamics}
	\gdef\@journalfull{Dynamics}
	\gdef\@journalshort{Dynamics}
	\gdef\@doiabbr{dynamics}
	\gdef\@ISSN{2673-8716}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{earth}{%
	\gdef\@journal{earth}
	\gdef\@journalfull{Earth}
	\gdef\@journalshort{Earth}
	\gdef\@doiabbr{earth}
	\gdef\@ISSN{2673-4834}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ebj}{%
	\gdef\@journal{ebj}
	\gdef\@journalfull{European Burn Journal}
	\gdef\@journalshort{Eur. Burn J.}
	\gdef\@doiabbr{ebj}
	\gdef\@ISSN{2673-1991}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{European Burns Association}
}
\DeclareOption{ecm}{%
	\gdef\@journal{ecm}
	\gdef\@journalfull{Emergency Care and Medicine}
	\gdef\@journalshort{Emerg. Care Med.}
	\gdef\@doiabbr{ecm}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ecologies}{%
	\gdef\@journal{ecologies}
	\gdef\@journalfull{Ecologies}
	\gdef\@journalshort{Ecologies}
	\gdef\@doiabbr{ecologies}
	\gdef\@ISSN{2673-4133}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{econometrics}{%
	\gdef\@journal{econometrics}
	\gdef\@journalfull{Econometrics}
	\gdef\@journalshort{Econometrics}
	\gdef\@doiabbr{econometrics}
	\gdef\@ISSN{2225-1146}
	\gdef\@societyowner{}
}
\DeclareOption{economies}{%
	\gdef\@journal{economies}
	\gdef\@journalfull{Economies}
	\gdef\@journalshort{Economies}
	\gdef\@doiabbr{economies}
	\gdef\@ISSN{2227-7099}
	\gdef\@societyowner{}
}
\DeclareOption{education}{%
	\gdef\@journal{education}
	\gdef\@journalfull{Education Sciences}
	\gdef\@journalshort{Educ. Sci.}
	\gdef\@doiabbr{educsci}
	\gdef\@ISSN{2227-7102}
	\gdef\@societyowner{}
}
\DeclareOption{ejihpe}{%
	\gdef\@journal{ejihpe}
	\gdef\@journalfull{European Journal of Investigation in Health, Psychology and Education}
	\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}
	\gdef\@doiabbr{ejihpe}
	\gdef\@ISSN{2254-9625}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{University Association of Education and Psychology}
}
\DeclareOption{electricity}{%
	\gdef\@journal{electricity}
	\gdef\@journalfull{Electricity}
	\gdef\@journalshort{Electricity}
	\gdef\@doiabbr{electricity}
	\gdef\@ISSN{2673-4826}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{electrochem}{%
	\gdef\@journal{electrochem}
	\gdef\@journalfull{Electrochem}
	\gdef\@journalshort{Electrochem}
	\gdef\@doiabbr{electrochem}
	\gdef\@ISSN{2673-3293}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{electronicmat}{%
	\gdef\@journal{electronicmat}
	\gdef\@journalfull{Electronic Materials}
	\gdef\@journalshort{Electron. Mater.}
	\gdef\@doiabbr{electronicmat}
	\gdef\@ISSN{2673-3978}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{electronics}{%
	\gdef\@journal{electronics}
	\gdef\@journalfull{Electronics}
	\gdef\@journalshort{Electronics}
	\gdef\@doiabbr{electronics}
	\gdef\@ISSN{2079-9292}
	\gdef\@societyowner{}
}
\DeclareOption{encyclopedia}{%
	\gdef\@journal{encyclopedia}
	\gdef\@journalfull{Encyclopedia}
	\gdef\@journalshort{Encyclopedia}
	\gdef\@doiabbr{encyclopedia}
	\gdef\@ISSN{2673-8392}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{endocrines}{%
	\gdef\@journal{endocrines}
	\gdef\@journalfull{Endocrines}
	\gdef\@journalshort{Endocrines}
	\gdef\@doiabbr{endocrines}
	\gdef\@ISSN{2673-396X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{energies}{%
	\gdef\@journal{energies}
	\gdef\@journalfull{Energies}
	\gdef\@journalshort{Energies}
	\gdef\@doiabbr{en}
	\gdef\@ISSN{1996-1073}
	\gdef\@societyowner{}
}
\DeclareOption{eng}{%
	\gdef\@journal{eng}
	\gdef\@journalfull{Eng}
	\gdef\@journalshort{Eng}
	\gdef\@doiabbr{eng}
	\gdef\@ISSN{2673-4117}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{engproc}{%
	\gdef\@journal{engproc}
	\gdef\@journalfull{Engineering Proceedings}
	\gdef\@journalshort{Eng. Proc.}
	\gdef\@doiabbr{engproc}
	\gdef\@ISSN{2673-4591}
	\gdef\@societyowner{}
}
%\DeclareOption{ent}{%
%	\gdef\@journal{ent}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{entomology}{%
	\gdef\@journal{entomology}
	\gdef\@journalfull{Entomology}
	\gdef\@journalshort{Entomology}
	\gdef\@doiabbr{entomology}
	\gdef\@ISSN{2813-0502}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{entropy}{%
	\gdef\@journal{entropy}
	\gdef\@journalfull{Entropy}
	\gdef\@journalshort{Entropy}
	\gdef\@doiabbr{e}
	\gdef\@ISSN{1099-4300}
	\gdef\@societyowner{}
}
\DeclareOption{environments}{%
	\gdef\@journal{environments}
	\gdef\@journalfull{Environments}
	\gdef\@journalshort{Environments}
	\gdef\@doiabbr{environments}
	\gdef\@ISSN{2076-3298}
	\gdef\@societyowner{}
}
\DeclareOption{environsciproc}{%
	\gdef\@journal{environsciproc}
	\gdef\@journalfull{Environmental Sciences Proceedings}
	\gdef\@journalshort{Environ. Sci. Proc.}
	\gdef\@doiabbr{environsciproc}
	\gdef\@ISSN{2673-4931}
	\gdef\@societyowner{}
}
\DeclareOption{epidemiologia}{%
	\gdef\@journal{epidemiologia}
	\gdef\@journalfull{Epidemiologia}
	\gdef\@journalshort{Epidemiologia}
	\gdef\@doiabbr{epidemiologia}
	\gdef\@ISSN{2673-3986}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{epigenomes}{%
	\gdef\@journal{epigenomes}
	\gdef\@journalfull{Epigenomes}
	\gdef\@journalshort{Epigenomes}
	\gdef\@doiabbr{epigenomes}
	\gdef\@ISSN{2075-4655}
	\gdef\@societyowner{}
}
\DeclareOption{esa}{%
	\gdef\@journal{esa}
	\gdef\@journalfull{Energy Storage and Applications}
	\gdef\@journalshort{Energy Storage Appl.}
	\gdef\@doiabbr{esa}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{est}{%
	\gdef\@journal{est}
	\gdef\@journalfull{Electrochemical Science and Technology}
	\gdef\@journalshort{Electrochem. Sci. Technol.}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{fermentation}{%
	\gdef\@journal{fermentation}
	\gdef\@journalfull{Fermentation}
	\gdef\@journalshort{Fermentation}
	\gdef\@doiabbr{fermentation}
	\gdef\@ISSN{2311-5637}
	\gdef\@societyowner{}
}
\DeclareOption{fibers}{%
	\gdef\@journal{fibers}
	\gdef\@journalfull{Fibers}
	\gdef\@journalshort{Fibers}
	\gdef\@doiabbr{fib}
	\gdef\@ISSN{2079-6439}
	\gdef\@societyowner{}
}
\DeclareOption{fintech}{%
	\gdef\@journal{fintech}
	\gdef\@journalfull{FinTech}
	\gdef\@journalshort{FinTech}
	\gdef\@doiabbr{fintech}
	\gdef\@ISSN{2674-1032}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fire}{%
	\gdef\@journal{fire}
	\gdef\@journalfull{Fire}
	\gdef\@journalshort{Fire}
	\gdef\@doiabbr{fire}
	\gdef\@ISSN{2571-6255}
	\gdef\@societyowner{}
}
\DeclareOption{fishes}{%
	\gdef\@journal{fishes}
	\gdef\@journalfull{Fishes}
	\gdef\@journalshort{Fishes}
	\gdef\@doiabbr{fishes}
	\gdef\@ISSN{2410-3888}
	\gdef\@societyowner{}
}
\DeclareOption{fluids}{%
	\gdef\@journal{fluids}
	\gdef\@journalfull{Fluids}
	\gdef\@journalshort{Fluids}
	\gdef\@doiabbr{fluids}
	\gdef\@ISSN{2311-5521}
	\gdef\@societyowner{}
}
\DeclareOption{foods}{%
	\gdef\@journal{foods}
	\gdef\@journalfull{Foods}
	\gdef\@journalshort{Foods}
	\gdef\@doiabbr{foods}
	\gdef\@ISSN{2304-8158}
	\gdef\@societyowner{}
}
\DeclareOption{forecasting}{%
	\gdef\@journal{forecasting}
	\gdef\@journalfull{Forecasting}
	\gdef\@journalshort{Forecasting}
	\gdef\@doiabbr{forecast}
	\gdef\@ISSN{2571-9394}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{forensicsci}{%
	\gdef\@journal{forensicsci}
	\gdef\@journalfull{Forensic Sciences}
	\gdef\@journalshort{Forensic Sci.}
	\gdef\@doiabbr{forensicsci}
	\gdef\@ISSN{2673-6756}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{forests}{%
	\gdef\@journal{forests}
	\gdef\@journalfull{Forests}
	\gdef\@journalshort{Forests}
	\gdef\@doiabbr{f}
	\gdef\@ISSN{1999-4907}
	\gdef\@societyowner{}
}
\DeclareOption{fossstud}{%
	\gdef\@journal{fossstud}
	\gdef\@journalfull{Fossil Studies}
	\gdef\@journalshort{Foss. Stud.}
	\gdef\@doiabbr{fossils}
	\gdef\@ISSN{2813-6284}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{foundations}{%
	\gdef\@journal{foundations}
	\gdef\@journalfull{Foundations}
	\gdef\@journalshort{Foundations}
	\gdef\@doiabbr{foundations}
	\gdef\@ISSN{2673-9321}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fractalfract}{%
	\gdef\@journal{fractalfract}
	\gdef\@journalfull{Fractal and Fractional}
	\gdef\@journalshort{Fractal Fract.}
	\gdef\@doiabbr{fractalfract}
	\gdef\@ISSN{2504-3110}
	\gdef\@societyowner{}
}
\DeclareOption{fuels}{%
	\gdef\@journal{fuels}
	\gdef\@journalfull{Fuels}
	\gdef\@journalshort{Fuels}
	\gdef\@doiabbr{fuels}
	\gdef\@ISSN{2673-3994}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{future}{%
	\gdef\@journal{future}
	\gdef\@journalfull{Future}
	\gdef\@journalshort{Future}
	\gdef\@doiabbr{future}
	\gdef\@ISSN{2813-2882}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{futureinternet}{%
	\gdef\@journal{futureinternet}
	\gdef\@journalfull{Future Internet}
	\gdef\@journalshort{Future Internet}
	\gdef\@doiabbr{fi}
	\gdef\@ISSN{1999-5903}
	\gdef\@societyowner{}
}
%\DeclareOption{futureparasites}{%
%	\gdef\@journal{futureparasites}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{futurepharmacol}{%
	\gdef\@journal{futurepharmacol}
	\gdef\@journalfull{Future Pharmacology}
	\gdef\@journalshort{Future Pharmacol.}
	\gdef\@doiabbr{futurepharmacol}
	\gdef\@ISSN{2673-9879}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{futurephys}{%
	\gdef\@journal{futurephys}
	\gdef\@journalfull{Future Physics}
	\gdef\@journalshort{Future Phys.}
	\gdef\@doiabbr{futurephys}
	\gdef\@ISSN{2624-6503}
	\gdef\@societyowner{}
}
\DeclareOption{futuretransp}{%
	\gdef\@journal{futuretransp}
	\gdef\@journalfull{Future Transportation}
	\gdef\@journalshort{Future Transp.}
	\gdef\@doiabbr{futuretransp}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{galaxies}{%
	\gdef\@journal{galaxies}
	\gdef\@journalfull{Galaxies}
	\gdef\@journalshort{Galaxies}
	\gdef\@doiabbr{galaxies}
	\gdef\@ISSN{2075-4434}
	\gdef\@societyowner{}
}
\DeclareOption{games}{%
	\gdef\@journal{games}
	\gdef\@journalfull{Games}
	\gdef\@journalshort{Games}
	\gdef\@doiabbr{g}
	\gdef\@ISSN{2073-4336}
	\gdef\@societyowner{}
}
\DeclareOption{gases}{%
	\gdef\@journal{gases}
	\gdef\@journalfull{Gases}
	\gdef\@journalshort{Gases}
	\gdef\@doiabbr{gases}
	\gdef\@ISSN{2673-5628}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{gastroent}{%
	\gdef\@journal{gastroent}
	\gdef\@journalfull{Gastroenterology Insights}
	\gdef\@journalshort{Gastroenterol. Insights}
	\gdef\@doiabbr{gastroent}
	\gdef\@ISSN{2036-7422}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{gastrointestdisord}{%
	\gdef\@journal{gastrointestdisord}
	\gdef\@journalfull{Gastrointestinal Disorders}
	\gdef\@journalshort{Gastrointest. Disord.}
	\gdef\@doiabbr{gidisord}
	\gdef\@ISSN{2624-5647}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{gastronomy}{%
	\gdef\@journal{gastronomy}
	\gdef\@journalfull{Gastronomy}
	\gdef\@journalshort{Gastronomy}
	\gdef\@doiabbr{gastronomy}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{gels}{%
	\gdef\@journal{gels}
	\gdef\@journalfull{Gels}
	\gdef\@journalshort{Gels}
	\gdef\@doiabbr{gels}
	\gdef\@ISSN{2310-2861}
	\gdef\@societyowner{}
}
\DeclareOption{genealogy}{%
	\gdef\@journal{genealogy}
	\gdef\@journalfull{Genealogy}
	\gdef\@journalshort{Genealogy}
	\gdef\@doiabbr{genealogy}
	\gdef\@ISSN{2313-5778}
	\gdef\@societyowner{}
}
\DeclareOption{genes}{%
	\gdef\@journal{genes}
	\gdef\@journalfull{Genes}
	\gdef\@journalshort{Genes}
	\gdef\@doiabbr{genes}
	\gdef\@ISSN{2073-4425}
	\gdef\@societyowner{}
}
\DeclareOption{geographies}{%
	\gdef\@journal{geographies}
	\gdef\@journalfull{Geographies}
	\gdef\@journalshort{Geographies}
	\gdef\@doiabbr{geographies}
	\gdef\@ISSN{2673-7086}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{geohazards}{%
	\gdef\@journal{geohazards}
	\gdef\@journalfull{GeoHazards}
	\gdef\@journalshort{GeoHazards}
	\gdef\@doiabbr{geohazards}
	\gdef\@ISSN{2624-795X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{geomatics}{%
	\gdef\@journal{geomatics}
	\gdef\@journalfull{Geomatics}
	\gdef\@journalshort{Geomatics}
	\gdef\@doiabbr{geomatics}
	\gdef\@ISSN{2673-7418}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{geometry}{%
	\gdef\@journal{geometry}
	\gdef\@journalfull{Geometry}
	\gdef\@journalshort{Geometry}
	\gdef\@doiabbr{geometry}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{geosciences}{%
	\gdef\@journal{geosciences}
	\gdef\@journalfull{Geosciences}
	\gdef\@journalshort{Geosciences}
	\gdef\@doiabbr{geosciences}
	\gdef\@ISSN{2076-3263}
	\gdef\@societyowner{}
}
\DeclareOption{geotechnics}{%
	\gdef\@journal{geotechnics}
	\gdef\@journalfull{Geotechnics}
	\gdef\@journalshort{Geotechnics}
	\gdef\@doiabbr{geotechnics}
	\gdef\@ISSN{2673-7094}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{geriatrics}{%
	\gdef\@journal{geriatrics}
	\gdef\@journalfull{Geriatrics}
	\gdef\@journalshort{Geriatrics}
	\gdef\@doiabbr{geriatrics}
	\gdef\@ISSN{2308-3417}
	\gdef\@societyowner{}
}
\DeclareOption{glacies}{%
	\gdef\@journal{glacies}
	\gdef\@journalfull{Glacies}
	\gdef\@journalshort{Glacies}
	\gdef\@doiabbr{glacies}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{grasses}{%
	\gdef\@journal{grasses}
	\gdef\@journalfull{Grasses}
	\gdef\@journalshort{Grasses}
	\gdef\@doiabbr{grasses}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{gucdd}{%
	\gdef\@journal{gucdd}
	\gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}
	\gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}
	\gdef\@doiabbr{gucdd}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{Gout, Hyperuricemia and Crystal Associated Disease Network}
}
\DeclareOption{hardware}{%
	\gdef\@journal{hardware}
	\gdef\@journalfull{Hardware}
	\gdef\@journalshort{Hardware}
	\gdef\@doiabbr{hardware}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{hazardousmatters}{%
	\gdef\@journal{hazardousmatters}
	\gdef\@journalfull{Hazardous Matters}
	\gdef\@journalshort{Hazard. Matters}
	\gdef\@doiabbr{}
	\gdef\@ISSN{0014-0014}
	\gdef\@societyowner{}
}
\DeclareOption{healthcare}{%
	\gdef\@journal{healthcare}
	\gdef\@journalfull{Healthcare}
	\gdef\@journalshort{Healthcare}
	\gdef\@doiabbr{healthcare}
	\gdef\@ISSN{2227-9032}
	\gdef\@societyowner{}
}
\DeclareOption{hearts}{%
	\gdef\@journal{hearts}
	\gdef\@journalfull{Hearts}
	\gdef\@journalshort{Hearts}
	\gdef\@doiabbr{hearts}
	\gdef\@ISSN{2673-3846}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{hemato}{%
	\gdef\@journal{hemato}
	\gdef\@journalfull{Hemato}
	\gdef\@journalshort{Hemato}
	\gdef\@doiabbr{hemato}
	\gdef\@ISSN{2673-6357}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{hematolrep}{%
	\gdef\@journal{hematolrep}
	\gdef\@journalfull{Hematology Reports}
	\gdef\@journalshort{Hematol. Rep.}
	\gdef\@doiabbr{hematolrep}
	\gdef\@ISSN{2038-8330}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{heritage}{%
	\gdef\@journal{heritage}
	\gdef\@journalfull{Heritage}
	\gdef\@journalshort{Heritage}
	\gdef\@doiabbr{heritage}
	\gdef\@ISSN{2571-9408}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{higheredu}{%
	\gdef\@journal{higheredu}
	\gdef\@journalfull{Trends in Higher Education}
	\gdef\@journalshort{Trends High. Educ.}
	\gdef\@doiabbr{higheredu}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{highthroughput}{%
	\gdef\@journal{highthroughput}
	\gdef\@journalfull{High-Throughput}
	\gdef\@journalshort{High-Throughput}
	\gdef\@doiabbr{ht}
	\gdef\@ISSN{2571-5135}
	\gdef\@societyowner{}
}
\DeclareOption{histories}{%
	\gdef\@journal{histories}
	\gdef\@journalfull{Histories}
	\gdef\@journalshort{Histories}
	\gdef\@doiabbr{histories}
	\gdef\@ISSN{2409-9252}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{horticulturae}{%
	\gdef\@journal{horticulturae}
	\gdef\@journalfull{Horticulturae}
	\gdef\@journalshort{Horticulturae}
	\gdef\@doiabbr{horticulturae}
	\gdef\@ISSN{2311-7524}
	\gdef\@societyowner{}
}
\DeclareOption{hospitals}{%
	\gdef\@journal{hospitals}
	\gdef\@journalfull{Hospitals}
	\gdef\@journalshort{Hospitals}
	\gdef\@doiabbr{hospitals}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{humanities}{%
	\gdef\@journal{humanities}
	\gdef\@journalfull{Humanities}
	\gdef\@journalshort{Humanities}
	\gdef\@doiabbr{h}
	\gdef\@ISSN{2076-0787}
	\gdef\@societyowner{}
}
\DeclareOption{humans}{%
	\gdef\@journal{humans}
	\gdef\@journalfull{Humans}
	\gdef\@journalshort{Humans}
	\gdef\@doiabbr{humans}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{hydrobiology}{%
	\gdef\@journal{hydrobiology}
	\gdef\@journalfull{Hydrobiology}
	\gdef\@journalshort{Hydrobiology}
	\gdef\@doiabbr{hydrobiology}
	\gdef\@ISSN{2673-9917}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{hydrogen}{%
	\gdef\@journal{hydrogen}
	\gdef\@journalfull{Hydrogen}
	\gdef\@journalshort{Hydrogen}
	\gdef\@doiabbr{hydrogen}
	\gdef\@ISSN{2673-4141}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{hydrology}{%
	\gdef\@journal{hydrology}
	\gdef\@journalfull{Hydrology}
	\gdef\@journalshort{Hydrology}
	\gdef\@doiabbr{hydrology}
	\gdef\@ISSN{2306-5338}
	\gdef\@societyowner{}
}
\DeclareOption{hygiene}{%
	\gdef\@journal{hygiene}
	\gdef\@journalfull{Hygiene}
	\gdef\@journalshort{Hygiene}
	\gdef\@doiabbr{hygiene}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{idr}{%
	\gdef\@journal{idr}
	\gdef\@journalfull{Infectious Disease Reports}
	\gdef\@journalshort{Infect. Dis. Rep.}
	\gdef\@doiabbr{idr}
	\gdef\@ISSN{2036-7449}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{iic}{%
	\gdef\@journal{iic}
	\gdef\@journalfull{Intelligent Infrastructure and Construction}
	\gdef\@journalshort{Intell. Infrastruct. Constr.}
	\gdef\@doiabbr{iic}
	\gdef\@ISSN{3042-4720}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijerph}{%
	\gdef\@journal{ijerph}
	\gdef\@journalfull{International Journal of Environmental Research and Public Health}
	\gdef\@journalshort{Int. J. Environ. Res. Public Health}
	\gdef\@doiabbr{ijerph}
	\gdef\@ISSN{1660-4601}
	\gdef\@societyowner{}
}
\DeclareOption{ijfs}{%
	\gdef\@journal{ijfs}
	\gdef\@journalfull{International Journal of Financial Studies}
	\gdef\@journalshort{Int. J. Financial Stud.}
	\gdef\@doiabbr{ijfs}
	\gdef\@ISSN{2227-7072}
	\gdef\@societyowner{}
}
\DeclareOption{ijgi}{%
	\gdef\@journal{ijgi}
	\gdef\@journalfull{ISPRS International Journal of Geo-Information}
	\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}
	\gdef\@doiabbr{ijgi}
	\gdef\@ISSN{2220-9964}
	\gdef\@societyowner{International Society for Photogrammetry and Remote Sensing}
}
\DeclareOption{ijmd}{%
	\gdef\@journal{ijmd}
	\gdef\@journalfull{International Journal of Medical Devices}
	\gdef\@journalshort{Int. J. Med. Devices}
	\gdef\@doiabbr{ijmd}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijms}{%
	\gdef\@journal{ijms}
	\gdef\@journalfull{International Journal of Molecular Sciences}
	\gdef\@journalshort{Int. J. Mol. Sci.}
	\gdef\@doiabbr{ijms}
	\gdef\@ISSN{1422-0067}
	\gdef\@societyowner{}
}
\DeclareOption{ijns}{%
	\gdef\@journal{ijns}
	\gdef\@journalfull{International Journal of Neonatal Screening}
	\gdef\@journalshort{Int. J. Neonatal Screen.}
	\gdef\@doiabbr{ijns}
	\gdef\@ISSN{2409-515X}
	\gdef\@societyowner{International Society for Neonatal Screening}
}
\DeclareOption{ijpb}{%
	\gdef\@journal{ijpb}
	\gdef\@journalfull{International Journal of Plant Biology}
	\gdef\@journalshort{Int. J. Plant Biol.}
	\gdef\@doiabbr{ijpb}
	\gdef\@ISSN{2037-0164}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijt}{%
	\gdef\@journal{ijt}
	\gdef\@journalfull{International Journal of Topology}
	\gdef\@journalshort{Int. J. Topol.}
	\gdef\@doiabbr{ijt}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijtm}{%
	\gdef\@journal{ijtm}
	\gdef\@journalfull{International Journal of Translational Medicine}
	\gdef\@journalshort{Int. J. Transl. Med.}
	\gdef\@doiabbr{ijtm}
	\gdef\@ISSN{2673-8937}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijtpp}{%
	\gdef\@journal{ijtpp}
	\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}
	\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}
	\gdef\@doiabbr{ijtpp}
	\gdef\@ISSN{2504-186X}
	\gdef\@societyowner{EUROTURBO European turbomachinery society}
}
\DeclareOption{ime}{%
	\gdef\@journal{ime}
	\gdef\@journalfull{International Medical Education}
	\gdef\@journalshort{Int. Med. Educ.}
	\gdef\@doiabbr{ime}
	\gdef\@ISSN{2813-141X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{Academic Society for International Medical Education}
}
\DeclareOption{immuno}{%
	\gdef\@journal{immuno}
	\gdef\@journalfull{Immuno}
	\gdef\@journalshort{Immuno}
	\gdef\@doiabbr{immuno}
	\gdef\@ISSN{2673-5601}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{informatics}{%
	\gdef\@journal{informatics}
	\gdef\@journalfull{Informatics}
	\gdef\@journalshort{Informatics}
	\gdef\@doiabbr{informatics}
	\gdef\@ISSN{2227-9709}
	\gdef\@societyowner{}
}
\DeclareOption{information}{%
	\gdef\@journal{information}
	\gdef\@journalfull{Information}
	\gdef\@journalshort{Information}
	\gdef\@doiabbr{info}
	\gdef\@ISSN{2078-2489}
	\gdef\@societyowner{}
}
\DeclareOption{infrastructures}{%
	\gdef\@journal{infrastructures}
	\gdef\@journalfull{Infrastructures}
	\gdef\@journalshort{Infrastructures}
	\gdef\@doiabbr{infrastructures}
	\gdef\@ISSN{2412-3811}
	\gdef\@societyowner{}
}
\DeclareOption{inorganics}{%
	\gdef\@journal{inorganics}
	\gdef\@journalfull{Inorganics}
	\gdef\@journalshort{Inorganics}
	\gdef\@doiabbr{inorganics}
	\gdef\@ISSN{2304-6740}
	\gdef\@societyowner{}
}
\DeclareOption{insects}{%
	\gdef\@journal{insects}
	\gdef\@journalfull{Insects}
	\gdef\@journalshort{Insects}
	\gdef\@doiabbr{insects}
	\gdef\@ISSN{2075-4450}
	\gdef\@societyowner{}
}
\DeclareOption{instruments}{%
	\gdef\@journal{instruments}
	\gdef\@journalfull{Instruments}
	\gdef\@journalshort{Instruments}
	\gdef\@doiabbr{instruments}
	\gdef\@ISSN{2410-390X}
	\gdef\@societyowner{}
}
\DeclareOption{inventions}{%
	\gdef\@journal{inventions}
	\gdef\@journalfull{Inventions}
	\gdef\@journalshort{Inventions}
	\gdef\@doiabbr{inventions}
	\gdef\@ISSN{2411-5134}
	\gdef\@societyowner{}
}
\DeclareOption{iot}{%
	\gdef\@journal{iot}
	\gdef\@journalfull{IoT}
	\gdef\@journalshort{IoT}
	\gdef\@doiabbr{iot}
	\gdef\@ISSN{2624-831X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{j}{%
	\gdef\@journal{j}
	\gdef\@journalfull{J}
	\gdef\@journalshort{J}
	\gdef\@doiabbr{j}
	\gdef\@ISSN{2571-8800}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jal}{%
	\gdef\@journal{jal}
	\gdef\@journalfull{Journal of Ageing and Longevity}
	\gdef\@journalshort{J. Ageing Longev.}
	\gdef\@doiabbr{jal}
	\gdef\@ISSN{2673-9259}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jcdd}{%
	\gdef\@journal{jcdd}
	\gdef\@journalfull{Journal of Cardiovascular Development and Disease}
	\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}
	\gdef\@doiabbr{jcdd}
	\gdef\@ISSN{2308-3425}
	\gdef\@societyowner{}
}
\DeclareOption{jcm}{%
	\gdef\@journal{jcm}
	\gdef\@journalfull{Journal of Clinical Medicine}
	\gdef\@journalshort{J. Clin. Med.}
	\gdef\@doiabbr{jcm}
	\gdef\@ISSN{2077-0383}
	\gdef\@societyowner{}
}
\DeclareOption{jcp}{%
	\gdef\@journal{jcp}
	\gdef\@journalfull{Journal of Cybersecurity and Privacy}
	\gdef\@journalshort{J. Cybersecur. Priv.}
	\gdef\@doiabbr{jcp}
	\gdef\@ISSN{2624-800X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jcs}{%
	\gdef\@journal{jcs}
	\gdef\@journalfull{Journal of Composites Science}
	\gdef\@journalshort{J. Compos. Sci.}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2504-477X}
	\gdef\@societyowner{}
}
\DeclareOption{jcto}{%
	\gdef\@journal{jcto}
	\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}
	\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}
	\gdef\@doiabbr{jcto}
	\gdef\@ISSN{2813-1053}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jdad}{%
	\gdef\@journal{jdad}
	\gdef\@journalfull{Journal of Dementia and Alzheimer’s Disease}
	\gdef\@journalshort{J. Dement. Alzheimer's Dis.}
	\gdef\@doiabbr{jdad}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jdb}{%
	\gdef\@journal{jdb}
	\gdef\@journalfull{Journal of Developmental Biology}
	\gdef\@journalshort{J. Dev. Biol.}
	\gdef\@doiabbr{jdb}
	\gdef\@ISSN{2221-3759}
	\gdef\@societyowner{}
}
\DeclareOption{jeta}{%
	\gdef\@journal{jeta}
	\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}
	\gdef\@journalshort{J. Exp. Theor. Anal.}
	\gdef\@doiabbr{jeta}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jfb}{%
	\gdef\@journal{jfb}
	\gdef\@journalfull{Journal of Functional Biomaterials}
	\gdef\@journalshort{J. Funct. Biomater.}
	\gdef\@doiabbr{jfb}
	\gdef\@ISSN{2079-4983}
	\gdef\@societyowner{}
}
\DeclareOption{jfmk}{%
	\gdef\@journal{jfmk}
	\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}
	\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}
	\gdef\@doiabbr{jfmk}
	\gdef\@ISSN{2411-5142}
	\gdef\@societyowner{}
}
\DeclareOption{jimaging}{%
	\gdef\@journal{jimaging}
	\gdef\@journalfull{Journal of Imaging}
	\gdef\@journalshort{J. Imaging}
	\gdef\@doiabbr{jimaging}
	\gdef\@ISSN{2313-433X}
	\gdef\@societyowner{}
}
\DeclareOption{jintelligence}{%
	\gdef\@journal{jintelligence}
	\gdef\@journalfull{Journal of Intelligence}
	\gdef\@journalshort{J. Intell.}
	\gdef\@doiabbr{jintelligence}
	\gdef\@ISSN{2079-3200}
	\gdef\@societyowner{}
}
\DeclareOption{jlpea}{%
	\gdef\@journal{jlpea}
	\gdef\@journalfull{Journal of Low Power Electronics and Applications}
	\gdef\@journalshort{J. Low Power Electron. Appl.}
	\gdef\@doiabbr{jlpea}
	\gdef\@ISSN{2079-9268}
	\gdef\@societyowner{}
}
\DeclareOption{jmahp}{%
	\gdef\@journal{jmahp}
	\gdef\@journalfull{Journal of Market Access \& Health Policy}
	\gdef\@journalshort{J. Mark. Access Health Policy}
	\gdef\@doiabbr{jmahp}
	\gdef\@ISSN{2001-6689}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{Market Access Society}
}
\DeclareOption{jmmp}{%
	\gdef\@journal{jmmp}
	\gdef\@journalfull{Journal of Manufacturing and Materials Processing}
	\gdef\@journalshort{J. Manuf. Mater. Process.}
	\gdef\@doiabbr{jmmp}
	\gdef\@ISSN{2504-4494}
	\gdef\@societyowner{}
}
\DeclareOption{jmp}{%
	\gdef\@journal{jmp}
	\gdef\@journalfull{Journal of Molecular Pathology}
	\gdef\@journalshort{J. Mol. Pathol.}
	\gdef\@doiabbr{jmp}
	\gdef\@ISSN{2673-5261}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jmse}{%
	\gdef\@journal{jmse}
	\gdef\@journalfull{Journal of Marine Science and Engineering}
	\gdef\@journalshort{J. Mar. Sci. Eng.}
	\gdef\@doiabbr{jmse}
	\gdef\@ISSN{2077-1312}
	\gdef\@societyowner{}
}
\DeclareOption{jne}{%
	\gdef\@journal{jne}
	\gdef\@journalfull{Journal of Nuclear Engineering}
	\gdef\@journalshort{J. Nucl. Eng.}
	\gdef\@doiabbr{jne}
	\gdef\@ISSN{2673-4362}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jnt}{%
	\gdef\@journal{jnt}
	\gdef\@journalfull{Journal of Nanotheranostics}
	\gdef\@journalshort{J. Nanotheranostics}
	\gdef\@doiabbr{jnt}
	\gdef\@ISSN{2624-845X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
} 
\DeclareOption{jof}{%
	\gdef\@journal{jof}
	\gdef\@journalfull{Journal of Fungi}
	\gdef\@journalshort{J. Fungi}
	\gdef\@doiabbr{jof}
	\gdef\@ISSN{2309-608X}
	\gdef\@societyowner{}
}
\DeclareOption{joitmc}{%
	\gdef\@journal{joitmc}
	\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}
	\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}
	\gdef\@doiabbr{joitmc}
	\gdef\@ISSN{2199-8531}
	\gdef\@societyowner{}
}
\DeclareOption{joma}{%
	\gdef\@journal{joma}
	\gdef\@journalfull{Journal of the Oman Medical Association}
	\gdef\@journalshort{J. Oman Med. Assoc.}
	\gdef\@doiabbr{joma}
	\gdef\@ISSN{2813-8759}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{Oman Medical Association}
}
\DeclareOption{jor}{%
	\gdef\@journal{jor}
	\gdef\@journalfull{Journal of Respiration}
	\gdef\@journalshort{J. Respir.}
	\gdef\@doiabbr{jor}
	\gdef\@ISSN{2673-527X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{journalmedia}{%
	\gdef\@journal{journalmedia}
	\gdef\@journalfull{Journalism and Media}
	\gdef\@journalshort{Journal. Media}
	\gdef\@doiabbr{journalmedia}
	\gdef\@ISSN{2673-5172}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jox}{%
	\gdef\@journal{jox}
	\gdef\@journalfull{Journal of Xenobiotics}
	\gdef\@journalshort{J. Xenobiot.}
	\gdef\@doiabbr{jox}
	\gdef\@ISSN{2039-4713}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jpbi}{%
	\gdef\@journal{jpbi}
	\gdef\@journalfull{Journal of Pharmaceutical and BioTech Industry}
	\gdef\@journalshort{J. Pharm. BioTech Ind.}
	\gdef\@doiabbr{jpbi}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jpm}{%
	\gdef\@journal{jpm}
	\gdef\@journalfull{Journal of Personalized Medicine}
	\gdef\@journalshort{J. Pers. Med.}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{2075-4426}
	\gdef\@societyowner{}
}
\DeclareOption{jrfm}{%
	\gdef\@journal{jrfm}
	\gdef\@journalfull{Journal of Risk and Financial Management}
	\gdef\@journalshort{J. Risk Financial Manag.}
	\gdef\@doiabbr{jrfm}
	\gdef\@ISSN{1911-8074}
	\gdef\@societyowner{}
}
\DeclareOption{jsan}{%
	\gdef\@journal{jsan}
	\gdef\@journalfull{Journal of Sensor and Actuator Networks}
	\gdef\@journalshort{J. Sens. Actuator Netw.}
	\gdef\@doiabbr{jsan}
	\gdef\@ISSN{2224-2708}
	\gdef\@societyowner{}
}
\DeclareOption{jtaer}{%
	\gdef\@journal{jtaer}
	\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}
	\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}
	\gdef\@doiabbr{jtaer}
	\gdef\@ISSN{0718-1876}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jvd}{%
	\gdef\@journal{jvd}
	\gdef\@journalfull{Journal of Vascular Diseases}
	\gdef\@journalshort{J. Vasc. Dis.}
	\gdef\@doiabbr{jvd}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jzbg}{%
	\gdef\@journal{jzbg}
	\gdef\@journalfull{Journal of Zoological and Botanical Gardens}
	\gdef\@journalshort{J. Zool. Bot. Gard.}
	\gdef\@doiabbr{jzbg}
	\gdef\@ISSN{2673-5636}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
%\DeclareOption{kidney}{%
%	\gdef\@journal{kidney}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{kidneydial}{%
	\gdef\@journal{kidneydial}
	\gdef\@journalfull{Kidney and Dialysis}
	\gdef\@journalshort{Kidney Dial.}
	\gdef\@doiabbr{kidneydial}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{kinasesphosphatases}{%
	\gdef\@journal{kinasesphosphatases}
	\gdef\@journalfull{Kinases and Phosphatases}
	\gdef\@journalshort{Kinases Phosphatases}
	\gdef\@doiabbr{kinasesphosphatases}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{knowledge}{%
	\gdef\@journal{knowledge}
	\gdef\@journalfull{Knowledge}
	\gdef\@journalshort{Knowledge}
	\gdef\@doiabbr{knowledge}
	\gdef\@ISSN{2673-9585}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{labmed}{%
	\gdef\@journal{labmed}
	\gdef\@journalfull{LabMed}
	\gdef\@journalshort{LabMed}
	\gdef\@doiabbr{labmed}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{laboratories}{%
	\gdef\@journal{laboratories}
	\gdef\@journalfull{Laboratories}
	\gdef\@journalshort{Laboratories}
	\gdef\@doiabbr{laboratories}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{land}{%
	\gdef\@journal{land}
	\gdef\@journalfull{Land}
	\gdef\@journalshort{Land}
	\gdef\@doiabbr{land}
	\gdef\@ISSN{2073-445X}
	\gdef\@societyowner{}
}
\DeclareOption{languages}{%
	\gdef\@journal{languages}
	\gdef\@journalfull{Languages}
	\gdef\@journalshort{Languages}
	\gdef\@doiabbr{languages}
	\gdef\@ISSN{2226-471X}
	\gdef\@societyowner{}
}
\DeclareOption{laws}{%
	\gdef\@journal{laws}
	\gdef\@journalfull{Laws}
	\gdef\@journalshort{Laws}
	\gdef\@doiabbr{laws}
	\gdef\@ISSN{2075-471X}
	\gdef\@societyowner{}
}
\DeclareOption{life}{%
	\gdef\@journal{life}
	\gdef\@journalfull{Life}
	\gdef\@journalshort{Life}
	\gdef\@doiabbr{life}
	\gdef\@ISSN{2075-1729}
	\gdef\@societyowner{}
}
\DeclareOption{lights}{%
	\gdef\@journal{lights}
	\gdef\@journalfull{Lights}
	\gdef\@journalshort{Lights}
	\gdef\@doiabbr{lights}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{limnolrev}{%
	\gdef\@journal{limnolrev}
	\gdef\@journalfull{Limnological Review}
	\gdef\@journalshort{Limnol. Rev.}
	\gdef\@doiabbr{limnolrev}
	\gdef\@ISSN{2300-7575}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{lipidology}{%
	\gdef\@journal{lipidology}
	\gdef\@journalfull{Lipidology}
	\gdef\@journalshort{Lipidology}
	\gdef\@doiabbr{lipidology}
	\gdef\@ISSN{2813-7086}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{liquids}{%
	\gdef\@journal{liquids}
	\gdef\@journalfull{Liquids}
	\gdef\@journalshort{Liquids}
	\gdef\@doiabbr{liquids}
	\gdef\@ISSN{2673-8015}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{literature}{%
	\gdef\@journal{literature}
	\gdef\@journalfull{Literature}
	\gdef\@journalshort{Literature}
	\gdef\@doiabbr{literature}
	\gdef\@ISSN{2410-9789}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{livers}{%
	\gdef\@journal{livers}
	\gdef\@journalfull{Livers}
	\gdef\@journalshort{Livers}
	\gdef\@doiabbr{livers}
	\gdef\@ISSN{2673-4389}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{logics}{%
	\gdef\@journal{logics}
	\gdef\@journalfull{Logics}
	\gdef\@journalshort{Logics}
	\gdef\@doiabbr{logics}
	\gdef\@ISSN{2813-0405}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{logistics}{%
	\gdef\@journal{logistics}
	\gdef\@journalfull{Logistics}
	\gdef\@journalshort{Logistics}
	\gdef\@doiabbr{logistics}
	\gdef\@ISSN{2305-6290}
	\gdef\@societyowner{}
}
\DeclareOption{lubricants}{%
	\gdef\@journal{lubricants}
	\gdef\@journalfull{Lubricants}
	\gdef\@journalshort{Lubricants}
	\gdef\@doiabbr{lubricants}
	\gdef\@ISSN{2075-4442}
	\gdef\@societyowner{}
}
\DeclareOption{lymphatics}{%
	\gdef\@journal{lymphatics}
	\gdef\@journalfull{Lymphatics}
	\gdef\@journalshort{Lymphatics}
	\gdef\@doiabbr{lymphatics}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{machines}{%
	\gdef\@journal{machines}
	\gdef\@journalfull{Machines}
	\gdef\@journalshort{Machines}
	\gdef\@doiabbr{machines}
	\gdef\@ISSN{2075-1702}
	\gdef\@societyowner{}
}
\DeclareOption{macromol}{%
	\gdef\@journal{macromol}
	\gdef\@journalfull{Macromol}
	\gdef\@journalshort{Macromol}
	\gdef\@doiabbr{macromol}
	\gdef\@ISSN{2673-6209}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{magnetism}{%
	\gdef\@journal{magnetism}
	\gdef\@journalfull{Magnetism}
	\gdef\@journalshort{Magnetism}
	\gdef\@doiabbr{magnetism}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{magnetochemistry}{%
	\gdef\@journal{magnetochemistry}
	\gdef\@journalfull{Magnetochemistry}
	\gdef\@journalshort{Magnetochemistry}
	\gdef\@doiabbr{magnetochemistry}
	\gdef\@ISSN{2312-7481}
	\gdef\@societyowner{}
}
\DeclareOption{make}{%
	\gdef\@journal{make}
	\gdef\@journalfull{Machine Learning and Knowledge Extraction}
	\gdef\@journalshort{Mach. Learn. Knowl. Extr.}
	\gdef\@doiabbr{make}
	\gdef\@ISSN{2504-4990}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{marinedrugs}{%
	\gdef\@journal{marinedrugs}
	\gdef\@journalfull{Marine Drugs}
	\gdef\@journalshort{Mar. Drugs}
	\gdef\@doiabbr{md}
	\gdef\@ISSN{1660-3397}
	\gdef\@societyowner{}
}
\DeclareOption{materials}{%
	\gdef\@journal{materials}
	\gdef\@journalfull{Materials}
	\gdef\@journalshort{Materials}
	\gdef\@doiabbr{ma}
	\gdef\@ISSN{1996-1944}
	\gdef\@societyowner{}
}
\DeclareOption{materproc}{%
	\gdef\@journal{materproc}
	\gdef\@journalfull{Materials Proceedings}
	\gdef\@journalshort{Mater. Proc.}
	\gdef\@doiabbr{materproc}
	\gdef\@ISSN{2673-4605}
	\gdef\@societyowner{}
}
\DeclareOption{mathematics}{%
	\gdef\@journal{mathematics}
	\gdef\@journalfull{Mathematics}
	\gdef\@journalshort{Mathematics}
	\gdef\@doiabbr{math}
	\gdef\@ISSN{2227-7390}
	\gdef\@societyowner{}
}
\DeclareOption{mca}{%
	\gdef\@journal{mca}
	\gdef\@journalfull{Mathematical and Computational Applications}
	\gdef\@journalshort{Math. Comput. Appl.}
	\gdef\@doiabbr{mca}
	\gdef\@ISSN{2297-8747}
	\gdef\@societyowner{}
}
\DeclareOption{measurements}{%
	\gdef\@journal{measurements}
	\gdef\@journalfull{Measurements}
	\gdef\@journalshort{Measurements}
	\gdef\@doiabbr{measurements}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{medicina}{%
	\gdef\@journal{medicina}
	\gdef\@journalfull{Medicina}
	\gdef\@journalshort{Medicina}
	\gdef\@doiabbr{medicina}
	\gdef\@ISSN{1648-9144}
	\gdef\@societyowner{Lithuanian University of Health Sciences}
}
\DeclareOption{medicines}{%
	\gdef\@journal{medicines}
	\gdef\@journalfull{Medicines}
	\gdef\@journalshort{Medicines}
	\gdef\@doiabbr{medicines}
	\gdef\@ISSN{2305-6320}
	\gdef\@societyowner{}
}
\DeclareOption{medsci}{%
	\gdef\@journal{medsci}
	\gdef\@journalfull{Medical Sciences}
	\gdef\@journalshort{Med. Sci.}
	\gdef\@doiabbr{medsci}
	\gdef\@ISSN{2076-3271}
	\gdef\@societyowner{}
}
\DeclareOption{membranes}{%
	\gdef\@journal{membranes}
	\gdef\@journalfull{Membranes}
	\gdef\@journalshort{Membranes}
	\gdef\@doiabbr{membranes}
	\gdef\@ISSN{2077-0375}
	\gdef\@societyowner{}
}
\DeclareOption{merits}{%
	\gdef\@journal{merits}
	\gdef\@journalfull{Merits}
	\gdef\@journalshort{Merits}
	\gdef\@doiabbr{merits}
	\gdef\@ISSN{2673-8104}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{metabolites}{%
	\gdef\@journal{metabolites}
	\gdef\@journalfull{Metabolites}
	\gdef\@journalshort{Metabolites}
	\gdef\@doiabbr{metabo}
	\gdef\@ISSN{2218-1989}
	\gdef\@societyowner{}
}
\DeclareOption{metals}{%
	\gdef\@journal{metals}
	\gdef\@journalfull{Metals}
	\gdef\@journalshort{Metals}
	\gdef\@doiabbr{met}
	\gdef\@ISSN{2075-4701}
	\gdef\@societyowner{}
}
\DeclareOption{meteorology}{%
	\gdef\@journal{meteorology}
	\gdef\@journalfull{Meteorology}
	\gdef\@journalshort{Meteorology}
	\gdef\@doiabbr{meteorology}
	\gdef\@ISSN{2674-0494}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{methane}{%
	\gdef\@journal{methane}
	\gdef\@journalfull{Methane}
	\gdef\@journalshort{Methane}
	\gdef\@doiabbr{methane}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{metrics}{%
	\gdef\@journal{metrics}
	\gdef\@journalfull{Metrics}
	\gdef\@journalshort{Metrics}
	\gdef\@doiabbr{metrics}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{metrology}{%
	\gdef\@journal{metrology}
	\gdef\@journalfull{Metrology}
	\gdef\@journalshort{Metrology}
	\gdef\@doiabbr{metrology}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{micro}{%
	\gdef\@journal{micro}
	\gdef\@journalfull{Micro}
	\gdef\@journalshort{Micro}
	\gdef\@doiabbr{micro}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{microarrays}{%
	\gdef\@journal{microarrays}
	\gdef\@journalfull{Microarrays}
	\gdef\@journalshort{Microarrays}
	\gdef\@doiabbr{microarrays}
	\gdef\@ISSN{2076-3905}
	\gdef\@societyowner{}
}
\DeclareOption{microbiolres}{%
	\gdef\@journal{microbiolres}
	\gdef\@journalfull{Microbiology Research}
	\gdef\@journalshort{Microbiol. Res.}
	\gdef\@doiabbr{microbiolres}
	\gdef\@ISSN{2036-7481}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{microelectronics}{%
       \gdef\@journal{microelectronics}
       \gdef\@journalfull{Microelectronics}
       \gdef\@journalshort{Microelectronics}
       \gdef\@doiabbr{microelectronics}
       \gdef\@ISSN{}
       \gdef\@continuouspages{yes}
       \gdef\@societyowner{}
}
\DeclareOption{micromachines}{%
	\gdef\@journal{micromachines}
	\gdef\@journalfull{Micromachines}
	\gdef\@journalshort{Micromachines}
	\gdef\@doiabbr{mi}
	\gdef\@ISSN{2072-666X}
	\gdef\@societyowner{}
}
\DeclareOption{microorganisms}{%
	\gdef\@journal{microorganisms}
	\gdef\@journalfull{Microorganisms}
	\gdef\@journalshort{Microorganisms}
	\gdef\@doiabbr{microorganisms}
	\gdef\@ISSN{2076-2607}
	\gdef\@societyowner{}
}
\DeclareOption{microplastics}{%
	\gdef\@journal{microplastics}
	\gdef\@journalfull{Microplastics}
	\gdef\@journalshort{Microplastics}
	\gdef\@doiabbr{microplastics}
	\gdef\@ISSN{2673-8929}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{microwave}{%
	\gdef\@journal{microwave}
	\gdef\@journalfull{Microwave}
	\gdef\@journalshort{Microwave}
	\gdef\@doiabbr{microwave}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{minerals}{%
	\gdef\@journal{minerals}
	\gdef\@journalfull{Minerals}
	\gdef\@journalshort{Minerals}
	\gdef\@doiabbr{min}
	\gdef\@ISSN{2075-163X}
	\gdef\@societyowner{}
}
\DeclareOption{mining}{%
	\gdef\@journal{mining}
	\gdef\@journalfull{Mining}
	\gdef\@journalshort{Mining}
	\gdef\@doiabbr{mining}
	\gdef\@ISSN{2673-6489}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{mmphys}{%
        \gdef\@journal{mmphys}
        \gdef\@journalfull{Modern Mathematical Physics}
        \gdef\@journalshort{Mod. Math. Phys.}
        \gdef\@doiabbr{mmphys}\gdef\@ISSN{3042-5034}
        \gdef\@continuouspages{yes}
       \gdef\@societyowner{}
}
\DeclareOption{modelling}{%
	\gdef\@journal{modelling}
	\gdef\@journalfull{Modelling}
	\gdef\@journalshort{Modelling}
	\gdef\@doiabbr{modelling}
	\gdef\@ISSN{2673-3951}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{molbank}{%
	\gdef\@journal{molbank}
	\gdef\@journalfull{Molbank}
	\gdef\@journalshort{Molbank}
	\gdef\@doiabbr{M}
	\gdef\@ISSN{1422-8599}
	\gdef\@societyowner{}
}
\DeclareOption{molecules}{%
	\gdef\@journal{molecules}
	\gdef\@journalfull{Molecules}
	\gdef\@journalshort{Molecules}
	\gdef\@doiabbr{molecules}
	\gdef\@ISSN{1420-3049}
	\gdef\@societyowner{}
}
\DeclareOption{mps}{%
	\gdef\@journal{mps}
	\gdef\@journalfull{Methods and Protocols}
	\gdef\@journalshort{Methods Protoc.}
	\gdef\@doiabbr{mps}
	\gdef\@ISSN{2409-9279}
	\gdef\@societyowner{}
}
\DeclareOption{msf}{%
	\gdef\@journal{msf}
	\gdef\@journalfull{Medical Sciences Forum}
	\gdef\@journalshort{Med. Sci. Forum}
	\gdef\@doiabbr{msf}
	\gdef\@ISSN{2673-9992}
	\gdef\@societyowner{}
}
\DeclareOption{mti}{%
	\gdef\@journal{mti}
	\gdef\@journalfull{Multimodal Technologies and Interaction}
	\gdef\@journalshort{Multimodal Technol. Interact.}
	\gdef\@doiabbr{mti}
	\gdef\@ISSN{2414-4088}
	\gdef\@societyowner{}
}
\DeclareOption{multimedia}{%
       \gdef\@journal{multimedia}
       \gdef\@journalfull{Multimedia}
       \gdef\@journalshort{Multimedia}
       \gdef\@doiabbr{multimedia}
       \gdef\@ISSN{}
       \gdef\@continuouspages{yes}
       \gdef\@societyowner{}
}
\DeclareOption{muscles}{%
	\gdef\@journal{muscles}
	\gdef\@journalfull{Muscles}
	\gdef\@journalshort{Muscles}
	\gdef\@doiabbr{muscles}
	\gdef\@ISSN{2813-0413}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{nanoenergyadv}{%
	\gdef\@journal{nanoenergyadv}
	\gdef\@journalfull{Nanoenergy Advances}
	\gdef\@journalshort{Nanoenergy Adv.}
	\gdef\@doiabbr{nanoenergyadv}
	\gdef\@ISSN{2673-706X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{nanomanufacturing}{%
	\gdef\@journal{nanomanufacturing}
	\gdef\@journalfull{Nanomanufacturing}
	\gdef\@journalshort{Nanomanufacturing}
	\gdef\@doiabbr{nanomanufacturing}
	\gdef\@ISSN{2673-687X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{nanomaterials}{%
	\gdef\@journal{nanomaterials}
	\gdef\@journalfull{Nanomaterials}
	\gdef\@journalshort{Nanomaterials}
	\gdef\@doiabbr{nano}
	\gdef\@ISSN{2079-4991}
	\gdef\@societyowner{}
}
\DeclareOption{ncrna}{%
	\gdef\@journal{ncrna}
	\gdef\@journalfull{Non-Coding RNA}
	\gdef\@journalshort{Non-Coding RNA}
	\gdef\@doiabbr{ncrna}
	\gdef\@ISSN{2311-553X}
	\gdef\@societyowner{}
}
\DeclareOption{ndt}{%
	\gdef\@journal{ndt}
	\gdef\@journalfull{NDT}
	\gdef\@journalshort{NDT}
	\gdef\@doiabbr{ndt}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{network}{%
	\gdef\@journal{network}
	\gdef\@journalfull{Network}
	\gdef\@journalshort{Network}
	\gdef\@doiabbr{network}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{neuroglia}{%
	\gdef\@journal{neuroglia}
	\gdef\@journalfull{Neuroglia}
	\gdef\@journalshort{Neuroglia}
	\gdef\@doiabbr{neuroglia}
	\gdef\@ISSN{2571-6980}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{neurolint}{%
	\gdef\@journal{neurolint}
	\gdef\@journalfull{Neurology International}
	\gdef\@journalshort{Neurol. Int.}
	\gdef\@doiabbr{neurolint}
	\gdef\@ISSN{2035-8377}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{neurosci}{%
	\gdef\@journal{neurosci}
	\gdef\@journalfull{NeuroSci}
	\gdef\@journalshort{NeuroSci}
	\gdef\@doiabbr{neurosci}
	\gdef\@ISSN{2673-4087}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{nitrogen}{%
	\gdef\@journal{nitrogen}
	\gdef\@journalfull{Nitrogen}
	\gdef\@journalshort{Nitrogen}
	\gdef\@doiabbr{nitrogen}
	\gdef\@ISSN{2504-3129}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{nri}{%
	\gdef\@journal{nri}
	\gdef\@journalfull{Natural Resources Informatics}
	\gdef\@journalshort{Nat. Resour. Inform.}
	\gdef\@doiabbr{nri}
	\gdef\@ISSN{2673-981X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{nursrep}{%
	\gdef\@journal{nursrep}
	\gdef\@journalfull{Nursing Reports}
	\gdef\@journalshort{Nurs. Rep.}
	\gdef\@doiabbr{nursrep}
	\gdef\@ISSN{2039-4403}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{nutraceuticals}{%
	\gdef\@journal{nutraceuticals}
	\gdef\@journalfull{Nutraceuticals}
	\gdef\@journalshort{Nutraceuticals}
	\gdef\@doiabbr{nutraceuticals}
	\gdef\@ISSN{1661-3821}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{nutrients}{%
	\gdef\@journal{nutrients}
	\gdef\@journalfull{Nutrients}
	\gdef\@journalshort{Nutrients}
	\gdef\@doiabbr{nu}
	\gdef\@ISSN{2072-6643}
	\gdef\@societyowner{}
}
\DeclareOption{obesities}{%
	\gdef\@journal{obesities}
	\gdef\@journalfull{Obesities}
	\gdef\@journalshort{Obesities}
	\gdef\@doiabbr{obesities}
	\gdef\@ISSN{2673-4168}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{oceans}{%
	\gdef\@journal{oceans}
	\gdef\@journalfull{Oceans}
	\gdef\@journalshort{Oceans}
	\gdef\@doiabbr{oceans}
	\gdef\@ISSN{2673-1924}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ohbm}{%
	\gdef\@journal{ohbm}
	\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}
	\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}
	\gdef\@doiabbr{ohbm}
	\gdef\@ISSN{2504-463X}
	\gdef\@societyowner{}
}
\DeclareOption{onco}{%
	\gdef\@journal{onco}
	\gdef\@journalfull{Onco}
	\gdef\@journalshort{Onco}
	\gdef\@doiabbr{onco}
	\gdef\@ISSN{2673-7523}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
%\DeclareOption{oncopathology}{%
%	\gdef\@journal{oncopathology}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{optics}{%
	\gdef\@journal{optics}
	\gdef\@journalfull{Optics}
	\gdef\@journalshort{Optics}
	\gdef\@doiabbr{opt}
	\gdef\@ISSN{2673-3269}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{oral}{%
	\gdef\@journal{oral}
	\gdef\@journalfull{Oral}
	\gdef\@journalshort{Oral}
	\gdef\@doiabbr{oral}
	\gdef\@ISSN{2673-6373}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{organics}{%
	\gdef\@journal{organics}
	\gdef\@journalfull{Organics}
	\gdef\@journalshort{Organics}
	\gdef\@doiabbr{org}
	\gdef\@ISSN{2673-401X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{organoids}{%
	\gdef\@journal{organoids}
	\gdef\@journalfull{Organoids}
	\gdef\@journalshort{Organoids}
	\gdef\@doiabbr{organoids}
	\gdef\@ISSN{2674-1172}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{osteology}{%
	\gdef\@journal{osteology}
	\gdef\@journalfull{Osteology}
	\gdef\@journalshort{Osteology}
	\gdef\@doiabbr{osteology}
	\gdef\@ISSN{2673-4036}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{oxygen}{%
	\gdef\@journal{oxygen}
	\gdef\@journalfull{Oxygen}
	\gdef\@journalshort{Oxygen}
	\gdef\@doiabbr{oxygen}
	\gdef\@ISSN{2673-9801}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{parasites}{%
	\gdef\@journal{parasites}
	\gdef\@journalfull{Parasites}
	\gdef\@journalshort{Parasites}
	\gdef\@doiabbr{parasites}
	\gdef\@ISSN{2673-5946}
	\gdef\@societyowner{}
}
\DeclareOption{parasitologia}{%
	\gdef\@journal{parasitologia}
	\gdef\@journalfull{Parasitologia}
	\gdef\@journalshort{Parasitologia}
	\gdef\@doiabbr{parasitologia}
	\gdef\@ISSN{2673-6772}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{particles}{%
	\gdef\@journal{particles}
	\gdef\@journalfull{Particles}
	\gdef\@journalshort{Particles}
	\gdef\@doiabbr{particles}
	\gdef\@ISSN{2571-712X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{pathogens}{%
	\gdef\@journal{pathogens}
	\gdef\@journalfull{Pathogens}
	\gdef\@journalshort{Pathogens}
	\gdef\@doiabbr{pathogens}
	\gdef\@ISSN{2076-0817}
	\gdef\@societyowner{}
}
\DeclareOption{pathophysiology}{%
	\gdef\@journal{pathophysiology}
	\gdef\@journalfull{Pathophysiology}
	\gdef\@journalshort{Pathophysiology}
	\gdef\@doiabbr{pathophysiology}
	\gdef\@ISSN{0928-4680}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{pediatrrep}{%
	\gdef\@journal{pediatrrep}
	\gdef\@journalfull{Pediatric Reports}
	\gdef\@journalshort{Pediatr. Rep.}
	\gdef\@doiabbr{pediatric}
	\gdef\@ISSN{2036-7503}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{pets}{%
	\gdef\@journal{pets}
	\gdef\@journalfull{Pets}
	\gdef\@journalshort{Pets}
	\gdef\@doiabbr{pets}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{pharmaceuticals}{%
	\gdef\@journal{pharmaceuticals}
	\gdef\@journalfull{Pharmaceuticals}
	\gdef\@journalshort{Pharmaceuticals}
	\gdef\@doiabbr{ph}
	\gdef\@ISSN{1424-8247}
	\gdef\@societyowner{}
}
\DeclareOption{pharmaceutics}{%
	\gdef\@journal{pharmaceutics}
	\gdef\@journalfull{Pharmaceutics}
	\gdef\@journalshort{Pharmaceutics}
	\gdef\@doiabbr{pharmaceutics}
	\gdef\@ISSN{1999-4923}
	\gdef\@societyowner{}
}
\DeclareOption{pharmacoepidemiology}{%
	\gdef\@journal{pharmacoepidemiology}
	\gdef\@journalfull{Pharmacoepidemiology}
	\gdef\@journalshort{Pharmacoepidemiology}
	\gdef\@doiabbr{pharma}
	\gdef\@ISSN{2813-0618}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{pharmacy}{%
	\gdef\@journal{pharmacy}
	\gdef\@journalfull{Pharmacy}
	\gdef\@journalshort{Pharmacy}
	\gdef\@doiabbr{pharmacy}
	\gdef\@ISSN{2226-4787}
	\gdef\@societyowner{}
}
\DeclareOption{philosophies}{%
	\gdef\@journal{philosophies}
	\gdef\@journalfull{Philosophies}
	\gdef\@journalshort{Philosophies}
	\gdef\@doiabbr{philosophies}
	\gdef\@ISSN{2409-9287}
	\gdef\@societyowner{}
}
\DeclareOption{photochem}{%
	\gdef\@journal{photochem}
	\gdef\@journalfull{Photochem}
	\gdef\@journalshort{Photochem}
	\gdef\@doiabbr{photochem}
	\gdef\@ISSN{2673-7256}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{photonics}{%
	\gdef\@journal{photonics}
	\gdef\@journalfull{Photonics}
	\gdef\@journalshort{Photonics}
	\gdef\@doiabbr{photonics}
	\gdef\@ISSN{2304-6732}
	\gdef\@societyowner{}
}
\DeclareOption{phycology}{%
	\gdef\@journal{phycology}
	\gdef\@journalfull{Phycology}
	\gdef\@journalshort{Phycology}
	\gdef\@doiabbr{phycology}
	\gdef\@ISSN{2673-9410}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{physchem}{%
	\gdef\@journal{physchem}
	\gdef\@journalfull{Physchem}
	\gdef\@journalshort{Physchem}
	\gdef\@doiabbr{physchem}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{physics}{%
	\gdef\@journal{physics}
	\gdef\@journalfull{Physics}
	\gdef\@journalshort{Physics}
	\gdef\@doiabbr{physics}
	\gdef\@ISSN{2624-8174}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{physiologia}{%
	\gdef\@journal{physiologia}
	\gdef\@journalfull{Physiologia}
	\gdef\@journalshort{Physiologia}
	\gdef\@doiabbr{physiologia}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{plants}{%
	\gdef\@journal{plants}
	\gdef\@journalfull{Plants}
	\gdef\@journalshort{Plants}
	\gdef\@doiabbr{plants}
	\gdef\@ISSN{2223-7747}
	\gdef\@societyowner{}
}
\DeclareOption{plasma}{%
	\gdef\@journal{plasma}
	\gdef\@journalfull{Plasma}
	\gdef\@journalshort{Plasma}
	\gdef\@doiabbr{plasma}
	\gdef\@ISSN{2571-6182}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{platforms}{%
	\gdef\@journal{platforms}
	\gdef\@journalfull{Platforms}
	\gdef\@journalshort{Platforms}
	\gdef\@doiabbr{platforms}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{pollutants}{%
	\gdef\@journal{pollutants}
	\gdef\@journalfull{Pollutants}
	\gdef\@journalshort{Pollutants}
	\gdef\@doiabbr{pollutants}
	\gdef\@ISSN{2673-4672}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{polymers}{%
	\gdef\@journal{polymers}
	\gdef\@journalfull{Polymers}
	\gdef\@journalshort{Polymers}
	\gdef\@doiabbr{polym}
	\gdef\@ISSN{2073-4360}
	\gdef\@societyowner{}
}
\DeclareOption{polysaccharides}{%
	\gdef\@journal{polysaccharides}
	\gdef\@journalfull{Polysaccharides}
	\gdef\@journalshort{Polysaccharides}
	\gdef\@doiabbr{polysaccharides}
	\gdef\@ISSN{2673-4176}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{populations}{%
	\gdef\@journal{populations}
	\gdef\@journalfull{Populations}
	\gdef\@journalshort{Populations}
	\gdef\@doiabbr{populations}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{poultry}{%
	\gdef\@journal{poultry}
	\gdef\@journalfull{Poultry}
	\gdef\@journalshort{Poultry}
	\gdef\@doiabbr{poultry}
	\gdef\@ISSN{2674-1164}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{powders}{%
	\gdef\@journal{powders}
	\gdef\@journalfull{Powders}
	\gdef\@journalshort{Powders}
	\gdef\@doiabbr{powders}
	\gdef\@ISSN{2674-0516}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{preprints}{%
	\gdef\@journal{preprints}
	\gdef\@journalfull{Preprints}
	\gdef\@journalshort{Preprints}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{proceedings}{%
	\gdef\@journal{proceedings}
	\gdef\@journalfull{Proceedings}
	\gdef\@journalshort{Proceedings}
	\gdef\@doiabbr{proceedings}
	\gdef\@ISSN{2504-3900}
	\gdef\@societyowner{}
}
\DeclareOption{processes}{%
	\gdef\@journal{processes}
	\gdef\@journalfull{Processes}
	\gdef\@journalshort{Processes}
	\gdef\@doiabbr{pr}
	\gdef\@ISSN{2227-9717}
	\gdef\@societyowner{}
}
\DeclareOption{prosthesis}{%
	\gdef\@journal{prosthesis}
	\gdef\@journalfull{Prosthesis}
	\gdef\@journalshort{Prosthesis}
	\gdef\@doiabbr{prosthesis}
	\gdef\@ISSN{2673-1592}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{proteomes}{%
	\gdef\@journal{proteomes}
	\gdef\@journalfull{Proteomes}
	\gdef\@journalshort{Proteomes}
	\gdef\@doiabbr{proteomes}
	\gdef\@ISSN{2227-7382}
	\gdef\@societyowner{}
}
\DeclareOption{psf}{%
	\gdef\@journal{psf}
	\gdef\@journalfull{Physical Sciences Forum}
	\gdef\@journalshort{Phys. Sci. Forum}
	\gdef\@doiabbr{psf}
	\gdef\@ISSN{2673-9984}
	\gdef\@societyowner{}
}
%\DeclareOption{psych}{%
%	\gdef\@journal{psych}
%	\gdef\@journalfull{Psych}
%   \gdef\@journalshort{Psych}
%	\gdef\@doiabbr{psych}
%	\gdef\@ISSN{2624-8611}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{psychiatryint}{%
	\gdef\@journal{psychiatryint}
	\gdef\@journalfull{Psychiatry International}
	\gdef\@journalshort{Psychiatry Int.}
	\gdef\@doiabbr{psychiatryint}
	\gdef\@ISSN{2673-5318}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{psychoactives}{%
	\gdef\@journal{psychoactives}
	\gdef\@journalfull{Psychoactives}
	\gdef\@journalshort{Psychoactives}
	\gdef\@doiabbr{psychoactives}
	\gdef\@ISSN{2813-1851}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{psycholint}{%
	\gdef\@journal{psycholint}
	\gdef\@journalfull{Psychology International}
	\gdef\@journalshort{Psychol. Int.}
	\gdef\@doiabbr{psycholint}
	\gdef\@ISSN{2813-9844}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{publications}{%
	\gdef\@journal{publications}
	\gdef\@journalfull{Publications}
	\gdef\@journalshort{Publications}
	\gdef\@doiabbr{publications}
	\gdef\@ISSN{2304-6775}
	\gdef\@societyowner{}
}
\DeclareOption{purification}{%
	\gdef\@journal{purification}
	\gdef\@journalfull{Purification}
	\gdef\@journalshort{Purification}
	\gdef\@doiabbr{purification}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{quantumrep}{%
	\gdef\@journal{quantumrep}
	\gdef\@journalfull{Quantum Reports}
	\gdef\@journalshort{Quantum Rep.}
	\gdef\@doiabbr{quantum}
	\gdef\@ISSN{2624-960X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{quaternary}{%
	\gdef\@journal{quaternary}
	\gdef\@journalfull{Quaternary}
	\gdef\@journalshort{Quaternary}
	\gdef\@doiabbr{quat}
	\gdef\@ISSN{2571-550X}
	\gdef\@societyowner{}
}
\DeclareOption{qubs}{%
	\gdef\@journal{qubs}
	\gdef\@journalfull{Quantum Beam Science}
	\gdef\@journalshort{Quantum Beam Sci.}
	\gdef\@doiabbr{qubs}
	\gdef\@ISSN{2412-382X}
	\gdef\@societyowner{}
}
\DeclareOption{radiation}{%
	\gdef\@journal{radiation}
	\gdef\@journalfull{Radiation}
	\gdef\@journalshort{Radiation}
	\gdef\@doiabbr{radiation}
	\gdef\@ISSN{2673-592X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{reactions}{%
	\gdef\@journal{reactions}
	\gdef\@journalfull{Reactions}
	\gdef\@journalshort{Reactions}
	\gdef\@doiabbr{reactions}
	\gdef\@ISSN{2624-781X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{realestate}{%
	\gdef\@journal{realestate}
	\gdef\@journalfull{Real Estate}
	\gdef\@journalshort{Real Estate}
	\gdef\@doiabbr{realestate}
	\gdef\@ISSN{2813-8090}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{receptors}{%
	\gdef\@journal{receptors}
	\gdef\@journalfull{Receptors}
	\gdef\@journalshort{Receptors}
	\gdef\@doiabbr{receptors}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{recycling}{%
	\gdef\@journal{recycling}
	\gdef\@journalfull{Recycling}
	\gdef\@journalshort{Recycling}
	\gdef\@doiabbr{recycling}
	\gdef\@ISSN{2313-4321}
	\gdef\@societyowner{}
}
\DeclareOption{regeneration}{%
	\gdef\@journal{regeneration}
	\gdef\@journalfull{Regeneration}
	\gdef\@journalshort{Regeneration}
	\gdef\@doiabbr{regeneration}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{religions}{%
	\gdef\@journal{religions}
	\gdef\@journalfull{Religions}
	\gdef\@journalshort{Religions}
	\gdef\@doiabbr{rel}
	\gdef\@ISSN{2077-1444}
	\gdef\@societyowner{}
}
\DeclareOption{remotesensing}{%
	\gdef\@journal{remotesensing}
	\gdef\@journalfull{Remote Sensing}
	\gdef\@journalshort{Remote Sens.}
	\gdef\@doiabbr{rs}
	\gdef\@ISSN{2072-4292}
	\gdef\@societyowner{}
}
\DeclareOption{reports}{%
	\gdef\@journal{reports}
	\gdef\@journalfull{Reports}
	\gdef\@journalshort{Reports}
	\gdef\@doiabbr{reports}
	\gdef\@ISSN{2571-841X}
	\gdef\@societyowner{}
}
\DeclareOption{reprodmed}{%
	\gdef\@journal{reprodmed}
	\gdef\@journalfull{Reproductive Medicine}
	\gdef\@journalshort{Reprod. Med.}
	\gdef\@doiabbr{reprodmed}
	\gdef\@ISSN{2673-3897}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{resources}{%
	\gdef\@journal{resources}
	\gdef\@journalfull{Resources}
	\gdef\@journalshort{Resources}
	\gdef\@doiabbr{resources}
	\gdef\@ISSN{2079-9276}
	\gdef\@societyowner{}
}
\DeclareOption{rheumato}{%
	\gdef\@journal{rheumato}
	\gdef\@journalfull{Rheumato}
	\gdef\@journalshort{Rheumato}
	\gdef\@doiabbr{rheumato}
	\gdef\@ISSN{2674-0621}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{risks}{%
	\gdef\@journal{risks}
	\gdef\@journalfull{Risks}
	\gdef\@journalshort{Risks}
	\gdef\@doiabbr{risks}
	\gdef\@ISSN{2227-9091}
	\gdef\@societyowner{}
}
\DeclareOption{robotics}{%
	\gdef\@journal{robotics}
	\gdef\@journalfull{Robotics}
	\gdef\@journalshort{Robotics}
	\gdef\@doiabbr{robotics}
	\gdef\@ISSN{2218-6581}
	\gdef\@societyowner{}
}
\DeclareOption{rsee}{%
	\gdef\@journal{rsee}
	\gdef\@journalfull{Regional Science and Environmental Economics}
	\gdef\@journalshort{Reg. Sci. Environ. Econ.}
	\gdef\@doiabbr{rsee}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ruminants}{%
	\gdef\@journal{ruminants}
	\gdef\@journalfull{Ruminants}
	\gdef\@journalshort{Ruminants}
	\gdef\@doiabbr{ruminants}
	\gdef\@ISSN{2673-933X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{safety}{%
	\gdef\@journal{safety}
	\gdef\@journalfull{Safety}
	\gdef\@journalshort{Safety}
	\gdef\@doiabbr{safety}
	\gdef\@ISSN{2313-576X}
	\gdef\@societyowner{}
}
\DeclareOption{sci}{%
	\gdef\@journal{sci}
	\gdef\@journalfull{Sci}
	\gdef\@journalshort{Sci}
	\gdef\@doiabbr{sci}
	\gdef\@ISSN{2413-4155}
	\gdef\@societyowner{}
}
\DeclareOption{scipharm}{%
	\gdef\@journal{scipharm}
	\gdef\@journalfull{Scientia Pharmaceutica}
	\gdef\@journalshort{Sci. Pharm.}
	\gdef\@doiabbr{scipharm}
	\gdef\@ISSN{2218-0532}
	\gdef\@societyowner{\"{O}sterreichische Pharmazeutische Gesellschaft}
}
\DeclareOption{sclerosis}{%
	\gdef\@journal{sclerosis}
	\gdef\@journalfull{Sclerosis}
	\gdef\@journalshort{Sclerosis}
	\gdef\@doiabbr{sclerosis}
	\gdef\@ISSN{2813-3064}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{seeds}{%
	\gdef\@journal{seeds}
	\gdef\@journalfull{Seeds}
	\gdef\@journalshort{Seeds}
	\gdef\@doiabbr{seeds}
	\gdef\@ISSN{2674-1024}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sensors}{%
	\gdef\@journal{sensors}
	\gdef\@journalfull{Sensors}
	\gdef\@journalshort{Sensors}
	\gdef\@doiabbr{s}
	\gdef\@ISSN{1424-8220}
	\gdef\@societyowner{}
}
\DeclareOption{separations}{%
	\gdef\@journal{separations}
	\gdef\@journalfull{Separations}
	\gdef\@journalshort{Separations}
	\gdef\@doiabbr{separations}
	\gdef\@ISSN{2297-8739}
	\gdef\@societyowner{}
}
\DeclareOption{sexes}{%
	\gdef\@journal{sexes}
	\gdef\@journalfull{Sexes}
	\gdef\@journalshort{Sexes}
	\gdef\@doiabbr{sexes}
	\gdef\@ISSN{2411-5118}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{signals}{%
	\gdef\@journal{signals}
	\gdef\@journalfull{Signals}
	\gdef\@journalshort{Signals}
	\gdef\@doiabbr{signals}
	\gdef\@ISSN{2624-6120}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sinusitis}{%
	\gdef\@journal{sinusitis}
	\gdef\@journalfull{Sinusitis}
	\gdef\@journalshort{Sinusitis}
	\gdef\@doiabbr{sinusitis}
	\gdef\@ISSN{2309-107X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{siuj}{%
	\gdef\@journal{siuj}
	\gdef\@journalfull{Soci\'{e}t\'{e} Internationale d'Urologie Journal}
	\gdef\@journalshort{Soc. Int. Urol. J.}
	\gdef\@doiabbr{siuj}
	\gdef\@ISSN{2563-6499}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{Soci\'{e}t\'{e} Internationale d'Urologie}
}
\DeclareOption{skins}{%
	\gdef\@journal{skins}
	\gdef\@journalfull{Skins}
	\gdef\@journalshort{Skins}
	\gdef\@doiabbr{skins}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{smartcities}{%
	\gdef\@journal{smartcities}
	\gdef\@journalfull{Smart Cities}
	\gdef\@journalshort{Smart Cities}
	\gdef\@doiabbr{smartcities}
	\gdef\@ISSN{2624-6511}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sna}{%
	\gdef\@journal{sna}
	\gdef\@journalfull{Sinusitis and Asthma}
	\gdef\@journalshort{Sinusitis Asthma}
	\gdef\@doiabbr{sna}
	\gdef\@ISSN{2624-7003}
	\gdef\@societyowner{}
}
\DeclareOption{societies}{%
	\gdef\@journal{societies}
	\gdef\@journalfull{Societies}
	\gdef\@journalshort{Societies}
	\gdef\@doiabbr{soc}
	\gdef\@ISSN{2075-4698}
	\gdef\@societyowner{}
}
\DeclareOption{socsci}{%
	\gdef\@journal{socsci}
	\gdef\@journalfull{Social Sciences}
	\gdef\@journalshort{Soc. Sci.}
	\gdef\@doiabbr{socsci}
	\gdef\@ISSN{2076-0760}
	\gdef\@societyowner{}
}
\DeclareOption{software}{%
	\gdef\@journal{software}
	\gdef\@journalfull{Software}
	\gdef\@journalshort{Software}
	\gdef\@doiabbr{software}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{soilsystems}{%
	\gdef\@journal{soilsystems}
	\gdef\@journalfull{Soil Systems}
	\gdef\@journalshort{Soil Syst.}
	\gdef\@doiabbr{soilsystems}
	\gdef\@ISSN{2571-8789}
	\gdef\@societyowner{}
}
\DeclareOption{solar}{%
	\gdef\@journal{solar}
	\gdef\@journalfull{Solar}
	\gdef\@journalshort{Solar}
	\gdef\@doiabbr{solar}
	\gdef\@ISSN{2673-9941}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{solids}{%
	\gdef\@journal{solids}
	\gdef\@journalfull{Solids}
	\gdef\@journalshort{Solids}
	\gdef\@doiabbr{solids}
	\gdef\@ISSN{2673-6497}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{spectroscj}{%
	\gdef\@journal{spectroscj}
	\gdef\@journalfull{Spectroscopy Journal}
	\gdef\@journalshort{Spectrosc. J.}
	\gdef\@doiabbr{spectroscj}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sports}{%
	\gdef\@journal{sports}
	\gdef\@journalfull{Sports}
	\gdef\@journalshort{Sports}
	\gdef\@doiabbr{sports}
	\gdef\@ISSN{2075-4663}
	\gdef\@societyowner{}
}
\DeclareOption{standards}{%
	\gdef\@journal{standards}
	\gdef\@journalfull{Standards}
	\gdef\@journalshort{Standards}
	\gdef\@doiabbr{standards}
	\gdef\@ISSN{2305-6703}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{stats}{%
	\gdef\@journal{stats}
	\gdef\@journalfull{Stats}
	\gdef\@journalshort{Stats}
	\gdef\@doiabbr{stats}
	\gdef\@ISSN{2571-905X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{std}{%
	\gdef\@journal{std}
	\gdef\@journalfull{Surgical Techniques Development}
	\gdef\@journalshort{Surg. Tech. Dev.}
	\gdef\@doiabbr{std}
	\gdef\@ISSN{2038-9582}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{stresses}{%
	\gdef\@journal{stresses}
	\gdef\@journalfull{Stresses}
	\gdef\@journalshort{Stresses}
	\gdef\@doiabbr{stresses}
	\gdef\@ISSN{2673-7140}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{surfaces}{%
	\gdef\@journal{surfaces}
	\gdef\@journalfull{Surfaces}
	\gdef\@journalshort{Surfaces}
	\gdef\@doiabbr{surfaces}
	\gdef\@ISSN{2571-9637}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{surgeries}{%
	\gdef\@journal{surgeries}
	\gdef\@journalfull{Surgeries}
	\gdef\@journalshort{Surgeries}
	\gdef\@doiabbr{surgeries}
	\gdef\@ISSN{2017-2017}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{suschem}{%
	\gdef\@journal{suschem}
	\gdef\@journalfull{Sustainable Chemistry}
	\gdef\@journalshort{Sustain. Chem.}
	\gdef\@doiabbr{suschem}
	\gdef\@ISSN{2673-4079}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sustainability}{%
	\gdef\@journal{sustainability}
	\gdef\@journalfull{Sustainability}
	\gdef\@journalshort{Sustainability}
	\gdef\@doiabbr{su}
	\gdef\@ISSN{2071-1050}
	\gdef\@societyowner{}
}
\DeclareOption{symmetry}{%
	\gdef\@journal{symmetry}
	\gdef\@journalfull{Symmetry}
	\gdef\@journalshort{Symmetry}
	\gdef\@doiabbr{sym}
	\gdef\@ISSN{2073-8994}
	\gdef\@societyowner{}
}
\DeclareOption{synbio}{%
	\gdef\@journal{synbio}
	\gdef\@journalfull{SynBio}
	\gdef\@journalshort{SynBio}
	\gdef\@doiabbr{synbio}
	\gdef\@ISSN{2674-0583}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{systems}{%
	\gdef\@journal{systems}
	\gdef\@journalfull{Systems}
	\gdef\@journalshort{Systems}
	\gdef\@doiabbr{systems}
	\gdef\@ISSN{2079-8954}
	\gdef\@societyowner{}
}
\DeclareOption{targets}{%
	\gdef\@journal{targets}
	\gdef\@journalfull{Targets}
	\gdef\@journalshort{Targets}
	\gdef\@doiabbr{targets}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{taxonomy}{%
	\gdef\@journal{taxonomy}
	\gdef\@journalfull{Taxonomy}
	\gdef\@journalshort{Taxonomy}
	\gdef\@doiabbr{taxonomy}
	\gdef\@ISSN{2673-6500}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{technologies}{%
	\gdef\@journal{technologies}
	\gdef\@journalfull{Technologies}
	\gdef\@journalshort{Technologies}
	\gdef\@doiabbr{technologies}
	\gdef\@ISSN{2227-7080}
	\gdef\@societyowner{}
}
\DeclareOption{telecom}{%
	\gdef\@journal{telecom}
	\gdef\@journalfull{Telecom}
	\gdef\@journalshort{Telecom}
	\gdef\@doiabbr{telecom}
	\gdef\@ISSN{2673-4001}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{Test}
	\gdef\@journalshort{Test}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{textiles}{%
	\gdef\@journal{textiles}
	\gdef\@journalfull{Textiles}
	\gdef\@journalshort{Textiles}
	\gdef\@doiabbr{textiles}
	\gdef\@ISSN{2673-7248}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{thalassrep}{%
	\gdef\@journal{thalassrep}
	\gdef\@journalfull{Thalassemia Reports}
	\gdef\@journalshort{Thalass. Rep.}
	\gdef\@doiabbr{thalassrep}
	\gdef\@ISSN{2039-4365}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{therapeutics}{%
	\gdef\@journal{therapeutics}
	\gdef\@journalfull{Therapeutics}
	\gdef\@journalshort{Therapeutics}
	\gdef\@doiabbr{therapeutics}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{thermo}{%
	\gdef\@journal{thermo}
	\gdef\@journalfull{Thermo}
	\gdef\@journalshort{Thermo}
	\gdef\@doiabbr{thermo}
	\gdef\@ISSN{2673-7264}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{timespace}{%
	\gdef\@journal{timespace}
	\gdef\@journalfull{Time and Space}
	\gdef\@journalshort{Time Space}
	\gdef\@doiabbr{timespace}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{tomography}{%
	\gdef\@journal{tomography}
	\gdef\@journalfull{Tomography}
	\gdef\@journalshort{Tomography}
	\gdef\@doiabbr{tomography}
	\gdef\@ISSN{2379-139X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{tourismhosp}{%
	\gdef\@journal{tourismhosp}
	\gdef\@journalfull{Tourism and Hospitality}
	\gdef\@journalshort{Tour. Hosp.}
	\gdef\@doiabbr{tourhosp}
	\gdef\@ISSN{2673-5768}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{toxics}{%
	\gdef\@journal{toxics}
	\gdef\@journalfull{Toxics}
	\gdef\@journalshort{Toxics}
	\gdef\@doiabbr{toxics}
	\gdef\@ISSN{2305-6304}
	\gdef\@societyowner{}
}
\DeclareOption{toxins}{%
	\gdef\@journal{toxins}
	\gdef\@journalfull{Toxins}
	\gdef\@journalshort{Toxins}
	\gdef\@doiabbr{toxins}
	\gdef\@ISSN{2072-6651}
	\gdef\@societyowner{}
}
\DeclareOption{transplantology}{%
	\gdef\@journal{transplantology}
	\gdef\@journalfull{Transplantology}
	\gdef\@journalshort{Transplantology}
	\gdef\@doiabbr{transplantology}
	\gdef\@ISSN{2673-3943}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{transportation}{%
	\gdef\@journal{transportation}
	\gdef\@journalfull{Transportation}
	\gdef\@journalshort{Transportation}
	\gdef\@doiabbr{transportation}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{traumacare}{%
	\gdef\@journal{traumacare}
	\gdef\@journalfull{Trauma Care}
	\gdef\@journalshort{Trauma Care}
	\gdef\@doiabbr{traumacare}
	\gdef\@ISSN{2673-866X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{traumas}{%
	\gdef\@journal{traumas}
	\gdef\@journalfull{Traumas}
	\gdef\@journalshort{Traumas}
	\gdef\@doiabbr{traumas}
	\gdef\@ISSN{2673-7477}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{tropicalmed}{%
	\gdef\@journal{tropicalmed}
	\gdef\@journalfull{Tropical Medicine and Infectious Disease}
	\gdef\@journalshort{Trop. Med. Infect. Dis.}
	\gdef\@doiabbr{tropicalmed}
	\gdef\@ISSN{2414-6366}
	\gdef\@societyowner{}
}
\DeclareOption{universe}{%
	\gdef\@journal{universe}
	\gdef\@journalfull{Universe}
	\gdef\@journalshort{Universe}
	\gdef\@doiabbr{universe}
	\gdef\@ISSN{2218-1997}
	\gdef\@societyowner{}
}
\DeclareOption{urbansci}{%
	\gdef\@journal{urbansci}
	\gdef\@journalfull{Urban Science}
	\gdef\@journalshort{Urban Sci.}
	\gdef\@doiabbr{urbansci}
	\gdef\@ISSN{2413-8851}
	\gdef\@societyowner{}
}
\DeclareOption{uro}{%
	\gdef\@journal{uro}
	\gdef\@journalfull{Uro}
	\gdef\@journalshort{Uro}
	\gdef\@doiabbr{uro}
	\gdef\@ISSN{2673-4397}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{vaccines}{%
	\gdef\@journal{vaccines}
	\gdef\@journalfull{Vaccines}
	\gdef\@journalshort{Vaccines}
	\gdef\@doiabbr{vaccines}
	\gdef\@ISSN{2076-393X}
	\gdef\@societyowner{}
}
\DeclareOption{vehicles}{%
	\gdef\@journal{vehicles}
	\gdef\@journalfull{Vehicles}
	\gdef\@journalshort{Vehicles}
	\gdef\@doiabbr{vehicles}
	\gdef\@ISSN{2624-8921}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{venereology}{%
	\gdef\@journal{venereology}
	\gdef\@journalfull{Venereology}
	\gdef\@journalshort{Venereology}
	\gdef\@doiabbr{venereology}
	\gdef\@ISSN{2674-0710}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{vetsci}{%
	\gdef\@journal{vetsci}
	\gdef\@journalfull{Veterinary Sciences}
	\gdef\@journalshort{Vet. Sci.}
	\gdef\@doiabbr{vetsci}
	\gdef\@ISSN{2306-7381}
	\gdef\@societyowner{}
}
\DeclareOption{vibration}{%
	\gdef\@journal{vibration}
	\gdef\@journalfull{Vibration}
	\gdef\@journalshort{Vibration}
	\gdef\@doiabbr{vibration}
	\gdef\@ISSN{2571-631X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{virtualworlds}{%
	\gdef\@journal{virtualworlds}
	\gdef\@journalfull{Virtual Worlds}
	\gdef\@journalshort{Virtual Worlds}
	\gdef\@doiabbr{virtualworlds}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{viruses}{%
	\gdef\@journal{viruses}
	\gdef\@journalfull{Viruses}
	\gdef\@journalshort{Viruses}
	\gdef\@doiabbr{v}
	\gdef\@ISSN{1999-4915}
	\gdef\@societyowner{}
}
\DeclareOption{vision}{%
	\gdef\@journal{vision}
	\gdef\@journalfull{Vision}
	\gdef\@journalshort{Vision}
	\gdef\@doiabbr{vision}
	\gdef\@ISSN{2411-5150}
	\gdef\@societyowner{}
}
\DeclareOption{waste}{%
	\gdef\@journal{waste}
	\gdef\@journalfull{Waste}
	\gdef\@journalshort{Waste}
	\gdef\@doiabbr{waste}
	\gdef\@ISSN{2813-0391}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{water}{%
	\gdef\@journal{water}
	\gdef\@journalfull{Water}
	\gdef\@journalshort{Water}
	\gdef\@doiabbr{w}
	\gdef\@ISSN{2073-4441}
	\gdef\@societyowner{}
}
\DeclareOption{wem}{%
	\gdef\@journal{wem}
	\gdef\@journalfull{Wildlife Ecology and Management}
	\gdef\@journalshort{Wildl. Ecol. Manag.}
	\gdef\@doiabbr{}
	\gdef\@ISSN{1234-4321}
	\gdef\@societyowner{}
}
\DeclareOption{wevj}{%
	\gdef\@journal{wevj}
	\gdef\@journalfull{World Electric Vehicle Journal}
	\gdef\@journalshort{World Electr. Veh. J.}
	\gdef\@doiabbr{wevj}
	\gdef\@ISSN{2032-6653}
	\gdef\@societyowner{World Electric Vehicle Association}
}
\DeclareOption{wild}{%
	\gdef\@journal{wild}
	\gdef\@journalfull{Wild}
	\gdef\@journalshort{Wild}
	\gdef\@doiabbr{wild}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{wind}{%
	\gdef\@journal{wind}
	\gdef\@journalfull{Wind}
	\gdef\@journalshort{Wind}
	\gdef\@doiabbr{wind}
	\gdef\@ISSN{2674-032X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{women}{%
	\gdef\@journal{women}
	\gdef\@journalfull{Women}
	\gdef\@journalshort{Women}
	\gdef\@doiabbr{women}
	\gdef\@ISSN{2673-4184}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{world}{%
	\gdef\@journal{world}
	\gdef\@journalfull{World}
	\gdef\@journalshort{World}
	\gdef\@doiabbr{world}
	\gdef\@ISSN{2673-4060}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{youth}{%
	\gdef\@journal{youth}
	\gdef\@journalfull{Youth}
	\gdef\@journalshort{Youth}
	\gdef\@doiabbr{youth}
	\gdef\@ISSN{2673-995X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{zoonoticdis}{%
	\gdef\@journal{zoonoticdis}
	\gdef\@journalfull{Zoonotic Diseases}
	\gdef\@journalshort{Zoonotic Dis.}
	\gdef\@doiabbr{zoonoticdis}
	\gdef\@ISSN{2813-0227}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}


==> chaptersPaper/ambiguity.tex <==
This section introduces the contributions of this paper. 
Starting with the problem statement, we quickly explain how the framework solves the problem and carry on to showing how this can be mapped to a quantum circuit. 
After presenting a brief study emphasising the effect of the framework, we relate the theory to the DisCoCat framework and give ideas for future work. 

In the state-of-the-art literature in QNLP, ... 

Consider the sentence: 
\begin{displayquote}
    \texttt{Alice drinks her tea and Mary does too.}
\end{displayquote}
There are two readings for this diagram: 
\jurek{two readings}
Following \citet{Wijnholds_2020}, these can be modelled using the two pregroup diagrams: 

\jurek{insert pregroup diagrams}

Consider: 
\begin{displayquote}
    \texttt{Cat hunts dog. It is fast.}
\end{displayquote}
Where there are two readings 
\jurek{two readings}
\citet{pronounResolution} argue that these two readings correspond to the pregroup diagrams: 
\jurek{pregroup diagrams, should I proof that this is indeed the case? }

In this section of the paper, we introduce probability distributions over different ways of reading sentences by assigning marker words certain morphisms, followed by elevating these morphisms to be quantum maps. 
We then describe the whole diagram as a probability distribution over the possible compositions. 
Finally, we show how to map the density matrix diagrams to quantum circuits, where entangling patterns are applied in appropriate places of the diagrams. 


There are many more examples, but for introducing the idea we stick to these two. 
In both of the above discussed examples, there exist two readings for the sentences, each modelled differently in the diagrammatic language. 

In the current DisCoCat framework, these are modelled separately from each other; either one or the other. 
Motivated by how the human mind works, we claim that these can be modelled in the same expression, which is a probability distribution over the two readings. 

In occasions like these, humans remember this ambiguity and resolve it only when more information is obtained. 
The meaning of the sentence \textbf{is} the ambiguity. 

As mentioned above, the goal is to create a probability distribution over the two readings, in such a way that the overall meaning of the sentence is a mixed state, composed of the two pure states corresponding to the respecitve meanings. 
\begin{equation}
    \rho_{\texttt{sentence}} = \alpha \cdot \rho_{\texttt{reading one}} + \beta \cdot \rho_{\texttt{reading two}}
\end{equation}
where $\rho$ are density matrices and $\alpha + \beta = 1$. 

We approach this in the following way: 
\begin{enumerate}
    \item We identify the ambiguous word in the sentence (the source of ambiguity in the sentence)
    \item We model the word as a morphism acting on the other words in the sentence 
    \item We create a probability distribution over these two readings by assigning a (naive) probability to each of the respective readings
\end{enumerate}

% *************************************
\subsection*{An introductory example}
% *************************************

We demonstrate this procedure for a number of examples. We start with a simple sentence, containing a simple example of lexical ambiguity. 
\begin{displayquote}
    \texttt{The Man sees the woman on a mountain.}
\end{displayquote}
The phrase \texttt{on a mountain} can describe either the \texttt{man} being on a mountain or the \texttt{woman} being on a mountain. 

The two possible DisCoCat diagrams arising from this sentence are: 

\ctikzfig{manWomanOnMountain}

where we \jurek{ignored} the words \texttt{the} and \texttt{a} and modelled \texttt{on mountain} as a noun modifier, modifying either \texttt{man} or \texttt{woman}. 

We want to find a general diagrammatic way of displaying the effect of the phrase \texttt{on mountain} on the sentence meaning, as in: 

\ctikzfig{manWomanOnMountainGeneral}

where then the map \texttt{on-mountain} acts on all the other words in the sentence. 
To fit the two readings above, the inner structure of the state \texttt{on-mountain} would then be either of these two: 

\ctikzfig{onMountain}

where the corresponding morphisms are for the left and right diagram, respectively: 
\begin{equation*}
\begin{split}
    &(\eta_N \otimes \eta_S) \circ (1_N \otimes 1_N \otimes 1_S \otimes \overrightarrow{\texttt{on-mountain}} \otimes 1_S) \circ (1_N \otimes 1_N \otimes 1_S \otimes \sigma_{NN} \otimes 1_S) \\
    &(\overrightarrow{\texttt{on-mountain}} \otimes \eta_S) \circ (1_N \otimes 1_N \otimes 1_S \otimes \eta_N \otimes 1_S)  \\
\end{split}
\end{equation*}
where $\sigma_{NN}$ is the \textit{swap morphism}. 
We create the probability distribution over the possible interpretations as: 

\ctikzfig{onMountainDoubled}

where we use the doubled diagrams as mentioned in section \ref{sec:intro} and $\alpha, \beta \in \mathbb{R}$, where $\alpha + \beta = 1$ 
To introduce this density matrix to the diagram as above, the whole diagram has to be doubled, where the remaining states are elevated to being described by density matrices. These states are \textit{pure states}, in contrast to the density matrix described by \texttt{on-mountain} which is a mixed density matrix over the two pure states shown above. 

Now, we see how powerful and useful this model is. 
We can now \textbf{keep the ambiguity alive}, because we do have a probability distribution over the two diagrams. 
The resulting density matrices can now be updated using the updating mechanism \textit{FUZZ} and \textit{PHASER} as introduced by \citet{meaningUpdatingDensMat}. 

\jurek{explain fuzz and phaser in more detail and how to update}

% *************************************
\subsection*{Relative Pronouns in Dutch}
% *************************************

There are many more types of ambiguity that our model can capture. 
Consider e.g. the Dutch phrase: 
\begin{displayquote}
    \texttt{Mensen die dieren eten}. 
\end{displayquote}
\citet{relPronCoecke} and \citet{Wijnholds_2020} discuss ways on how to model relative pronouns. As argued by \citet{Wijnholds_2020}, in the Dutch language, the sentences \texttt{humans who eat animals} and \texttt{humans whom animals eat} have the same meaning \texttt{mensen, die dieren eten}.
In a similar fashion to the above discussed, we want a diagram structure as follows: 

\ctikzfig{mensenDierenEten}

where then the word \texttt{die} is modelled in either of these ways: 

\ctikzfig{dieModelling}

and we can form a superposition over the two states as above, by elevating the states to being density matrices. 







% *************************************
\subsection*{Pronoun resolution}
% *************************************

Consider, as a third example, the sentence 
\begin{displayquote}
    \texttt{Dog hunts cat. It is fast.}
\end{displayquote}
The phenomenon in this sentence is called \textit{coreference} and we see that the word \texttt{it} refers to a noun phrase (either \texttt{cat} or \texttt{dog}) in the former sentence. 
\citet{pronounResolution} use \textit{truncated Fock spaces} to model the mapping $V \rightarrow V\otimes V$. They model the copied word as a vector in a truncated Fock space 
\jurek{explain this shortly}. 
where they use the \textit{projection} to the $n$-th layer to access the vector in the vector space $V \otimes \ldots \otimes V$. 
Using the projection in the 2nd layer, the corresponding diagram for the example sentence \texttt{John slept. He snored.} is: 

\ctikzfig{johnSleepsHeSnores}

where we copied \texttt{cat} as an explicit example. 

Because this is not the way we would like to model our things in and to make it consistent, we translate the mechanism to the Pregroup formalism. 
Recall the Frobenius map: 
\begin{equation}
    \Delta_V : V \rightarrow V \otimes V
\end{equation}
which puts a vector on the diagonal of a matrix. 
In a pregroup diagram, the use of the $\Delta$ Frobenius map amounts to copying information, so that we can model the diagram above as: 

\ctikzfig{johnSleepsHeSnoresPregroups}

Where, generally for the modelling of a vector $v$ we have the following correspondence: 

\begin{equation*}
    \tikzfig{elementProjectionFock} \longmapsto \tikzfig{fockToPrg}
\end{equation*}
Having established this, we can introduce a probability distribution over copying either \texttt{cat} or \texttt{dog} as: 
\ctikzfig{catHuntsDogGeneral}

where again, the word it is modelled as either of the two: 

\ctikzfig{itPossibleRealisations}

where \texttt{it} is a mapping that copies either \texttt{dog} or \texttt{cat}:

\ctikzfig{itPossibleMorphismOne}

\ctikzfig{itPossibleMorphismTwo}

Now, we elevate these two morphisms to being \textit{quantum states} and create the resulting word \texttt{it} as a \textit{mixed quantum state} describing a probability distribution over the two \textit{pure quantum states} as: 

\ctikzfig{itDiagrammaticDM}

where we used the doubled diagrammatic notation introduced above, indicating that these diagrams are representing density matrices, which are themselves representing pure states. 
Now, again, the word \texttt{it} is elevated to describe a density matrix over the two pure states above. 

Note that for all the above discussed, it is possible to use the process state duality to turn states into processes, where then the notion of the \textit{marker words} being \textit{processes} that change the meaning of the words in the sentence makes much intuitive sense. 
Applied to the above example, we can model the word \texttt{it} as a density matrix acting locally on the two pure states \texttt{cat} and \texttt{dog} as: 
% The placement of the copied noun in the former case can be understood as a feature arising from the translation of the Lambek Calculus with control modalities to the Pregroup formalism. 
% The quantum states arising after the morphism has been applied are composed according to the Pregroup rules. 

\ctikzfig{catHuntsDogDesired}

This is because \textit{Only connectivity matters!}
Where, as mentioned above, the whole diagram is now drawn with thick wires, as all of the states are represented by density matrices. 

% we see that this diagram describes a probability distribution over, in this case, two different possible diagrams. In conclusion, we say that this diagram describes a mixed state, containing pure states that correspond to the simple copying mechanisms. 

Note that we have two open sentence wires. The left one captures the meaning of \texttt{cat hunts dog}, a pure state, whereas the right one captures the meaning of \texttt{it is fast}, which is a mixed state over \texttt{cat is fast} and \texttt{dog is fast}. 



% *************************************
\subsection*{Verb Phrase Ellipsis with Anaphora}
% *************************************

Consider the sentence: 
\begin{displayquote}
    \texttt{Bill eats and drinks. Mary does too.}
\end{displayquote}
With the three possible readings:
\begin{itemize}
    \item \texttt{Bill eats and drinks. Mary eats.}
    \item \texttt{Bill eats and drinks. Mary drinks.}
    \item \texttt{Bill eats and drinks. Mary eats and drinks.}
\end{itemize}
where the second phrase refers to the verb in the noun phrase. We use the methods used by \citet{Wijnholds_2020} to deal with the phrase \texttt{does too}. 
However, we go one step further in, again, integrating the copying of the verb in the former sentence into the phrase \texttt{does too}. 

\citet{Wijnholds_2020} models the phrase \texttt{does too} as: 

\ctikzfig{doesToo}

where the information in the former sentence is copied explicitly. We want to integrate these illinearities into the phrase itself as: 

\ctikzfig{billEatsDrinksMaryDoesToo}

where we used the \texttt{and} representation for verbs as: 

\ctikzfig{copyVerb}

We simplify this using the process-state duality as above: 

\jurek{process state duality applied to above}

so that the two different wirings for the word \texttt{does too} are: 

\jurek{does too wirings}

\jurek{mention that the same thing can be done, using the explicit representations of the words his or her in the case of anaphor}

We thus expand the theory by \citet{Wijnholds_2020} and capture all of the illinearity in the phrase \texttt{does too}.

\jurek{what other upsides are there to the locality of the ambiguity source???}
Other than being able to create probability distributions over mechanisms in diagrams, this procedure is a more general approach to this type of ambiguity. 
The presence of the phrase \texttt{does too} implies that information has to be copied. 


\subsection{Multiple Sources of Ambiguity}

Consider now the notion of introducing two sources of ambiguity, as in: 
\begin{displayquote}
    \texttt{The man saw the woman on the mountain with a telescope.}
\end{displayquote}
where there's six readings for this sentence: 
\begin{itemize}
    \item \texttt{The (man on the mountain) saw the (woman with a telescope)}
    \item \texttt{The (man with a telescope) saw the (woman on the mountain)}
    \item \texttt{The (man on the mountain with a telescope) saw the woman}
    \item \texttt{The man saw the (woman on the mountain with a telescope)}
    \item \texttt{The (man on the mountain) saw (with a telescope) the woman}
    \item \texttt{The man saw (with a telescope) the (woman on the mountain)}
\end{itemize}
Note that \texttt{with telescope} can either mean \texttt{who has a telescope} or \texttt{use a telescope to do something}. 
Following the reasoning above that \textit{only connectivity matters}, we can model all of these six readings within one diagram as: 

\ctikzfig{manWomanTelescope}

where, in one of the cases, the phrase \texttt{with telescope} acts as a verb modifier on the verb \texttt{saw}, and the nouns are simple wires.  

\jurek{in the appendix, we give more examples of ambiguous sentences and how to model them.}

\jurek{More examples... What examples do I show? What do I put into the appendix? There's too many. }

One can extend this to other languages as well. Consider the phrase 
\begin{displayquote}
    \texttt{Mensen, die dieren eten.}
\end{displayquote}
in Dutch, which means \texttt{Humans who eat animals}, \textbf{or} \texttt{Humans whom animals eat.}
We can create a mixed state that allows for both these readings using the formalism developed by \citet{relPronCoecke} and \citet{Wijnholds_2020}. 




Consider the simple example in which we want to compare the density matrix arising from the ambiguity above with how \texttt{TRUE} one or the other reading is. 
One can take the trace inner product with the density matrix: 
\begin{equation*}
    \Tr \big( \rho_{\texttt{it is fast}} \cdot \rho_{\texttt{TRUE}}\big)
\end{equation*}
where only $\rho_2$  





% auskommentiert .... 



%*************************
\subsection{Reasoning with the Quantum Probability Distribution }
%*************************

The reason that this approach is useful is the \textbf{maintaining} and modelling of the ambiguity. 
To emphasize this effect, consider a density matrix describing a probability distribution over different readings of a diagram in some sentence \texttt{sent1}. Consider now the meaning of a second sentence \texttt{sent2}, represented by a second density matrix. 
The interaction of these density matrices will yield a new density matrix which will then contain an updated probability distribution over the two possible readings of the first diagram, given the information acquired within the second density matrix. 

As \citet{meaningUpdatingDensMat} argue that imposing a proposition onto a density matrix is according to: 

\begin{equation*}
    P \circ - \circ P
\end{equation*}
where $P$ is a \textit{projector} in the quantum-theoretic sense. They argue that every projector is a (potentially not-normalized) density matrix and each density matrix admits a \textit{spectral decomposition} as: 
\begin{equation*}
    \sum_i x_i P_i
\end{equation*}
where $P_i$ are projectors into the eigenspace. 
\jurek{cite missing, look into meaning updating paper}
.. and ... argue that it is a natural way to reason about properties being imposed onto words as applying appropriate projectors. 

This is a very natural approach to language and ultimately models closer how the human brain works than the models before it. 
This is because, if one was to hear a sentence like \texttt{the man saw the woman on a mountain with a telescope}, one would wait until obtaining more information about said woman or man until fully collapsing the wave function. 



Consider the case in which we are dealing with \textit{real} uncertainty. Because of the lack of context, we cannot know what word is to be copied. We want to emphasize that this is not to do with the model itself, because we cannot model what we don't know. 

The powerfulness comes from \textbf{maintaining the ambiguity} and adjusting the probability distribution representing it when seeing more context. 
The meaning represented by the density matrix can the be updated via the methods \texttt{FUZZ} or \texttt{PHASER} introduced by \citet{meaningUpdatingDensMat}. 
One can furthermore compare density matrices and measure their similarity by employing methods like the \textit{trace inner product} or the \textit{fidelity}. 

These are established methods and do not contribute to the novelty of our work. We will go into more detail in section \ref{sec:experiments}. 

Consider, as a second example the sentence: 
\begin{displayquote}
    \texttt{Alice drinks her tea and Mary does too.}
\end{displayquote}
from above, as investigated by \citet{Wijnholds_2020}. 
We can unify the two diagrams into one superposition diagram in the following manner: 

%*************************
\subsection{Connection to DisCoCirc}
%*************************
As we can see in the model above, the words that are the sources of ambiguity are processes that alter the meaning of the rest of the words in the sentence. 

\citet{DisCoCirc} argue that a sentence is a \textit{process} that alters the meaning of the words that make it up. 
They argue that a sentence is in its most basic form nouns interacting and being imposed properties on by verbs, adjectives and other nouns. 

\textit{Dynamic} nouns are such whose meaning evolve with the text. These nouns are modelled as density matrices whose meanings are updated using methods introduced above. 
\textit{Static} nouns are such whose meaning is static within the sentence. The corresponding density matrices are not updated with the evolution of the sentence. 

Consider the example \texttt{Man sees woman on mountain with telescope} from above. 
The dynamic nouns in this example are \texttt{man} and \texttt{woman}. 
This sentence can be split in three parts: 
\begin{enumerate}
    \item \texttt{Man or woman is on mountain.}
    \item \texttt{Man or woman has telescope or man is using telescope.}
    \item \texttt{Man sees woman.}
\end{enumerate}

The process of sentences being processes acting on dynamic nouns is displayed as: 

\ctikzfig{sentences}

And applied to our example, this is: 

\ctikzfig{manWomanDisCoCirc}

where now the meanings of the density matrices \texttt{man} and \texttt{woman} are updated by the sentences. The initial states for \texttt{man} and \texttt{woman} can be understood as prior knowledge about \texttt{man} or \texttt{woman}. 
The individual density matrices in the diagram above are: 

\ctikzfig{saw}

Where the grey dot is either the \textit{fuzz} or \textit{phaser} discussed above. 
Note that, however, this system does not allow the meaning updating of verbs. 
As discussed above, we want to also be able to update the meaning of the verb \texttt{saw} using the density matrix \texttt{with telescope}. 
Thus, one could view the verb as a \textit{dynamic verb} whose meaning is updated after interacting with \texttt{with telescope} and afterwards applied to \texttt{man} and \texttt{woman}. 
We can model a dynamic verb e.g., as: 

\ctikzfig{dynamicVerb}

where we see that the processes \texttt{with telescope} and \texttt{on mountain} will alter the meaning of the verb as well, which will only act on the nouns \texttt{man} and \texttt{woman} when its scope is over. 

To answer the question of scope, one can end the scope of the dynamic verb by explicitly composing it with the dynamic nouns in the appropriate part of the sentence, so that: 

\ctikzfig{dynamicVerbScope}

 where we see that in the rightmost of these options, the phrase \texttt{with telescope} is a verb modifier.




%*************************
\subsection{Mapping to Quantum Circuits}
%*************************
In order to map the density matrices representing diagrams to quantum circuits, we remember the concept of entanglement from ... 

The way we approach the probability distribution over diagrams is the following: 

\ctikzfig{simpleExample}
\jurek{replace the three dots with the discarding map}
where operation $O_1$ is only executed when operation $O_2$ is not executed and vice versa. 
The above statement can be seen easily using the following calculation: 
\jurek{add calculation from your thesis}


This quantum circuit will be the ansatz for all of the examples of ambiguity that we are dealing with in this work. 
Note that, however, if there were more possible readings, one can extend the number of readings that can be displayed by adding qubits to the diagrams (adding $n$ qubits to the diagram will allow us to model $2^n$ times the ambiguity)

\jurek{explain this further}

Our quantum circuit for the example sentence \texttt{cat hunts dog. It is fast.} then structurally looks like: 

\ctikzfig{catHuntsDogQC}

where then the qubit encoding the meaning \texttt{it} will be discarded and the non-sentence wires will be connected according to the Pregroup formalism. 

Note that the same works for e.g. the sentence \texttt{Mensen die dieren eten} or \texttt{The man sees the woman on the mountain.} 
In each case, only one of the mappings is realised. 

This is one other advantages of using our model. We can model all of the possible ambiguities of all possible types at once. 
\jurek{rephrase or delete}

In the appendix, we give a step-by-step overview over how the algorithm learns the parameters for a simplified example. In the following, we introduce a dataset and learn a model. 
We then show how we can reason with the learned model to model ambiguity. 































==> chaptersPaper/discocat.tex <==

\section{Linguistics and Quantum Circuits}

%*************************
\subsection{The DisCoCat Model}
%*************************

The evolution of language learning models in the past few years has been ... 

The nature of language being both compositional and distributional is reflected by the DisCoCat model \citep{discocat}. 

\jurek{search for good introduction sentences to discocat}


The DisCoCat model is built on the framework of Category Theory, which unifies the mathematical structures of grammar and meaning by identifying both the Pregroup grammar \citep{pregroups} as well as Vector spaces and linear maps between them as \textit{compact closed categories}. The introduction of a \textit{functor} between these categories then maps grammar reductions in the grammar category to composition of tensors, whose order depends on the grammatical type assigned in the Pregroup formalism. 

The compositions of these tensors in the DisCoCat model become \textit{tensor networks}, where the implementation using \textit{quantum circuits} is a natural choice. 
Indeed, one can instead of using the category of vector spaces and linear maps between them, use the category of Hilbert spaces and linear maps between them, \texttt{FHilb}, fitting the choice of quantum circuits as an implementation method even better. 

The DisCoCat framework orginally evolved from \textit{categorical quantum mechanics} \citep{discocat}, but has been mostly adapted to dealing with tensors, not least because of 

\jurek{because of what?}

In the Pregroup grammar \citep{pregroups}, words are assigned types $p$ corresponding to their grammatical function. 
The two reduction rules: 
\begin{equation}
    p^l \cdot p \rightarrow 1 \quad \qquad p \cdot p^r \rightarrow 1
\end{equation}
guide the composition of words in a sentence, where each word is assigned one type. 
Consider the sentence \texttt{Alice plays guitar}: assigning a type to each of the words (\texttt{Alice} $\rightarrow n$, \texttt{plays} $\rightarrow n^r \cdot s \cdot n^l$ and \texttt{guitar} $\rightarrow n$), following their grammatical function, and applying the reduction rules, we get:
\begin{equation*}
    \texttt{Alice plays guitar}: \quad \quad n \cdot \big( n^r \cdot s \cdot n^l \big) \cdot n \rightarrow 1 \cdot s \cdot 1 \rightarrow s
\end{equation*}
indicating that this sentence is indeed grammatical. 
In general, compact closed categories have a diagrammatical language associated to them, called \textit{string diagrams}. In this language, grammar reductions as above can be presented as follows: 

\ctikzfig{alicePlaysGuitarPregroup}

Using a \textit{functor}, one can map derivations in the compact closed category \texttt{Preg} to compositions of tensors in the compact closed category \texttt{FVect}. 

As mentioned above, the ranks of the resulting tensors correspond to the grammatical type assigned in \texttt{Preg}. 
Sticking with our example, \texttt{Alice} and \texttt{guitar} are assigned rank-one tensors (vectors) in the \textit{noun space}, labelled $N$: $\Vec{v}_{\texttt{Alice}}, \Vec{v}_{\texttt{guitar}} \in N$. 
And the transitive verb \texttt{plays} is a rank three tensor: $\Vec{v}_{\texttt{plays}} \in N \otimes S \otimes N$, where $S$ is denoted the \textit{sentence space}. 

Again, the composition of these tensors can be captured by string diagrams, where the boxes represent tensors and the wires represent how these tensors are composed: 

\ctikzfig{meaningGrammar}

These diagrams are the basic language that this paper is written in. 

\jurek{mention that this is a very rough introduction, give citations}


==> chaptersPaper/introduction.tex <==
How does one obtain the meaning of a sentence given the meaning of the words that make it up? This question central to Natural Language Processing is addressed in the DisCoCat (DIStributional COmpositional CATegorical) model of meaning introduced by \citet{discocat} by modelling words as tensors and mapping grammar derivations to composition rules of tensors.

\jurek{mention diagrams and that the diagrams can be mapped to quantum circuits -> qnlp! }


In the DisCoCat framework, words are modelled as quantum states, whose composition is governed by a grammar logic called Pregroup \citep{pregroups}.
The connection between the grammar (Pregroup) and Hilbert spaces together with linear maps between them is provided via \textit{Category Theory}. 
Grammar as well as Hilbert spaces and linear maps between them are identified as \textit{Compact Closed Categories}, called \texttt{Preg} and \texttt{FHilb}, respectively. Grammar derivations in \texttt{Preg} are mapped to the composition of Quantum States in \texttt{FHilb} via a \textit{Functor}. 

The field subsequently arising is called Quantum Natural Language Processin (QNLP).

The concept of a density matrix in physics is applied in numerous cases adressing ambiguity and hierarchy \jurek{search for the formal word}
The use of density matrices in QNLP is not a novel one. 
\citet{densMat} use density matrices to ..., while ... use density matrices for 
\jurek{collect applications for density matrices}. 
Indeed, although not formally explicitly mentioned, the existence of a word being represented by a density matrix in a sentence results in the sentence being represented by a density matrix as a probability distribution over the possible realisations of the sentence. 



In this paper, we propose a way of modelling the syntactic structures in DisCoCat diagrams using density matrices. We subsequently introduce a probability distribution over diagrams, in which diagrams are differently wired, corresponding to different ways of interpreting the sentences represented by the diagram.

This approach finds applications in Lexical Ambiguity. Consider for example the sentence: 
\begin{displayquote}
    \texttt{The dog hunts the cat. It is fast.}
\end{displayquote}
There are two possible grammatical readings to the sentence: 
\begin{displayquote}
    \texttt{The dog hunts the cat. The dog is fast.} \newline 
    \texttt{The dog hunts the cat. The cat is fast.}
\end{displayquote}
The diagrams and the concepts of modelling these different readings have been established by \citet{pronounResolution}, using \textit{Lambek Calculus with soft modalities}. \jurek{with a connection to Fock Spaces. }

In order to briefly motivate the problem, consider a human information processing approach to this pair of sentences. We consider both the \texttt{dog} and the \texttt{cat} to be possible readings, until further information is encountered. 
The goal for our research was to mimic this aspect of the human information processing approach, in that probabilites are assigned to the different sentences and subsequently a probability distribution over the different setnences is introduced. 

The contribution of this work is the introduction of a probability distribution \textbf{over} these two possible readings. 

This probability distribution emerges as a probalbiilty distribution over different functions associated with some \emph{source-word}, acting on the other words in the sentence. 
Indeed, the source word becomes a process that acts on the other words in the sentence. 

We present the density matrix representing the source word as a process, which can be constructed as the tensor products of individual density matrices acting on  one or two qubits only. 

\jurek{or maybe say: We want to associate one function with every reading that we can create a probability distribution over. This function is related to words, and will be in some cases replaced with the words. But the function is }


We can say that this ambiguity, represented by the source word, is acting on the relevant words in the sentence. 
\jurek{however, to be able to connect the words together in the right way, the ambiguous word acts on all!!!!! words in the sentence. }

We model the composition of the words in the sentences themselves as quantum probability distributions (density matrices), and show that a model trained on meanings of sentences can recover the syntactic copying structure without being explicitly learned on it. 


\jurek{We view the ambiguity as a probability distribution. And the beatiful thing is that we can recover the correct reading not by training the model explicitly, but by training the model generally, and then reason about different cases of ambiguity. We could, in theory, use this model to use semantics, rather than syntax, to choose if a sentence is a subject - or an object relative clause. }


\jurek{HOw can WE EXPRESS THIS NOTION OF: BOTH COULD BE POSSIBLE, USING THE FRAMEWORK THAT WE HAVE??? using density matrices. }


\jurek{maybe start with, the sentence that solves the problem. then from there say: Where does this come from? }

\jurek{natural question: how can this process of finding the source word be generalised? }



\jurek{In this presentation, we lack genearlisation! This means, we only construct these things very explicitly for explicit examples. We cannot say how these words are generally found. }


\jurek{we show how we can model these ambiguities in the Discocat framework. 
DO THIS BY SHOWING THE RESULTS
we show how this is mapped to quanutm circuits. Now, where exactly these ambiguities come from, one can philosophise. 

BESCHREIB DIE LOESUNG, DANN STELL UEBERLEGUNGEN AN, WOHER DAS KOMMEN KOENNTE. ES IST SCHON SO, DASS immer worter involviert sind, die komplettt durch wires ersetzt werden. DAs kann es sein. 
Aber dann: the man sees the woman on the mountain, da wird nichts ersetzt. 

HIER, NUR SYNTACTICALLY AMBIGUOUS SENTENCES! in diesem paper
}

\jurek{we argue that this presentation is the equivalent to moving from pure states to mixed states in the discocirc framework}


\jurek{VQCs implicitly learn the ability to differentiate between subject and object relative pronouns!! And other things, like ...}


The powerfulness of the model emerges from the fact that this way of modelling ambiguity is closer to how the humand mind works. Using our model, ambiguity can be \textbf{maintained} until further information is acquired. 


The paper is structured as follows. 
Firstly, we identify related work, mentioning in particular work that this piece of research builds on. We present one particulary important paper, whose experiment really emphasises the importance and applicability of the here introduced theory.
We discuss the DisCoCat framework as the basis on which the contributions of this paper will take place. In a next step, we establish the connection of the arising diagrams to \emph{quantum circuits}, which allow for the theory to be put into practice. In this context, the notion of a density matrix and its application in the context of QNLP are discussed. Density matrices are used to model ambiguity in words. This is where our contribution takes place. 
We mention the \emph{DisCoCirc} framework, which models the evolution of text as sentences being density matrices that are continuously updated as the text evolves.

In a next section, we present the shortcomings of the state-of-the-art mechanisms and present a novel way of creating quantum probability distributions to account for these shortcomings.
We explain, using mostly diagrammatic language, the workings of the theory and illustrate the latter by mapping arising diagrams to quantum circuits, followed by a brief study evaluating the proposed model.

We present the workings of the theory both in the DisCoCat, and in the DisCoCirc framework. 



% What follows is an overview over how to deal with ambiguity in the DisCoCat framework by copying information using \textit{Frobenius maps}, subsequently motivating the idea introduced in this paper. 

We then show how to create probability distributions over the different copying mechanisms introduced above.
We do this in the following way: 
We capture the ambiguity in the sentence in a single word (trying to localise the source as well as possible)
We then model the words as morphisms, acting on the rest of the words in the sentence.
Lastly, we model the word as a mixed state, representing a probability distribution over the possible readings that arise from its ambiguous nature. 
We give numerous examples and draw a connection to the DisCoCirc framework \citep{DisCoCirc}, in which the evolution of text is modelled as density matrices acting on other density matrices in so called updating mechanisms. 


We explain how to map this formalism to quantum circuits, and give one detailed example of how one can recover syntactic rules from a parametrised quantum circuit learned on semantics alone. 

We train a model to learn semantics from a newly created dataset, and we demonstrate how to reason with probability distributions over syntax. 


Concretely, there are three contributions to this paper: 
\begin{enumerate}
    \item We introduce a novel way of reasoning with density matrices that allows modelling ambiguity in language as a quantum probability distribution over sentences that possibly contain different syntax
    \item We show how this way of reasoning can be immediately mapped to quantum circuits and thus be evaluated in experiments. We briefly conduct a small experiment  
    \item We relate the proposed theory to the \texttt{DisCoCirc} framework \citep{DisCoCirc}.
\end{enumerate}
Ultimately, this model allows us to model how ambiguity over different syntactic connections can be \emph{maintained} and updated using context. 


\jurek{You have to decide on how you want to tell the story. 
Just saying that we can now have a probability distribution over differently syntactic sentences as well? 

}





==> chaptersPaper/practice.tex <==
\jurek{I think everything is already captured by the above practice section}

==> chaptersPaper/quantumComputing.tex <==



\jurek{we relate the discocat model to quantum circuits and we explain the learning process.}

The wonderful thing about the above introduced DisCoCat diagrams is the ability to map them directly to quantum circuits. 
This, in turn, means that the meaning of a sentence can be displayed as a quantum state encoded on a qubit. 


\jurek{mention frobenius, spiders }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Quantum Computing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We briefly introduce concepts from quantum computing, while focussing on the parts highly relevant for the current piece of research. 
For a thorough introduction to quantum computing, consider e.g. \jurek{cite}. 

Firstly, why would the diagrams be mapped to quantum circuits? The answer to that is simple: in doing so, we obtain machine learning models, capable of being trained and capable of predicting sentence meaning. In this work, we will train the arising variational quantum circuits on specific tasks to illustrate what exactly the learning process looks like. 

Because the DisCoCat diagrams as discussed in the above section provide instructions on how tensors are composed, they are tensor networks. 

As \citet{tensorNetworksQML} \jurek{check the cite} argue, there is a direct correspondence between tensor networks and quantum circuits, which means that the DisCoCat diagrams can naturally be mapped to quantum circuits capturing their meaning.
Subsequently, the meaning of words and sentences are encoded onto one or more quantum bits (\textit{qubits}), which are the basic building blocks of quantum computing. 
While a classical bit can only assume the values 0 and 1, the qubit naturally assumes values in between as well: 
\begin{equation}
\label{eq:qubit}
    \ket{{q}} = \alpha \ket{0} + \beta \ket{1}
\end{equation}
where $\ket{q}$ is the quantum state of a qubit, $\alpha, \beta \in \mathbb{C}$ are constants and $|\alpha|^2 + |\beta|^2 = 1$. 
Quantum gates are the basic building blocks of quantum circuits, which capture the algorithms to be executed on the qubits.
Mathematically, quantum gates are represented by unitary matrices $U$, for which: 
\[
    U^\dag U = I = U U^\dag
\]
where the symbol $\dag$ (dagger) indicates the hermitian adjoint.
In the circuit notation, which is the most common notation for quantum algorithms \jurek{check and rephrase}, these unitaries are represented as boxes acting on wires, as in the following example: 

which amounts to doing matrix multiplication of the Unitary matrices with the states of the qubits. 
\jurek{how much quantum computing should I do?}

\textit{Quantum circuits} are sequences of quantum gates. These circuits represent instructions on how to operate on the qubits in the circuit. 

\subsection{From Diagrams to Quantum Circuits}

\jurek{mention tensor networks, ZX-calculus}

As stated above, the meaning of a sentence, captured by a DisCoCat diagram can be represented by a quantum circuit. 
In Quantum Machine Learning (QML), the approach one takes is to map diagrams to parametrised quantum circuit. 
This means that in a quantum circuit representing the meaning of a sentence composed of its constituent words, one particular part of the circuit is modelling the meaning of one particular word of the corresponding sentence. 
In choosing the explicit quantum circuit representation, one has to choose an ansatz, which controls how many qubits the meanings of different words are encoded on. 
Consider the simple example \texttt{Alice plays guitar}, where we choose to model both the sentence space and the noun space on one qubit: 

\jurek{insert parametrised quantum circuit for alice plays guitar}

We see that the circuit is initialised to a composition of different subcircuits, that are all parametrised with different parameters. 
The explicit structure that the parametrised gates are embedded in (a series of Hadamard gates) is due to the choice of \texttt{IQP-}ansatz \citep{iqp}. 

This really shows the compositional nature of this approach. Different parts of the circuit model different words and, reflecting the compositional nature of the approach, the different subcircuits are composed in a means of the Pregroup grammar, resulting in the meaning of the sentence. 


\jurek{stress that, arising from the connection between DisCoCat and Quantum Computing, there arise quantum machine learning models.}



\jurek{eliminated the section for the learning process, just mention the learning process briefly. }

% %*************************
% \subsection{The Learning Process}
% \label{subsec:QC-learningProcess}
% %*************************
\jurek{discuss the difference to a neural network, stress the relation to human learning}


The learning procedure in a QNLP setting is different to the learning procedure in a classical machine learning setting with e.g., neural networks. 

In the learning process, the above mentioned parameters, parametrising the meaning of words, are learned from the meaning of sentences. 
This means that, as argued by \citet{qnlpInPractice}, the learning procedure follows a top-down approach where the meaning of the whole is learned from the meaning of its parts. 

Thus, in the process of learning sentence meaning, the meanings of words are learned (in the very exclusive sentence setting). 

Furhtermore, a word is always parametrised in the same way. The parameters for a word in a given sentence is updated to fit the meaning of the sentence, but it is then updated further to fit the meaning of the next sentence it appears in. 
This reflects the compositional nature of the learning process. 












%*************************
\subsection{Density Matrices and Mixed States}
%*************************


\jurek{from thesis: density matrices, entropy and fidelity, and directly its relation to linguistic as well. }

% \subsection{Density Matrices}
% \label{subsec:QT-densityMatrices}
 
Density matrices are of central interest in the context of QNLP due to their ability to, on the one hand, model ambiguity in language and on the other hand, capture hierarchy between word meanings. Density matrices find many applications in the field of QNLP: 
\citet{meaningUpdatingDensMat} introduce updating techniques for density matrices representing words. \citet{word2dm} introduce a new framework called \texttt{word2DM} to learn density matrix representations for words using neural networks. This framework is an extension to the \texttt{word2vec} approach (introduced in section \ref{ch:amplitudeEncoding-word2vec}), which learns word embeddings with a neural network. Based on this idea, \citet{Bruhn_2022} learns density matrix representations using quantum circuits to represent density matrices. 
% Density matrices are an ongoing field of research in QNLP. 
In section \ref{subsec:densityMatricesInQNLP} we explore density matrices in the context of QNLP, and subsequently introduce the category of completely positive maps. In this section, we give a brief introduction to the density matrix and its properties. 

The density matrix is a positive semi-definite, hermitian operator $\rho$ with trace one that represents a probability distribution over pure quantum states. The density matrix can represent mixed states, while the common state vector can only represent pure states. 
A density matrix $\rho$ is generally defined as: 
\begin{equation}
    \rho = \sum_i p_i \ket{\psi_i} \bra{\psi_i}
\end{equation}
for a series of pure quantum states $\ket{\psi_1}, \ket{\psi_2}, \ldots$ and corresponding probabilities $p_1, p_2, \ldots$.
Consider some observable $A$ in the system described by $\rho$. We obtain the expected value of $A$ in this system as: 
\begin{equation}
    \langle A \rangle = \Tr \big(\, \rho \, A \,\big)
\end{equation}
where, in contrast, the expectation value for the pure state case is described by: \[ \langle A \rangle = \braket{ \, \psi \, | \, A \, | \, \psi \, }\]
where $\ket{\psi}$ is some pure state. As we saw in the spectral theorem, every operator $A$ in quantum mechanics can be decomposed as:
\begin{equation}
    A = \sum_i p_i \ket{\psi_i} \bra{\psi_i}
\end{equation}
where the $\ket{\psi_i}$ are the eigenvectors of $A$. As shown by \citet{shjw} in the Schrödinger-HJW theorem, this state is not unique:
consider some finite dimensional Hilbert space $\mathcal{H}_1$ and some mixed state $\rho$ defined on $\mathcal{H}$. 
According to the Schrödinger-HJW theorem, the state $\rho$ can be \textit{purified}: it can be represented by a partial trace of a \textit{pure state} in a composite Hilbert space $\mathcal{H} = \mathcal{H}_2 \otimes \mathcal{H}_2$. 
Mathematically speaking, this means that there always exists a pure state $\psi_{12}$, for which: 
\begin{equation*}
    \rho = \Tr_2 \big( \, \ket{\psi_{12}} \bra{\psi_{12}} \, \big)
\end{equation*}
where $\Tr_2$ is the \textit{partial trace} over Hilbert space $\mathcal{H}_2$. This density matrix is called a \textit{reduced density matrix}. This will become relevant in chapter \ref{ch:densityMatrices}, where one can explicitly construct mixed states \emph{from} pure states by taking the partial trace, which is the \textit{discarding effect} in the framework of quantum picturialism introduced in section \ref{subsec:quantumPicturialism}.  
The process of \textit{discarding} a qubit amounts to tracing out its corresponding Hilbert space, as we will elaborate on further in section \ref{subsec:quantumPicturialism}.  
% Consider some entangled state $\rho_{12}$ in the tensor-product space $\mathcal{H}_1\otimes \mathcal{H}_2$.
% If we want to describe only one subsystem $\mathcal{H}_1$ or $\mathcal{H}_2$, we take the partial trace over the Hilbert space $\mathcal{H}_2$ and end up with the reduced density matrix $\rho_1 = \Tr_2(\rho_{12})$.
% The process of tracing out $\mathcal{H}_2$ amounts to{forgetting} the degrees of freedom corresponding to subsystem $\mathcal{H}_2$, by which we \textit{discard} the second qubit. 

There are measures quantifying the {mixedness} of some state $\rho$. One of these measures is the \textit{Purity}. 
\begin{definition}[\texttt{Purity}]
\label{def:purity}
    The \textit{purity} $\gamma$ of a quantum state $\rho$ is: 
    \begin{equation}
        \label{eq:purity}
        \gamma = \Tr{\rho^2}
    \end{equation}
    where $1/{d} \leq \gamma \leq 1$, with $d$ the dimension of the corresponding Hilbert space. 
\end{definition}
The {purity} of a quantum state indicates how \textit{pure} it is, meaning the more mixed the state, the lower its purity.   
The lowest possible value, corresponding to some quantum circuit consisting of $N_q$ qubits, is $1 / 2^{N_q}$.
Another measure to quantify the mixedness of a quantum state $\rho$ is the \textit{Von Neumann Entropy}. 


\jurek{don't have a designated section for the Von Neumann Entropy, just mention it briefly. }
% \subsection{The Von Neumann Entropy}
\label{subsec:vonNeumannEntropy}
Similar to  purity, the Von Neumann entropy captures the \textit{mixedness} of a given quantum state. The Von Neumann entropy can be understood as the quantum theoretical equivalent to the \textit{Shannon entropy} \citep{shannon1948mathematical}. In information theory, the {Shannon entropy} of some variable is a measure of \textit{uncertainty} or amount of \textit{information} in this variable. The Shannon entropy in information theory is defined as: 
\begin{equation}
    \label{eq:shannon}
    H_\text{Shannon} = - \sum_{x \in \mathcal{X}} p(x) \log_2 p(x)
\end{equation}
where $x$ is a discrete random variable in the set $\mathcal{X}$ and $p(x) \in [0,1]$. 
% In a physics context, we use the entropy defined as: 
% \begin{equation}
%     \label{eq:physicsEntropy}
%     S = -k_\text{B} \sum_i p_i \ln p_i
% \end{equation}
% where $p_i$ is the probability corresponding to a physical system being in some state, and $k_\text{B}$ is Boltzmann's constant. 
The Von Neumann entropy \citep{vonNeumann} is defined as: 
\begin{equation}
\label{eq:vonNeumannEntropy}
    S_\text{Von Neumann} = - \Tr \big( \, \rho \ln \rho  \, \big)
\end{equation}
where $\rho$ is a density matrix describing a quantum physical system. 
As discussed above, the density matrix $\rho$ can be written in terms of its eigenvectors as: 
\[
\rho = \sum_i p_i \ket{\psi_i} \bra{\psi_i}
\]
so that: 
\begin{equation*}
    S_\text{Von Neumann} = - \sum_i p_i \ln p_i
\end{equation*}
since 
\begin{equation}
    \Tr  \rho  = \sum_i p_i
\end{equation}
where $p_i$ are the eigenvalues of $\rho$ so that the eigenvalues of $\rho \ln \rho$ are $p_i \ln p_i$ so that: 
\begin{equation}
    \Tr ( \rho \ln \rho ) = \sum_i p_i \ln p_i
\end{equation}
% One important difference between the Shannon- and the Von Neumann entropy is that, while the Shannon entropy is bounded between 0 and 1, t
The Von Neumann entropy lies between 0 (for a pure state) and $\ln (d)$ for $d$ the dimension of the corresponding Hilbert space. 
In this work, we use the Von Neumann entropy to reason about the information and uncertainty captured in certain quantum circuits representing words and sentences. 
In section \ref{subsec:densityMatricesInQNLP}, we introduce methods to compare density matrices to each other, e.g., the \textit{quantum relative entropy} or the \textit{fidelity}. 


\jurek{This is Density matrices in a QNLP context}
\jurek{I emilinated this section, connect it to the above directly. }

% \subsection{Density Matrices in QNLP}
% \label{subsec:densityMatricesInQNLP}

% As mentioned in section \ref{subsec:QT-densityMatrices}, density matrices prove useful in the field of QNLP. 
% In the following, we discuss their use in the current QNLP literature \citep{coecke2020foundations}. The properties of density matrices discussed here will be immediately useful in the implementation in chapter \ref{ch:taskOne}.
% % To include features of language like hierarchy or ambiguity, the density matrix is suited as a model representing these things. 
% We present a category in which they live (the category of completely positive maps) and we explain methods to compare and interpret density matrices to each other. We use measures like the \textit{Von Neumann entropy} (equation \ref{eq:vonNeumannEntropy}) and \textit{purity} (definition \ref{eq:purity}), which are measures of the amount of (quantum) information stored in density matrices. 

\jurek{briefly mention the cateogry in which they live}
 
As stated above, density matrices represent ambiguity about the state that a given system is in. 
Firstly, consider the example of the word \verb|bank|. This could be a \texttt{financial institute}, it could be a \texttt{river bank}, it could be a \texttt{computer memory bank}. There are several meanings for the same word, which makes it \textit{ambiguous}. To capture the {ambiguity} in this word, we introduce the density matrix as a probability distribution over the pure states capturing the meanings of the words. This makes the density matrix a mixed state $\rho_\text{bank}$, i.e. a probability distribution over pure states as: 
\begin{equation*}
    \begin{split}
        \rho_{\texttt{bank}} &= \alpha \, \ket{\texttt{bank}_{\texttt{river}}} \bra{\texttt{bank}_{\texttt{river}}} \\
                    &+ \beta \, \ket{\texttt{bank}_{\texttt{finance}}} \bra{\texttt{bank}_{\texttt{finance}}} \\
                    &+ \gamma \,\ket{\texttt{bank}_{\texttt{memory}}} \bra{\texttt{bank}_{\texttt{memory}}}
    \end{split}
\end{equation*}
where $\alpha, \beta, \gamma \in \mathbb{C}$ and $\alpha + \beta + \gamma = 1$.
Words in context, represented by other quantum states, can then disambiguate the word represented by the density matrix. 
On a lower level, all the pure states $\ket{\texttt{bank}_{\texttt{river}}}, \ket{\texttt{bank}_{\texttt{finance}}}, \ldots$ are represented in terms of some basis states $\texttt{word}_i$, similar to the context-words mentioned in section \ref{subsec:distributionalSemantics}. 
% They are in a superposition of these pure states. 
If a word similar to the word \verb|riverbank| appears in context, like \verb|fish|, this disambiguates the word \verb|bank| modelled by the density matrix $\rho_{\texttt{bank}}$ above. 

% Concretely, consider the above example, where the words \texttt{riverbank, financial bank} and \texttt{computer memory bank} are three basis words of a vector space. 
% Consider now the noun \[\ket{\texttt{fish}} = 0 \cdot \ket{\texttt{bank}_{\texttt{finance}}} + 0 \cdot \ket{\texttt{bank}_{\texttt{memory}}} + 1 \cdot \ket{\texttt{bank}_{\texttt{river}}}\] 
% The disambiguation effect the word \texttt{fish} has on the word \texttt{bank} is: 
% \begin{equation*}
% \begin{split}
%     \rho_{\texttt{bank}} \circ \ket{\texttt{fish}} = \, &\big( \alpha \, \ket{\texttt{bank}_{\texttt{river}}}  \bra{\texttt{bank}_{\texttt{river}}} \\&+ \beta \, \ket{\texttt{bank}_{\texttt{finance}}} \bra{\texttt{bank}_{\texttt{financial}}} \\&+ \gamma \, \ket{\texttt{bank}_{\texttt{memory}}} \bra{\texttt{bank}_{\texttt{memory}}}\big) \\  \circ \, &\big( 0 \cdot \ket{\texttt{bank}_{\texttt{financial}}} \\&+ 0 \cdot \ket{\texttt{bank}_{\texttt{memory}}} \\&+ 1 \cdot \ket{\texttt{bank}_{\texttt{river}}} \big)     
%     \\
%     &= \alpha \, \ket{\texttt{bank}_{\texttt{river}}}
% \end{split}
% \end{equation*}
% assuming that $\ket{\texttt{bank}_{\texttt{river}}}, \ket{\texttt{bank}_{\texttt{finance}}}$ and $\ket{\texttt{bank}_{\texttt{memory}}}$ form an orthonormal basis, which means that they are orthogonal so that their scalar product yields 0.
% We could also model the word \texttt{fish} as a density matrix \[\rho_{\texttt{fish}} = \ket{\texttt{fish}} \bra{\texttt{fish}} = \ket{\texttt{bank}_{\texttt{river}}}\bra{\texttt{bank}_{\texttt{river}}}\]
% where then: 
% \begin{equation}
%     \rho_{\texttt{bank}} \circ \rho_{\texttt{fish}} = \alpha \, \ket{\texttt{bank}_{\texttt{river}}} \bra{\texttt{bank}_{\texttt{river}}} =  \rho_{\texttt{bank}_{\texttt{river}}}
% \end{equation}
As argued in section \ref{subsec:QT-densityMatrices}, density matrices are series of weighted projection operators, which is an intuitive approach to the above. By composing the density matrices $\rho_{\texttt{fish}}$ and $\rho_{\texttt{bank}}$, we project out the \texttt{fish} part from $\rho_{\texttt{bank}}$, which is \texttt{riverbank}. 
The pure eigenstates of the density matrix (\texttt{riverbank, financial bank, computer memory bank}) are usually themselves made up of more basic words. It is common to train high dimensional vector spaces with around \num{1000} basis words; these vector spaces are called \textit{count-based} vector spaces. They are trained based on so called \textit{context-windows} around the word of interest. We introduce this concept in section \ref{ch:amplitudeEncoding-word2vec}.

The second reason density matrices are useful in QNLP is due to their ability to capture hierarchichal relations between words. 
\jurek{I commented this out, perhaps just refer to Coecke.}
% Consider the words \texttt{pear}, \texttt{fruit} and \texttt{food}. Clearly, every \texttt{pear} is a \texttt{fruit} and every \texttt{fruit} is a type of \texttt{food}. 
% Using density matrices, we can model the three words as: 
% \begin{equation*}
%     \begin{split}
%         \rho_{\texttt{pear}} &= \ket{0} \bra{0} \\
%         \rho_{\texttt{fruit}} &= \ket{0} \bra{0} + \ket{1} \bra{1} \\
%         \rho_{\texttt{food}} &= \ket{0} \bra{0} + \ket{1} \bra{1} + \ket{2} \bra{2}
%     \end{split}
% \end{equation*}
% where we see that, e.g., the density matrix $\rho_{\texttt{food}}$ contains the density matrix $\rho_{\texttt{fruit}}$, capturing the hierarchical property. 
% When it comes to density matrices in diagrams, it is simply a question of interpretation. 

Now, we integrate the density matrix formalism into the DisCoCat framework: the application of the grammar, represented by the function $f_\mathcal{G}$, to the word meanings, now represented by density matrices, transforms from: 
\begin{equation*}
    f_\mathcal{G} \circ (\psi_{w_1} \otimes \ldots \otimes \psi_{w_N}) 
\end{equation*}
where $\psi_{w_1}$ are pure states representing the meanings of words, to:
\begin{equation*}
    f_\mathcal{G} \circ (\rho_{w_1} \otimes \ldots \otimes \rho_{w_N}) \circ f_\mathcal{G}^\dag
\end{equation*}
where $\rho_{w_i}$ are word meanings represented by density matrices. 
Diagrammatically, the transition from the DisCoCat diagrams used up to now, to the DisCoCat diagrams modelling density matrices, amounts to doubling, introduced in section \ref{subsec:quantumPicturialism}.
% Among one of the first advances to introduce density matrices in Natural Language Processing was the work by \citet{firstDMApproach}. 
\jurek{Eliminated the conclusion sentence}
% In conclusion, in QNLP, density matrices are probability distributions over pure states, which themselves represent the meaning of words:
% \[
%     \rho_{\texttt{word}} = \sum_i p_i \ket{\texttt{word}_i} \bra{\texttt{word}_i}
% \]
% These pure states are in superposition of a number of basis (or context-) words:
% \[
%     \ket{\texttt{word}_i} = \sum_{j} \lambda_j \ket{\texttt{basis-word}_j}
% \]
% In the following, we explain the diagrammatic representation of density matrices upon introducing the category of \textit{Completely Positive Maps} (\texttt{CPM}).



\jurek{eliminated quantum relative entropy, and its classical equivalent}

% To quantify distinguishability, \citet{densMat} introduce the \textit{relative entropy} between two density matrices as: 
% \begin{definition}[\texttt{Quantum relative entropy}]
% The \textit{Quantum Relative Entropy} $N(\rho \, ||\, \sigma)$ between two density matrices is defined as:
%     \begin{equation}
%         N(\rho\,||\,\sigma) = \operatorname{tr}(\rho \log \rho) - \operatorname{tr}(\rho \log \sigma)
%     \end{equation}
%     where $0 \log 0 = 0$ and $x \log 0 = \infty$ when $x \neq 0$. 
% \end{definition}
% \noindent
% To understand the notion of \textit{relative entropy}, we present the classical equivalent, known as \textit{Kullback-Leibler} divergence, developed by \citet{klDivergence}.  Consider a probability distribution $P = \{p_1, \ldots, p_N\}$ and another probability distribution $Q = \{ q_1, \ldots, q_N \}$. 
% Following \citet{idyomBoundaries}, the information content $h(q_i)$ after observing the $i$-th event is: 
% \begin{equation*}
%     h(q_i) = - \log q_i
% \end{equation*}
% Consider now the distribution $Q$ to be our assumed probability distribution for $P$. We can capture the assumed average information content of all events in $Q$ as: 
% \[
% - \sum_i p_i \log q_i
% \]
% where the Shannon entropy, introduced above (equation \ref{eq:shannon}) captures the actual average information content: 
% \[
% -\sum_i p_i \log p_i
% \]
% The difference between these two measures: 
% \[
% \sum_i p_i \log p_i - \sum_i p_i \log q_i
% \]
% is what we consider the classical \textit{relative entropy}. It thus measures the {distinguishability} between these two probability distributions. 










\jurek{explain how density matrices can model ambiguity over words, and over sentences but not over differently wired diagrams.}

\jurek{specific words are modelled as probability distributions over different morphisms, yielding the ultimate density matrix}

Of particular interest for this paper is the integration of density matrices into the DisCoCat framework. 

Density matrices are part of a category, too, the category of \textit{completely positive maps} termed \textbf{CPM}. 

String diagrams for quantum states represented by density matrices are drawn \textit{thick}, so that: 

\jurek{transition from thin to thick wires.}

In the furhter course of this work, if a wire is drawn thick, it represents a density matrix. 


We see in the above that density matrices may be used to model probability distributions over \emph{word meanings} or, as a result of plugging in this density matrix in the sentence, over \emph{sentence meanings}. 
However, importantly, we note that the probability distribution over the different sentence meanings is a probability distribution over sentences that are wired in the same way: meaning, they have the same syntax. 
The current state-of-the-art use of density matrices does not involve creating probability distributions over sentences containing different syntax. 

In this work, we illustrate the upside of using density matrices for this task as well, and show in particular how this allows for more general, human-like learning of machines. 







\jurek{The DisCoCirc framework gets its own designated subsection}
\subsection{The DisCoCirc framework}

\jurek{why do we introduce the DisCoCirc framework here? Can we model anything with it that we cannot model with the DisCoCat framework? No. But it helps us illustrate how the mechanism works in a more intuitive manner.}


We present the working of the proposed theory in this work both using the state-of-the-art DisCoCat, as well as the DisCoCirc framework. 
The DisCoCirc framework, proposed by \citet{DisCoCirc} explains a sentence as being a \emph{process} altering the meaning of the words that make it up.

In this work, we will provide this model with explicit representations of sentences altering the meanings of words and, additionally, sentences being probability distributions over how these words are altered. 

Really then, there are two research points that this paper tackles. 
Firstly, advancing the theory of density matrices in the DisCoCat framework to acccount different wirings, and secondly, as starting from the DisCoCirc framework, where we argue that in some cases, it is only the nouns that are dynamic, but in other cases, it might well be verbs or adjectives. 

We will below argue how exactly one can determine which word is dynamic and which other words are static, this involves the concept of \emph{boundary entropy} as suggested by \citet{idyom}.


\jurek{DisCoCirc introduction from my thesis}


In this section, we present \textit{DisCoCirc}, one of the numerous extensions to the DisCoCat framework.
% The DisCoCirc extension has been applied to the language Urdu \citep{englishUrdu}. 
In other approaches, DisCoCat has been applied to translations between languages \citep{discocattranslations}, it has led to the developement of \textit{language circuits}, introduced by \citet{distilling} and there are studies investigating the inner structure of words themselves, breaking them up into even smaller parts \citep{grammarEq}. Furthermore, the DisCoCat framework has been applied to music by \citet{discocatmusic}, subsequently developing \textit{Quanthoven}, a quantum model to compose music. 

% \citet{DisCoCirc} extend the DisCoCat framework to allow for the modelling and composition of \textit{sentence} meanings. 
% Subsequently, the DisCoCirc framework is introduced. 
Similar to DisCoCat, in DisCoCirc, there are different approaches to composing sentences to give a meaning of the whole. A Bag-Of-Sentences model only works for commuting sentences (sentences, for which the order they are read in does not matter) like:
\begin{verbatim}
    Bob does not like Alice.
    A man likes eating mediterranian food.
    The rook is a chess piece.
\end{verbatim}
In the case of non-commuting sentences: 
\begin{verbatim}
    Bob gets up. 
    Bob brushes his teeth. 
    Bob leaves the house. 
\end{verbatim}
some kind of structure is necessary to guide the composition of these sentences to account for the order of time. 
Rather than modelling the interaction of words to give the meaning of sentences, as in the DisCoCat framework, the DisCoCirc framework models the interaction of sentences with each other. 
Following \citet{DisCoCircBook}, text can be seen as \textit{a process that alters the meaning of words}.
The diagram one ends up with when investigating how sentences $\sigma_1, \ldots, \sigma_5$ act on a number of words is depicted in the following (the diagrams in this section are created after \citet{DisCoCirc}): 

\ctikzfig{sentences}
Some nouns are \textit{dynamic nouns} whose meanings are altered by the sentence. These dynamic nouns are modelled by density matrices, whose meaning is continuously updated. 
We will explain this updating mechanism in detail in section \ref{subsec:densityMatricesInQNLP}. However, firstly, {only} nouns can be dynamic, and secondly, only some of these nouns are indeed dynamic. Other words are \textit{static}, which means that their meaning is not updated by other words. However, these words are modelled by density matrices as well, which update the dynamic nouns via mechanisms discussed in section \ref{subsec:densityMatricesInQNLP}. 

There is one aspect regarding the types of words, that is important to note when modelling words as density matrices in the above presented fashion. 
Note that in standard NLP literature, all types of words live in the same vector space. The corresponding representations of the vectors for nouns, adjectives and verbs are: 
\ctikzfig{OneSpace}
where the \texttt{verb} could be transitive, intransitive or ditransitive. We see that this interpretation of words as vectors does not allow grammar formalisms or words living and interacting in different spaces. 
In the DisCoCat framework, the adjective is a matrix $N \otimes N$, while the transitive verb is a rank-three tensor $N \otimes S \otimes N$, where $S$ is the sentence space, and the noun is a vector in the noun space $N$. 

In the DisCoCirc framework, the sentence type is made up of two noun types, which means that the sentence space is the tensor product space $N \otimes N$. Consider the sentence: 
\[
\texttt{Alice likes Bob}
\]
This is:

\ctikzfig{aliceLikesBobDisCoCat}
where the verb, as \citet{coecke2020foundations} argue, has an internal wiring as: 

\ctikzfig{verb}
% which reduces the exponential blowup encountered when investigating verb dimension. 
where the notation using the \enquote{$*$} is explained in the following. 
% We will see how to understand verbs and adjectives to be \textit{imposed} onto noun states shortly. 
% First, consider the verb \texttt{likes} from the diagram above. 
In the DisCoCat framework, the verb \texttt{likes} lives in a vector space $\mathbb{C}^2 \otimes \mathbb{C}^{2k} \otimes \mathbb{C}^2$ for $k$ the dimension of the sentence space. 
What the above model suggests is that the verb actually lives in a lower dimensional vector space $\mathbb{C}^2 \otimes \mathbb{C}^2$ which lets us model verbs in practice (e.g., for a noun space of 1000 dimensions, the verb space has a dimension of $1000^2 = 10^6$ rather than $1000^3 = 10^{9}$ for $k=1$). This lower-dimensional representation of the word \texttt{likes} is labelled $*\texttt{likes}*$. 
In fact, what seems to be a hack turns out to be a feature intrinsic to quantum theory, which can be used to reinterpret the information flow in these diagrams where the verb is now considered to imply a relationship on the involved nouns. 

\ctikzfig{verbImposeNoun}
Adjectives can also be considered features imposed onto nouns as: 

\ctikzfig{adjdot3}
These images display the connection to quantum circuits. The states \texttt{Alice}, \texttt{*plays*} and \texttt{guitar} are prepared states encoded on (sets of) qubits. We will further explain this connection, together with the translation of these diagrams to quantum circuits, in section \ref{subsec:sentencesToQC}. 
% The methodologies developed in this work are developed in the DisCoCat framework and integrated into the DisCoCirc framework subsequently. 
In chapter \ref{ch:SyntaxDistribution-oldmanship}, besides dynamic nouns, we suggest the concept of a \textit{dynamic verb} as a density matrix modelling a verb, whose meaning is updated in the process of working through the text.  
% And meanings of sentences, represented by density matrices can be compared to each other using the trace $\Tr ()$:
% \ctikzfig{sentenceTrace}
% This representation of the trace is explained in \ref{subsec:quantumPicturialism}. 
% We will further discuss the modelling of words as \textit{evolving} density matrices in chapter \ref{ch:implementation}. 


\jurek{but the meaning updating of density matrices does not get a subsection!}

% \subsection{Meaning updating of these Density Matrices}


Because we apply this concept to the meaning of \textit{sentences}, modelled by density matrices, being continuously updated upon encountering further text, we give a short explanation about the state-of-the-art methodology of updating density matrices in QNLP. The following discussion is based on \citep{meaningUpdatingDensMat}. 
\citet{meaningUpdatingDensMat} consider the fact that meaning evolves in the course of a text and thus, using the DisCoCirc framework introduced above, model nouns as \textit{wires} rather than states. Thus, they suggest the sentence type be the same as the type of the incoming nouns. 
This is illustrated for the example sentence \texttt{Bob bites Alice} as: 

\ctikzfig{bobBitesAlice}
Note that this idea is closely related to the concepts discussed in section \ref{subsec:extensionsDisCoCat}, where the DisCoCirc model is presented. In this model, we elevate the concepts from section \ref{subsec:extensionsDisCoCat} to density matrices and explain the concept of a \textit{Dynamic Noun}, introduced in the DisCoCirc framework. Since we are working with density matrices here, we draw all the involved boxes and wires doubled, since the boxes and the wires represent density matrices, as reasoned in section \ref{subsec:quantumPicturialism}. 
In this way, the evolution of the meanings of \texttt{Alice} and \texttt{Bob} in the sentence pair:  
\[
\texttt{Bob fears Alice. Bob bites Alice.}
\]
looks as follows: 
\ctikzfig{bobFearsBobBites}
Indeed, the notion of nouns that appear in context with our density-matrix wires is re-established as a \textit{feature} being imposed on the \texttt{Bob}-wire: 

\ctikzfig{bobDog}
where the operation that composes these two density matrices is indicated by a gray dot. Next, we discuss the nature of this grey dot. Imposing such a feature onto a density matrix would work via Projectors $P_\text{dog}$ as: 
\begin{equation*}
    P_{\texttt{dog}} \circ \rho_{\texttt{bob}} \circ P_{\texttt{dog}}
\end{equation*}
and because every projector is a density matrix \citep{meaningUpdatingDensMat}, we can illustrate the feature \texttt{dog} being imposed on \texttt{bob} as the interaction of two density matrices via the grey dot:
\ctikzfig{bobIsADog}
\citet{meaningUpdatingDensMat} argue that spiders, due to their commutativity, cannot take the place of this gray dot. As a demonstration, consider the sentence: 
\begin{displayquote}
    \texttt{Bob gets up and goes to work.}
\end{displayquote}
If spiders were the composition methods of $\rho_{\texttt{gets up}}$ and $\rho_{\texttt{goes to work}}$ that are imposed onto the state $\rho_{\texttt{Bob}}$, there would be no way to differentiate between the sentences: \[\texttt{Bob goes to work and gets up.}\] and \[\texttt{Bob gets up and goes to work.}\] 
Consequently, due to the commutativity of spiders, they are not a suitable candidate for the grey dot. 

Rather, \citet{meaningUpdatingDensMat} introduce two other mechanisms: the \textit{Fuzz} \citep[originally introduced by][]{DisCoCirc, fuzz} and the \textit{Phaser} \citep[originally introduced by][]{phaser1, phaser2, phaser3}. Both fuzz and phaser are guitar pedals, which are also defined by \citet{meaningUpdatingDensMat} as the mathematical composition symbols. We choose to represent the Fuzz using the symbol {'$\sharp$'} and the Phaser using the symbol {'$\flat$'}.
% The \textit{fuzz} and \textit{phaser} are defined in the following. 

\begin{definition}[\texttt{Fuzz}]
\label{def:fuzz}
    The \textit{fuzz} $\sharp$ is defined as the following operation between density matrices $\sigma$ and $\rho$:
    \begin{equation}
        \rho \, \sharp \, \sigma = \sum_i x_i \, \Big(P_i \circ \rho \circ P_i\Big) \qquad \qquad \text{with}\quad  \sigma := \sum_i x_i P_i
    \end{equation}
\end{definition}
\noindent
The {fuzz} can be diagrammatically displayed as: 

\ctikzfig{fuzz}
% \begin{equation}
%     \begin{split}
%         \rho \, \sharp \, \sigma &= \sum_i x_i (P_i \circ \rho \circ P_i) \tabto{1000mm}  \text{with}\quad  \sigma := \sum_i x_i P_i \\
%         \rho \flat \sigma &= ( \sum_i x_i P_i ) \circ \rho \circ ( \sum_j x_j P_j ) \tabto{25mm} \text{with} \quad \sigma := \sum_i x_i^2 P_i \\
%     \end{split}
% \end{equation}
\begin{definition}[\texttt{Phaser}]
\label{def:phaser}
    The \textit{phaser} $\flat$ is defined as the following operation between density matrices $\sigma$ and $\rho$:
    \begin{equation}
        \rho \, \flat \, \sigma = \Big( \sum_i x_i P_i \Big) \circ \rho \circ \Big( \sum_j x_j P_j \Big) \qquad \qquad \text{with} \quad \sigma := \sum_i x_i^2 P_i
    \end{equation}
\end{definition}
% \begin{alignat*}{2}
%     \rho \, \sharp \, \sigma &= \sum_i x_i \Big(P_i \circ \rho \circ P_i\Big)&\text{with}\quad  \sigma := \sum_i x_i P_i \\
%     \rho \, \flat \, \sigma &= \Big( \sum_i x_i P_i \Big) \circ \rho \circ \Big( \sum_j x_j P_j \Big) \qquad \qquad & \text{with} \quad \sigma := \sum_i x_i^2 P_i \\
% \end{alignat*}
\noindent
The {phaser} is diagrammatically:

\ctikzfig{phaser}
The application of either the fuzz or the phaser to update the meaning of density matrices is not a trace preserving operation. This means that the resulting density matrices are not normalised, which one has to ensure manually. 
The concept of updating the meaning of density matrices in this way lays a foundation for our contribution in chapter \ref{ch:SyntaxDistribution}, where we model the meaning of sentences as a probability distribution over different wirings of DisCoCat diagrams to account for ambiguity in language. 
% In this work, we will update the meaning of density matrices. However, we will do it in a way where \textit{sentences} are density matrices. The meaning of these sentences is then updated upon encountering further sentences. 
% The work presented here, done by \citet{meaningUpdatingDensMat} works on the level of \textit{words} being density matrices. 
% \jurek{mention where the fuzz and phaser will be relevant in this work and mention that the resulting density matrices are not normalized.}



























==> chaptersPaper/relatedWork.tex <==
\jurek{you want to tell a story here that is two fold, or three fold. 
Firstly, \citet{pronounResolution} and perhaps \citet{relPronCoecke}. 
Secondly, the simple motivation of teaching a machine how to think like a computer. 
Thirdly, DisCoCirc. 
}


Mention the papers that exploit density matrices as ways to reason about entailment (food fruit apple) and hierarchy and ambiguity (bank).

\jurek{stuart, etc. oxford papers.}

We introduce further ways of reasoning about information flow between words in a sentence. 
\citet{DisCoCirc} introduces a way of reasoning about a sentence as a \textit{process that changes the meanings of words}. 

\jurek{talk about discocirc, and the upcdating of density matrices via Fuzz, Phaser}


% Modelling lexical ambiguity, gijs and pronounresolution. There are others, draw the connection. 
% Try to keep it in the pregroup formalism. 
% \cite{Wijnholds_2020}

The ways to reason about and deal with lexical ambiguity presented in this paper have partially been developed by \citet{Wijnholds_2020}, \citet{pronounResolution}. 


The research that the current research is heavily based on is that by \citet{discocat}, which introduce the mathematical framework that allows to model linguistic meaning in terms of quantum states. 

The application of density matrices to account for ambiguity is not a novel approach and ... 

In this paper, we model certain words as density matrices: probability distributions over connecting the other words in a sentence in different ways. 
The scheme after which the word of interest is selected is currently the executor's task. However, in future work we hope to be able to automate this process using bounday entropy, as used in the IDyOM framework \citep{idyom}. 

A particularly important piece of research is that of \citet{pronounResolution}, because we argue that what they explicitly train a model to do can be a result of implicitly training a model on a broader task, and then recover this effect (that \citet{pronounResolution} explicitly trained the model on) from the very broad, basic model. This really illustrates the contribution here. 













==> chaptersPaper/syntaxAmbiguity.tex <==


\subsection{Problem Statement}

\jurek{motivate the problem. Explain the problem using the sentence: the dog broke the vase. It was clumsy. Use this example to explain \citet{pronounResolution} work in more detail}


Consider the pair of example sentences \citep[after][]{pronounResolution}: 
\[
\texttt{The dog broke the vase. It was clumsy.}
\]
There are, on third glance, three readings to this sentence. Consider the two readings of either the dog or the vase being clumsy for simplicity reasons. 
A human mind will likely choose one option over the other in the process of processing information. Upon reading the sentence, we are aware that both the \texttt{dog}, as well as the \texttt{vase} can be clumsy. However, the \texttt{dog} being clumsy is the more likely reading: we assign probabilities to the individual readings, subsequently creating a probability distribution over the two readings. 

We want to, driven by the goal of making machines creative, be able to model this process of processing information using (an extension to) the existing DisCoCat framework and its relation to density matrices. 

Note that, if the sentence were: 
\[
\texttt{John likes the queen.}
\]
we are already model this process of having a probability distribution over what queen \texttt{John} likes. It could be the chess piece, or it might be the queen of England. 
Note however the difference to the sentence above, in which it is not clear what noun the word \texttt{it} relates to. 

In short, we will be able to extend the extent to which we are able to model ambiguity in language, so, conrcretely, we will be able to move from 

\jurek{diagram for john likes the queen.}

to: 

\jurek{diagram for dog broke vase}

where, in the latter case, the density matrix describes a probability distribution over different ways of connecting words to each other. 
The \emph{internal wirings} coming along with this theory will be discussed in detail in the following. 

In this, we give a concrete account of how a sentence is a \emph{process} that alters the meaning of the words that make it up - directly connecting our proposed mechanism to the DisCoCirc framework. 
In our framework, individual words can be understood as dynamic words that are altered by the sentences which, in turn, are themselves \emph{mixed states} updating the meaning of the dynamic words.








\subsection{The Idea}



\jurek{and this way of presenting it is not the best, I believe.}


The presentation of the theory itself is structured as follows. 
We explain, always keeping in mind the model of a sentence being a \emph{process} altering the meaning of the parts that make it up, how we can view this in terms of the DisCoCat framework and, in particular, how we can create a probability distribution over different realisations of this sentence. 

We give numerous examples involving both the DisCoCat, and the DisCoCirc framework, and in the following, we explain how the presented theory can be mapped to a quantum circuit, representing exactly this probability distribution. 



% We give a short outline of the general procedure of creating a probability distribution over diagrams containing different syntax. 
% As in the cases seen in chapter \ref{ch:densityMatrices}, individual words are modelled as density matrices. In contrast to these words being simple nouns, as e.g. in the case of the word \texttt{bank}, discussed in detail in section \ref{subsec:densityMatricesInQNLP}, these words have {internal wirings}, which results in the ultimate diagrams representing the sentences being wired differently. This means that the ultimate diagrams describe sentences with different syntax. 
% We explain the procedure in the following sections, guided by the general series of steps provided in the following. 
% \begin{enumerate}
%     \item Starting from a sentence containing ambiguity, such as the sentence \[\texttt{the man sees the woman on the mountain.}\]
%     discussed in the next section, we {localise the source} of ambiguity. This means that we try to find a \textbf{general form of the diagram}, in which the word or phrase causing the ambiguity is modelled as a general state that interacts with the states of all other words in the sentence. The motivation behind this step is that we want to reduce the ambiguity in the diagrams to an ambiguity over a series of \textbf{instructions} that can be carried out on a quantum computer. 
%     \jurek{mention that this general form of the diagram will immediately be connected to the DisCoCirc framework}
%     \item From this general diagram, we identify the \textbf{internal wiring} of the word or phrase causing the ambiguity. This means that we search for the possible diagrammatic representations for the respective ambiguous word that, when plugged into the general diagram, give the possible readings of the overall sentence. 
%     \item We then regard the word causing the ambiguity as a \textbf{probability distribution} over the possible internal wirings, subsequently modelling the word as a density matrix, where each internal wiring is modelled by a pure state. 
%     Plugging in this probability distribution over the different wirings into the most general diagram results in the diagram representing the sentence itself being a probability distribution over the digrams modelling the possible readings of the initial sentence (this is related to the density matrices addressed in chapter \ref{ch:densityMatrices}, where the process of forgetting words yields probability distributions over the sentences, or the model's predictions themselves. However, in the current example, these words in the respective sentences are wired differently).
%     \item As a last step, the states can be regarded as \textbf{morphisms} acting on the states representing the respective words in the sentence. In choosing this representation of the ambiguous words, we can develop a very straight-forward mapping for this concept to \textbf{quantum circuits}. The main difference to the experiments in chapter \ref{ch:densityMatrices} is that the probability distribution is now not only over the \textbf{meaning} of a word, but the \textbf{function} of a word in the context of information flow in the sentence.
%     \item We map the diagram to a quantum circuit using the example circuit presented below. 
% \end{enumerate}
% In the following sections, we illustrate the working of this framework in detail, using explicit examples. We address limitations, and we explain the mapping to quantum circuits, followed by a small experiment to illustrate the framework's abilities using language data.

The idea is given above. We model, e.g. the sentence 
\[\texttt{The dog broke the vase. It was clumsy}\]
as a probability distribution. 
We start by investigating this type of ambiguity. We use quantum circuits to create a probability distribution over different ways of manipulating words. 
This circuit is: 

\jurek{perhaps already show the simple circuit}

where either O1 or O2 is executed due to ... 

we can understand these operations as ways to connect words in the sentence, and I will show you how. 

Use the general sentence structure \[\texttt{Subject verb object, it verb* adjective.}\]
and map it to a quantum circuit. 
\jurek{mention the CCNOT gate earlier in the process}

The \texttt{CCNOT} gate allows us to control a \texttt{CNOT} gate and thus control an operation that connects words to each other in different ways.

Now, to relate this circuit to a general sentence, I give the following diagram: 

\jurek{diagram of prob dist}

And this type of diagram comes about due to the two different wirings that we obtain: 

\jurek{prob dist}

Now, a natural question to ask is: how does the ambiguity enter the sentence, where is it created? 
Firstly, we as humans always know where ambiguity is created, so we can - for every sentence individually - state what word is the source of ambiguity (the word \texttt{it} in the example above). 
In order to explore where this ambiguity could come from, we present another example: 

\jurek{does too example, Gijs}

And another one 

\jurek{the on-mountain example}

We see that, for all of these different cases, we find words that are responsible for creating the ambiguity. 
We thus suggest that the ambiguity arises as a probability distribution over the different realisations of the word, which then yields a probability distribution over the different realisations of the sentence. 

When it comes to multiple sources of ambiguity, we see that the individual density matrices now interact. E.g. 
\jurek{on mountain with telescope}

Further, we can consider probability distributions over different types of words.




\subsection{A Series of Examples}
\label{ch:SyntaxDistribution-Examples}

\jurek{it is important that you say: in the DisCoCat context, the sentence does not really alter the meaning of the words, also not with our model. It is only, when we introduce DisCoCirc, that the sentence becomes a process.}

\jurek{say, in the DisCoCat context, we can see that now we introduce processess so that certain words are processes connecting the words in different ways, but: this does not mean that the sentence is a process altering the meaning of the words. The word is a process, yes, but not one that alters the meaning of words, it alters the meaning of the sentence.}

\jurek{an important question is: How do we identify these source words? Generally, one could say that they are relative pronouns. However, only in certain contexts does it make sense to model the pronouns in such a way. Namely when there is ambiguity. 
Is there a mechanism to indicate if there is ambiguity present? 
It is not automated yet. But this is not really a problem, because there is another paper in which this is not automated, namely \citet{pronounResolution}

I believe that it is mostly pronoun resolution. 

}


In this section, we collect numerous examples to present the working of the framework presented in section \ref{ch:SyntaxDistribution-general}. 
After discussing a series of introductory examples, we briefly address the function of the word \texttt{and} as a connector and introduce multiple sources of ambiguity. 
A list of example sentences containing ambiguity can be found online\footnote{\url{https://www.examples.com/english/sentence/ambiguous-sentence.html} (accessed 12.08.2024)}. The example sentences in this chapter are in parts motivated by sentences in this collection. 


\jurek{List the examples without them having their designated subsections}

% % *************************************
% \subsection{An introductory Example}
% \label{ch:SyntaxDistribution-firstExample}
% % *************************************

We demonstrate the procedure of obtaining a probability distribution over diagrams for a number of examples, starting with the following sentence: 
\begin{displayquote}
    \texttt{The Man sees the woman on a mountain.}
\end{displayquote}
% This is a common example sentence in demonstrating ambiguity in language. This is because there are many different readings for this one single sentence, due to the individual phrases being ambiguous themselve. 
Here, the phrase \texttt{on a mountain} is the source of ambiguity. The phrase \texttt{on a mountain} can describe either the \texttt{man} being on a mountain, the \texttt{woman} being on a mountain, or both the \texttt{man} and the \texttt{woman} being on the mountain. Here, we choose to rule the third option of both \texttt{man} and \texttt{woman} being on the mountain out for now and give a fully integrated model in section \ref{ch:syntaxDistribution-multipleSources}, later in this chapter. 
The two possible DisCoCat diagrams for both the possible sentences are (either the \texttt{woman} or the \texttt{man} being on the mountain, respectively): 

\ctikzfig{manWomanOnMountain}
where we omit the words \texttt{the} and \texttt{a} and model \texttt{on mountain} as a noun modifier, modifying either \texttt{man} or \texttt{woman}. 

Now, the goal is to find a general diagrammatic way of displaying the effect of the phrase \texttt{on mountain} on the sentence meaning, where the phrase itself has internal ambiguity. 
We suggest the following: 

\ctikzfig{manWomanOnMountainGeneral}
where then the map \texttt{on-mountain} interacts with all the other words in the sentence.
Indeed, in this depiction, we do not choose to model either of the possible realisations of the sentence, but simply model the phrase \texttt{on-mountain} as a general state. 
To give meaning to this way of depicting the interaction of words, we need an inner structure for the phrase \texttt{on-mountain}. 
To fit the two readings above, the inner structure of the state \texttt{on-mountain} would then be either of these two: 

\ctikzfig{onMountain}
where the corresponding morphisms are for the left and right diagram, respectively: 
\begin{equation*}
\begin{split}
    &(\eta_N \otimes \eta_S) \circ (1_N \otimes 1_N \otimes 1_S \otimes \overrightarrow{\texttt{on-mountain}} \otimes 1_S) \circ (1_N \otimes 1_N \otimes 1_S \otimes \sigma_{NN} \otimes 1_S) \\
    &(\overrightarrow{\texttt{on-mountain}} \otimes \eta_S) \circ (1_N \otimes 1_N \otimes 1_S \otimes \eta_N \otimes 1_S)  \\
\end{split}
\end{equation*}
where $\sigma_{NN}$ is the \textit{swap morphism}. 
So far, we rewrote the diagram in a fashion that localises the difference in the two diagrams in the phrase \texttt{on-mountain} that is creating the ambiguity. Plugging in the two different wirings in the general diagram then yields the two initial readings of the sentence. 
% We moved the ambiguity (which is the reason for the different readings of the diagram) into one phrase.  

Now, in order to be able to model the ambiguity itself, we create a probability distribution over the two quantum states. 
A probability distribution over quantum states is a density matrix. This means that the phrase \texttt{on-mountain} is now represented by a density matrix as follows: 

\ctikzfig{onMountainDoubled}
where we use the doubled diagrams as mentioned in section \ref{subsec:quantumPicturialism} and $\alpha, \beta \in \mathbb{R}$, where $\alpha + \beta = 1$.
To introduce this density matrix to the diagram as above, the whole diagram has to be doubled, where the remaining states are elevated to being described by density matrices. These states are \textit{pure states}, in contrast to the density matrix described by \texttt{on-mountain}, which is a mixed density matrix over the two pure states shown above. 

% Now, we see how powerful and useful this model is. 
% We can now \textbf{keep the ambiguity alive}, because we do have a probability distribution over the two diagrams. 
We obtain the density matrix representing the meaning of the sentence by plugging in the probability distribution over the different wirings as above. 
We then obtain: 
\begin{equation*}
% \hspace*{-3cm}
    \resizebox{\textwidth}{!}{\tikzfig{onMountainFinalDiagram}}
\end{equation*}
% \ctikzfig{onMountainFinalDiagram}
as the density matrix representing the meaning of the ambiguous sentence. 
We see how the introduction of an ambiguous word, modelled by a mixed state, led to the diagram being modelled as a mixed state over the possible readings involving the respective realisations of the ambiguous word. 
The resulting density matrices can now be updated using the updating mechanism \textit{fuzz} or \textit{phaser} as introduced by \citet{meaningUpdatingDensMat}, mentioned in section \ref{subsec:densityMatricesInQNLP}. 
Step four in the list of instructions in section \ref{ch:SyntaxDistribution-general} is discussed shortly. First, we explore the application of the proposed framework to other examples containing linguistic ambiguity. 

% We continue by giving examples on how to employ the model to other cases of ambiguity. 





% *************************************
\subsection{Relative Pronouns in Dutch}
\label{ch:SyntaxDistribution-relPronDutch}
% *************************************

Following \citet{Wijnholds_2020}, consider, e.g., the Dutch phrase: 
\begin{displayquote}
    \texttt{Mensen die dieren eten}. 
\end{displayquote}
which translates to both: \[
\texttt{Humans who eat animals} \qquad \text{and} \qquad \texttt{Humans whom animals eat}
\]
making it an ambiguous sentence in Dutch. 
% \citet{relPronCoecke} and \citet{Wijnholds_2020} discuss ways on how to model relative pronouns. As argued by \citet{Wijnholds_2020}, in the Dutch language, the sentences \texttt{humans who eat animals} and \texttt{humans whom animals eat} have the same meaning \texttt{mensen, die dieren eten}.
Similarly to the above discussed, we propose a diagram structure as follows: 

\ctikzfig{mensenDierenEten}
where then the word \texttt{die} is modelled in either of these ways: 

\ctikzfig{dieModelling}
and we can form a superposition over the two states as above, by elevating the states to being density matrices. 


\subsection{We saw her duck}
\label{ch:SyntaxDistribution-herDuck}

In the following example: 
\begin{displayquote}
    \texttt{We saw her duck.}
\end{displayquote}
the two readings are: 
\begin{displayquote}
    \texttt{We saw the duck that belongs to her.} \newline 
    \texttt{We saw her ducking down.}
\end{displayquote}
Here, ambiguity is introduced by the word \texttt{duck}. 
In the former case, \texttt{duck} is a noun, and \texttt{her} is a modifier of this noun. In the latter case, \texttt{her} is a noun, where \texttt{duck} is a modifier of this noun. 
We thus have the following diagram: 

\ctikzfig{herDuck}
where the density matrix $\rho_{\texttt{duck}}$ is a probability distribution over the two diagrams as follows: 

\ctikzfig{duck}
where, in the former case, \texttt{duck} is a noun and in the latter case it is a noun modifier (it describes a certain property of \texttt{her}). 

% \section*{She fed her cat food}
% \label{ch:SyntaxDistribution-catFood}


% *************************************
\subsection{Pronoun Resolution}
\label{ch:SyntaxDistribution-pronounResolution}
% *************************************

Consider, as a third example, the sentence 
\begin{displayquote}
    \texttt{Dog hunts cat. It is fast.}
\end{displayquote}
The word \texttt{it} refers to a noun phrase (either \texttt{cat} or \texttt{dog}) in the first sentence, as discussed in section \ref{sec:pronounResolution}.  
We can introduce a probability distribution over copying either \texttt{cat} or \texttt{dog} as: 
\ctikzfig{catHuntsDogGeneral}
where, again, the word \texttt{it} is modelled as either of the two: 

\ctikzfig{itPossibleRealisations}
Now, we present a way of understanding the word \texttt{it} as a \textit{process} acting on the other words in the sentence, which corresponds to step four in the list of instructions given in section \ref{ch:SyntaxDistribution-general}. We can then regard the function of the word \texttt{it} as a probability distribution over copying either the word \texttt{dog} or \texttt{cat} in the sentence. 
We demonstrate this by plugging in the first of the above representations of the word \texttt{it} in the DisCoCat diagram above. 

\ctikzfig{makeStateProcess}
\clearpage
We remove some of the cups and caps like this: 

\ctikzfig{makeStateProcessTwo}
which we can rewrite as: 

\ctikzfig{makeStateProcessThree}
where we identified the word \texttt{it} as a morphism acting on the rest of the words in the sentence. 
Note that this representation of the word \texttt{it} is {different} from the representation of the word \texttt{it} as a state. This means that obtaining a morphism from the state representation does not simply entail rewiring of the word's diagrammatic representation, but rather choosing a different representation altogether. 
Upon following the same procedure for the second representation of the word \texttt{it}, we find the two morphisms: 

% \ctikzfig{itPossibleMorphismOne}

\ctikzfig{itPossibleMorphismTwo}
We can now model the resulting word \texttt{it} as a \textit{mixed quantum state} describing a probability distribution over the two \textit{pure quantum states} as: 

\begin{equation*}
% \hspace*{-3cm}
    \resizebox{\textwidth}{!}{\tikzfig{itDiagrammaticDM}}
\end{equation*}
% \ctikzfig{itDiagrammaticDM}
where we used the doubled diagrammatic notation introduced above, indicating that these diagrams are representing density matrices, which are themselves representing pure states. We will stick to the representation of displaying probability distributions over morphisms using dashed lines as above. 

% Note that for all the above discussed, it is possible to use the process state duality to turn states into processes, where then the notion of the \textit{marker words} being \textit{processes} that change the meaning of the words in the sentence makes much intuitive sense. 
Applied to the above example, we can model the word \texttt{it} as a density matrix acting locally on the two pure states \texttt{cat} and \texttt{dog}, this makes it clearer in which part of the diagram the ambiguity arises, as: 

\ctikzfig{catHuntsDogDesired}
% We can rewrite the diagrams in this fashion because \textit{only connectivity matters} \citep{coeckebook}. However, 
We termed the morphism $\rho^*_{\texttt{it}}$ with an asterisk, because it is a different morphism than the above presented $\rho_{\texttt{it}}$. 

Since it is the more general approach, we stick to modelling the morphisms in the former manner (ambiguous words are morphisms acting on all words in the circuit rather than some words). The motivation behind choosing this representation will become apparent in the process of mapping these diagrams to quantum circuits in section \ref{ch:SyntaxDistribution-mappingtoQC}. 

% There are numerous other examples which can be modelled using this framework, e.g.: 
% \begin{displayquote}
%     \texttt{He fed her cat food} \newline 
%     \texttt{John said on Monday he will cook.}
% \end{displayquote}
% Due to time reasons, we will not model these examples in detail. 
% we see that this diagram describes a probability distribution over, in this case, two different possible diagrams. In conclusion, we say that this diagram describes a mixed state, containing pure states that correspond to the simple copying mechanisms. 
% Note that we have two open sentence wires. The left one captures the meaning of \texttt{cat hunts dog}, a pure state, whereas the right one captures the meaning of \texttt{it is fast}, which is a mixed state over \texttt{cat is fast} and \texttt{dog is fast}. 

% *************************************
\subsection{Verb Phrase Ellipsis}
\label{ch:SyntaxDistribution-gijs}
% *************************************

We now consider the case of Verb phrase ellipsis in this light, using the following sentence: 
\begin{displayquote}
    \texttt{Bill eats and drinks. Mary does too.}
\end{displayquote}
With the three possible readings:
\begin{itemize}
    \item \texttt{Bill eats and drinks. Mary eats.}
    \item \texttt{Bill eats and drinks. Mary drinks.}
    \item \texttt{Bill eats and drinks. Mary eats and drinks.}
\end{itemize}
where the second phrase refers to the verb in the noun phrase. 
Starting from the model suggested by \citet{Wijnholds_2020}, we integrate the copying of the verb in the base sentence into the phrase \texttt{does too}. 
\citet{Wijnholds_2020} models the phrase \texttt{does too} as: 

\ctikzfig{doesToo}
Additionally, the information in the former sentence (either \texttt{eats}, \texttt{drinks} or \texttt{eats and drinks}) is copied explicitly. We integrate these nonlinearities into the phrase itself as: 

\begin{equation*}
% \hspace*{-3cm}
    \resizebox{\textwidth}{!}{\tikzfig{billEatsDrinksMaryDoesToo}}
\end{equation*}
where we used the representation of the word \texttt{and} for combining verbs as: 

\ctikzfig{copyVerb}
\clearpage
We simplify this, turning the state into a process as above: 

\ctikzfig{billEatsDrinksMaryDoesTooMorphism}
so that the three different wirings for the word \texttt{does too} are: 

\begin{equation*}
% \hspace*{-3cm}
    \resizebox{\textwidth}{!}{\tikzfig{doesTooInternalWiring}}
\end{equation*}
where the first diagram represents \texttt{\ldots Mary eats and drinks}, the second one represents \texttt{\ldots Mary eats} and the third one represents \texttt{\ldots Mary drinks}.  
We thus expand the theory by \citet{Wijnholds_2020} and capture all the nonlinearity in the phrase \texttt{does too}.

% \jurek{what other upsides are there to the locality of the ambiguity source???}
% Other than being able to create probability distributions over mechanisms in diagrams, this procedure is a more general approach to this type of ambiguity. 
% The presence of the phrase \texttt{does too} implies that information has to be copied. 


\subsection{The Word \texttt{and}}

We discuss one example involving the connector-word \texttt{and} as the source of ambiguity. 
% Indeed we will discover that the word \texttt{and}, fusing together either adjectives or nouns, is the same. 
The following presentation does not directly relate to the methodology as the basic idea of this thesis. However, it does help reason about how only in certain situations the replacement of words by combinations of wires in diagrams is advantageous.  
Consider the example sentence: 
\[
\texttt{Bob has blue and green hats.}
\]
This sentence has two readings: 
\begin{displayquote}
    \texttt{Bob has blue hats and green hats.} \newline 
    \texttt{Bob has hats that are both blue and green.}
\end{displayquote}
where, in the first sentence, the word \texttt{and} is: 

\ctikzfig{nounAnd}
and in the second case: 

\ctikzfig{adjectiveAnd}
where two adjectives are fused, and an adjective is a vector in the space $N \otimes N$. 
We plug in the second one of these representations (the word \texttt{and} acting on the adjectives): 

\jurek{I suppose I could make the 'and'-argument shorter}

\begin{equation}
\label{eq:bobbluegreenhats}
    \tikzfig{bobBlueGreenHats}
\end{equation}
\clearpage
For the first one of these representations (the word \texttt{and} acting on the noun \texttt{hats}):

\begin{equation}
\label{eq:bobbluegreenhatstwo}
    \tikzfig{bobBlueGreenHatsTwo}
\end{equation}
% Now, before moving further with the methodology introduced above, w
We now take a closer look at these two diagrams. 
By pulling the right spider in diagram \ref{eq:bobbluegreenhats} to the position of the word \texttt{hats}: 

\ctikzfig{bobBlueGreenHatsThree}
we have exactly diagram \ref{eq:bobbluegreenhatstwo}, which means that, within the way of modelling this sentence in the pregroup formalism here, the sentences are indistinguishable. 
% This means that the pregroup formalism is not a suitable framework for modelling these types of semantics.  
% The two different sentences are distinct in the following property: 
% \[
% \texttt{(blue and green) } \circ \texttt{ hats } \quad \textbf{vs.} \quad  \texttt{ (blue } \circ \texttt{ hats) } \texttt{ and } \texttt{ (green } \circ \texttt{ hats) }
% \]
% Note that in the first case the word \texttt{and}, as the source of ambiguity furthermore entails the copying of the word \texttt{hats}. If we reinterpret \texttt{and} in this way, what we find is the \textbf{same} representation for \texttt{and} as if we were to fuse the words \texttt{green} and \texttt{blue} via a spider.   
% We have to ask ourselves why this is the case. 
% \citet{Wijnholds_2020} argues that the problem of using the Pregroup grammar as an underlying framework lies in copying information using the Frobenius map: the Frobenius map puts a vector on the diagonal of a matrix. The copied word is then entangled, and interaction with the non-entangled vector is not possible anymore \citep[p.101, 102][]{Wijnholds_2020}. 
% % argues that the copying by the Frobenius map, followed by entanglement, is the main problem. 
% % He gives the example sentence: 
% % \begin{displayquote}
% %     \texttt{Alice loves herself.}
% % \end{displayquote}
% % where the vector $\overrightarrow{\texttt{alice}} = \sum_i a_i \overrightarrow{v}_i$ is assigned to \texttt{Alice} and the tensor $\overrightarrow{\texttt{loves}} = \sum_{jkl} c_{jkl} ( \overrightarrow{v}_j \otimes \overrightarrow{s}_j \otimes \overrightarrow{v}_l )$ is assigned to the word \texttt{loves}. 
% \citet{Wijnholds_2020} avoids this problem by moving to a simply typed lambda calculus in which to interpret proofs in the Lambek calculus in. This framework is introduced in section \ref{subsec:lambdaCalculus}. 
We argue that the problem, in this specific case, arises in the assignment of the meaning of the word \texttt{and} as structures of wires. 
As we can see in the diagrams above, the meaning of the word \texttt{and} changes between diagram \ref{eq:bobbluegreenhats} and \ref{eq:bobbluegreenhatstwo}: in diagram \ref{eq:bobbluegreenhats}, it combines the meaning of two adjectives $\in N \otimes N$, whereas in diagram \ref{eq:bobbluegreenhatstwo}, the word \texttt{and} combines two nouns $\in N$. 
We argue that the problem arises due to the source of the ambiguity in the sentence, in this case the word \texttt{and}, not having inherent meaning but redirecting the flow of information in the form of numerous wires. 
Note that if the meaning of \texttt{and} would be static, represented by, e.g.: 
\ctikzfig{andDilemma}
Then, the problem of rearranging the spiders to obtain a different representation of the word \texttt{and} would not occur. 
Upon rewriting the diagram, we change the meaning of the word \texttt{and}. Thus, the meaning of the sentences represented in diagrams \ref{eq:bobbluegreenhats} and \ref{eq:bobbluegreenhatstwo} changes.

% We argue, in the specific case encountered here, that distinctions between distributive relations like the above are not modellable using the pregroup formalism, because it inherently is distributive. 
% Furthermore, as mentioned in section \ref{subsec:quantumPicturialism}, the spider is commutative. Thus, the spider as a copying operation does not differentiate between the order of fusing the adjectives and copying 

As mentioned above, the model works in other sentences when the word \texttt{and} is not the \textit{source} of ambiguity, as in e.g.: 
\begin{displayquote}
    \texttt{Bob reads and writes. He does it well.}
\end{displayquote}
% where the three readings are: 
% \begin{displayquote}
%     \texttt{Bob reads and writes. Bob reads well.} \newline 
%     \texttt{Bob reads and writes. Bob writes well.} \newline 
%     \texttt{Bob reads and writes. Bob both reads and writes well.}
% \end{displayquote}
% Thus, we have to copy the information of the verbs. In the first case \texttt{reads}, in the second case \texttt{writes}, and in the latter case \texttt{reads and writes}. 
% The ambiguity in this example arises from the word pair \texttt{does it}, which is to be replaced with the appropriate choice of verb. 
This example is similar to the case of verb phrase ellipsis, discussed in section \ref{ch:SyntaxDistribution-gijs}. 
% The modelling works in the same way. 
% \ctikzfig{bobReadsAndWrites}
% where we then model the phrase \texttt{does it}, which is the source of ambiguity here, as: 
% \jurek{missing}
% Note that we can do the same thing for nouns as in: 
% \[
% \texttt{The old men and women left the room.}
% \]
% The adjective \texttt{old} can relate to the men, or both the men and women. 
% We can thus create a superposition over these two readings in a fashion that is completely similar to the approach presented above.

% The aspect addressed in this thesis is important to keep in mind, when ambiguouos words that are modelled completely as wires, without inherent meaning, but via the redirection of information in the diagrams. 


% The two possible readings are: 
% \begin{itemize}
%     \item \texttt{He fed food to her cat}
%     \item \texttt{He fed her using cat food.}
% \end{itemize}
% (ignoring the nonsensical sentence of \texttt{He fed the product which is cat food.})

% This is a slightly more involved example, since in the first example, the word \texttt{her cat} is the object, when in the second example the word \texttt{her} is the object. On the other hand, what is being fed is, in the first case \texttt{food} and in the second case \texttt{cat food}. 

% Firstly, we search for the ambiguity source. In this case, this would be the word \texttt{her}. 

% \jurek{I don't know if I should really do this... too involved}

% Note that sentences like: 

% \texttt{on Monday} could be both acting on \texttt{said} or \texttt{he will cook}. 

% \jurek{the above: limit it to a list of possible investigations}


\subsection{Multiple Sources of Ambiguity}
\label{ch:syntaxDistribution-multipleSources}

Consider now introducing two sources of ambiguity, as in: 
\begin{displayquote}
    \texttt{The man saw the woman on the mountain with a telescope.}
\end{displayquote}
where there are at least nine readings for this sentence: 
\begin{itemize}
    \item \texttt{The (man on the mountain) saw the (woman with a telescope)}
    \item \texttt{The (man with a telescope) saw the (woman on the mountain)}
    \item \texttt{The (man on the mountain with a telescope) saw the woman}
    \item \texttt{The man saw the (woman on the mountain with a telescope)}
    \item \texttt{The (man on the mountain) (saw with a telescope) the woman}
    \item \texttt{The man (saw with a telescope) the (woman on the mountain)}
    \item \texttt{The man and the woman are on the mountain. The man saw the (woman with a telescope)}
    \item \texttt{The man and the woman are on the mountain. The (man with a telescope) saw the woman}
    \item \texttt{The man and the woman are on the mountain. The man (saw with a telescope) the woman}
\end{itemize}
Note that \texttt{with telescope} can either mean \texttt{who has a telescope} or \texttt{use a telescope to do something}. 
Following the reasoning above, we can model all of these nine readings within one diagram as: 

\ctikzfig{manWomanTelescope}
where, in one of the cases, the phrase \texttt{with telescope} acts as a verb modifier on the verb \texttt{saw}, and the nouns are simple wires.  
Obtaining these wirings is similar to the above cases. 
% As a more involved example consider the following sentence: 
% \begin{displayquote}
%     \texttt{Bob hates Gary and he likes his garden.}
% \end{displayquote}
% All of these readings can be captured by the following diagram: 
% \ctikzfig{bobLikesGaryAndSoOn}
% where both the words \texttt{his} and \texttt{he} are density matrices as discussed above. 
% We do not give explicit representations for the words \texttt{he} and \texttt{his} here. 
% Although \citet{Wijnholds_2020} introduced ways to reason about the anaphor \texttt{he}/\texttt{her}, he argued that this is not translatable to the pregroup formalism. 
% Note that we use the process state duality all the time: 
% The above diagrams are modelled as states (with some number $N$ wires coming in). But these can be modelled as effects with some number $N-n$ wires coming in and some $n$ wires going out. 
One can now reason further with these density matrices, using the comparison to other density matrices via fidelity or the updating mechanisms \textit{fuzz} (definition \ref{def:fuzz}) and \textit{phaser} (definition \ref{def:phaser}) introduced in section \ref{subsec:densityMatricesInQNLP}. 

 

%*************************
\subsection{Reasoning with the Quantum Probability Distribution}
\label{ch:SyntaxDistribution-reasoning}
%*************************

\jurek{the part about reasoning has been taken from my thesis, but I think I would like to re-do it and move away from the specific example. It feels a little bit redundant. }

% \jurek{perhaps take the above and put it here? The idea behind this section is to explain how to reason with the above, using also the trace inner product etc. }

% After introducing a series of examples, we explain in detail the advantages of this model compared to the state-of-the-art methodology. 
% In this section, we explain in more detail the upside of the above presented model. 
% The reason that this approach is useful is the \textbf{maintaining} and modelling of the ambiguity. 
We discuss the process of reasoning with the created density matrices using one explicit example, followed by a connection to work by \citet{pronounResolution}, presented in section \ref{sec:pronounResolution}. 
In general, the process of changing the meaning of a sentence represented by a density matrix entails updating this density matrix by other density matrices, representing the meaning of further sentences.  
% \jurek{explain how actually, we can map this to quantum circuits and that we can, compared to the work done by \citet{pronounResolution} do this from semantics alone!! we have to note that our probability distribution works only on the basis of interacting density matrices. If we only have the sentence dog hunts cat it is fast, this doesn't give us anything. We do need the information that either of cat or dog are fast to make this model powerful.
% We don't have to learn the things like \citet{pronounResolution} did, it is learned already!! We just have to access it!! }
% We start with the updating mechanism for density matrices. As mentioned in section \ref{subsec:QT-densityMatrices}, \citet{meaningUpdatingDensMat} argue that imposing a proposition onto a density matrix is according to: 
% \begin{equation*}
%     P \circ - \circ P
% \end{equation*}
% where $P$ is a \textit{projector}. They argue that every projector is a (potentially not-normalized) density matrix and each density matrix admits a \textit{spectral decomposition} as: 
% \begin{equation*}
%     \sum_i x_i P_i
% \end{equation*}
% where $P_i$ are projectors into the eigenspace. 
% The above process is carried out by both the \textit{Fuzz} and \textit{Phaser} presented in section \ref{subsec:densityMatricesInQNLP}. 
% \jurek{cite missing, look into meaning updating paper}
% .. and ... argue that it is a natural way to reason about properties being imposed onto words as applying appropriate projectors. 
% This is a very natural approach to language and ultimately models closer how the human brain works than the models before it. 
% This is because, if one was to hear a sentence like \texttt{the man saw the woman on a mountain with a telescope}, one would wait until obtaining more information about said woman or man until fully collapsing the wave function. 
% Consider a density matrix $\rho_{\texttt{s1}}$ describing a probability distribution over different readings of a diagram in some sentence and the meaning of a second sentence $\rho_{\texttt{s1}}$. 
% The interaction of these density matrices will yield a new density matrix which will then contain an updated probability distribution over the two possible readings of the diagram corresponding to the first sentence, given the information acquired within the second density matrix. 
% Consider the case in which we are dealing with \textit{real} uncertainty. Because of the lack of context, we cannot know what word is to be copied. We want to emphasize that this is not to do with the model itself, because we cannot model what we don't know. 
% The powerfulness comes from \textbf{maintaining the ambiguity} and adjusting the probability distribution representing it when seeing more context. 
% The meaning represented by the density matrix can the be updated via the methods \texttt{FUZZ} or \texttt{PHASER} introduced by \citet{meaningUpdatingDensMat}. 
% One can furthermore compare density matrices and measure their similarity by employing methods like the \textit{trace inner product} or the \textit{fidelity}. 
% These are established methods and do not contribute to the novelty of our work. We will go into more detail in section \ref{sec:experiments}. 
To explain the reasoning process using density matrices, we use the example sentence 
\[
\texttt{Bob hates Gary and he likes his garden.}
\]
There are four possible readings to this sentence: 
\begin{displayquote}
    \texttt{Bob hates Gary and Bob likes Gary's garden.} \newline 
    \texttt{Bob hates Gary and Bob likes Bob's garden.} \newline 
    \texttt{Bob hates Gary and Gary likes Gary's garden.} \newline 
    \texttt{Bob hates Gary and Gary likes Gary's garden.} 
\end{displayquote}
And the two words causing the ambiguity in the sentence are the words \texttt{he} and \texttt{his}. The corresponding diagram is: 

\ctikzfig{bobLikesGaryAndSoOn}
where the word \texttt{he} copies the appropriate person \texttt{Bob} or \texttt{Gary}, and the word \texttt{his} relates either \texttt{Bob} or \texttt{Gary} to the noun \texttt{garden}. We will not discuss the internal wirings of the words \texttt{his} or \texttt{he} in detail. For a way of modelling this sentence using the Lambek calculus with control modalities discussed in section \ref{subsec:Gijs-theory}, we refer to \citet[][p.93-98]{Wijnholds_2020}. 
The density matrix describing the sentence will be referred to as $\rho_{\texttt{s1}}$. 
Given some new information in the form of another sentence $\rho_{\texttt{s2}}$, we update the meaning of $\rho_{\texttt{s1}}$ using $\rho_{\texttt{s2}}$. 
Consider the explicit second sentence: 
\begin{displayquote}
    \texttt{Bob likes his garden.}
\end{displayquote}
In the following, we use the spider as a composition method of density matrices to keep the calculations simple. 
For the composition of the density matrices, one can use the spider, or the fuzz $\sharp$ (definition \ref{def:fuzz}), or the phaser $\flat$ (definition \ref{def:phaser}). 
While we use the symbol $'\circ'$ for the composition, the following discussion applies to either of the three. 
As argued in section \ref{subsec:densityMatricesInQNLP}, the fuzz and phaser are to be preferred in general. 
We have for $\rho_{\texttt{s1}} \circ \rho_{\texttt{s2}}$:
\begin{equation*}
\begin{split}
        & \quad \underbrace{\rho_{\texttt{Bob hates Gary and he likes his garden}}}_{\text{mixed state}} \circ \, \rho_{\texttt{Bob likes his garden}} \\
        & = \alpha \cdot  \underbrace{\rho_{\texttt{Bob hates Gary and Bob likes Gary's garden}}}_{\text{pure state}} \circ \, \rho_{\texttt{Bob likes his garden}}\\
        & + \beta \cdot  \underbrace{\rho_{\texttt{Bob hates Gary and Bob likes Bob's garden}}}_{\text{pure state}} \circ \, \rho_{\texttt{Bob likes his garden}}\\
        & + \gamma \cdot  \alpha \cdot  \underbrace{\rho_{\texttt{Bob hates Gary and Gary likes Gary's garden}}}_{\text{pure state}} \circ \, \rho_{\texttt{Bob likes his garden}}\\
        & + \delta \cdot  \underbrace{\rho_{\texttt{Bob hates Gary and Gary likes Bob's garden}}}_{\text{pure state}} \circ \, \rho_{\texttt{Bob likes his garden}}\\
\end{split}
\end{equation*}
where $\alpha, \beta, \gamma$ and $\delta$ are real coefficients. 
% where, here, the composition $\circ$ could be either of \textit{Fuzz}, \textit{Phaser}, or even the \textit{Spider}. Here, for reasons of simplicity, we assume the $\circ$ to be a spider as presented in section \ref{subsec:quantumPicturialism}. 
Then, using: 
\begin{equation*}
    \rho_{\texttt{Bob hates Gary and Bob likes Bob's garden}} = \rho_{\texttt{Bob hates Gary}} \circ \rho_{\texttt{Bob likes Bob's garden}}
\end{equation*}
if we assume for simplicity here that these states commute (the order in which the respective sentences occur in the text are irrelevant). 
Now, we see that the pure state representing the meaning of: 
\begin{equation}
\label{eq:readingBob}
    \texttt{Bob hates Gary and Bob likes Bob's garden}
\end{equation}
will yield the highest probability, when composed with $\rho_{\texttt{s2}}$,  
% \[
%  {\rho_{\texttt{Bob hates Gary and Bob likes Bob's garden}}} \circ \, \rho_{\texttt{Bob likes his garden}}
% \]
whereas the probabilities for the other cases will be lower in the resulting probability distribution, which means that the resulting probability distribution includes all possible readings, with the reading shown in equation \ref{eq:readingBob} being the most likely. 
% Note that we can employ other methods like the fuzz (definition \ref{def:fuzz}) and phaser (definition \ref{def:phaser}) here as well, by replacing the spider $\circ$ with either fuzz $\sharp$ or phaser $\flat$. If we look at the explicit definitions of fuzz and phaser in section \ref{subsec:densityMatricesInQNLP}, we see that the probability of composing $\rho_{\texttt{s1}}$ with $\rho_{\texttt{s2}}$ will also yield the term in equation \ref{eq:readingBob} being assigned the highest probability in the distribution. 

Consider a second example sentence:
\[
\texttt{Bob does not like his garden.}
\]
as an updating sentence for the first sentence $\rho_{\texttt{s1}}$. 
The corresponding state is orthogonal to the state corresponding to: 
\[
\texttt{Bob likes his garden.}
\]
which means $\braket{\psi_{\texttt{Bob does not like his garden}}|\psi_{\texttt{Bob likes his garden}}} = 0$. 
This subsequently means that the corresponding term in the composition of the density matrices 
% \[
%  {\rho_{\texttt{Bob hates Gary and Bob likes Bob's garden}}} \circ \, \rho_{\texttt{Bob does not like his garden}}
% \]
will yield the probability of zero, which results in this pure state vanishing from the density matrix $\rho_{\texttt{Bob hates Gary and he likes his garden}}$ upon composition. 
% Ultimately, what we do with this procedure is the following. We have a probability distribution over certain meanings (\texttt{Bob likes Bob's garden}, \texttt{Bob likes Gary's garden} etc.). Upon encountering more information, in the form of sentences which are modelled as density matrices, we can update this probability distribution over meanings. 
% This probability distribution is updated continuously with the sentences in the context. 
% Once the text is finished, we obtain a probability distribution over the possible compositions of the individual sentences. This is merely a probability distribution over possible \textit{text meanings}. 
% By updating a density matrix continuously using other density matrices, ultimately, we obtain a density matrix which is a probability distribution over all the possible meanings arising from the interaction of the sentences. 

This is also valid when combining ambiguous sentences.
% , as we have shown using the sentence \texttt{Bob hates Gary and he likes his garden.}
% The ambiguities caused by the words \texttt{he} and \texttt{his} interact to ultimately give four possible readings for the whole sentence. 
If a second sentence updating the first one were to be ambiguous as well: 
\begin{displayquote}
    \texttt{Gary likes Bob. He is nice.}
\end{displayquote}
the arising probability distribution (consisting of two terms, either \texttt{Gary} or \texttt{Bob} being nice) in this sentence will interact with the four terms in the former density matrix to give a density matrix made up of eight individual pure states, each with the corresponding probability. 
\newline \newline 
We address the concrete upsides to this approach in QNLP tasks.  
Consider the task executed by \citet{pronounResolution}, presented in \ref{sec:pronounResolution}. They learned a model to be able to classify diagrams in one of two categories: a pronoun referring to the object or the subject in a sentence. 
One of the example sentences used by \citet{pronounResolution} in the training procedure is: 
\begin{displayquote}
    \texttt{The dog broke the vase. It was fragile.}
\end{displayquote}
where, in this example, the object (\texttt{the vase}) is to be copied. 
We claim that one does not explicitly have to teach the model this differentiation, rather that one can achieve this differentiation with a model that learned the \textit{semantics} of all the involved words. 
In our approach, this procedure would be a mere reasoning with the learned model. 
If, in the training procedure, the model acquires the information that a \texttt{vase} can be \texttt{fragile}, while a \texttt{dog} cannot, ultimately a probability distribution is created with a higher probability associated to the \texttt{vase} being copied than to the \texttt{dog} being copied. 
Concretely, consider a binary classification task, in which the two categories are \texttt{True} and \texttt{False}. 
% The training set could then look as displayed in table \ref{tab:exampleSet}.
% \begin{table}[h]
%     \centering
%     \begin{tabular}{cc}
%         \textbf{Sentence} & \textbf{Label}\\
%         \texttt{Dog is fragile} & \texttt{False} \\
%         \texttt{Vase is fragile} & \texttt{True} \\
%         \texttt{The dog broke something} & \texttt{True} \\
%         \texttt{The vase is something} & \texttt{True} \\
%     \end{tabular}
%     \caption{Example training set. For context see main text}
%     \label{tab:exampleSet}
% \end{table}
% Note that this is a very simple example, which can however be extended to more complex examples. 
% Let's consider that the model learned a mapping for all of these words correctly (using processes presented in section \ref{sec:training-pipeline}). 
After processing the above sentence, our framework models the probability distribution as: 
\begin{equation*}
    \rho_{\texttt{whole sentence}} = \num{0.5} \cdot \rho_{\texttt{dog broke vase, dog is fragile}} + \num{0.5} \cdot \rho_{\texttt{dog broke vase, vase is fragile}}
\end{equation*}
We now want to assess the truthfulness of the individual terms in the probability distribution. 
% We want to find which of the possible readings is the most true. 
For this, as reasoned above, we \textit{project out} the true part by updating the density matrix using the pure density matrix corresponding to the pure state $\rho_{\texttt{True}}$.
% As an example, consider the label \texttt{True} to be represented by $\ket{1}$, while \texttt{False} is represented by $\ket{0}$, so that: 
% \begin{equation*}
%     \rho_{\texttt{True}} = \ket{1}\bra{1}
% \end{equation*}
Updating the meaning using the {spider} yields the following: 
\begin{equation*}
\begin{split}
    \qquad \qquad  \rho_{\texttt{whole sentence}} \circ \rho_{\texttt{True}}
    & = \num{0.5} \cdot \rho_{\texttt{dog broke vase, dog is fragile}} \circ \rho_{\texttt{True}} \\
    &+ \num{0.5} \cdot \rho_{\texttt{dog broke vase, vase is fragile}} \circ \rho_{\texttt{True}} \\
    & = \num{0.5} \cdot \rho_{\texttt{dog broke vase, vase is fragile}}
\end{split}
\end{equation*}
which then is to be renormalised as mentioned in section \ref{subsec:densityMatricesInQNLP}. 
We see that, by firstly creating the probability distribution over the possible diagrams and then projecting out the diagram that is true by composing the density matrix with the pure density matrix $\rho_{\texttt{True}}$, we are able to recover the correct sentence wiring from the semantics of the words. 

We illustrated that we can recover the correct {syntax} from the {semantics} only. 
This works for more involved examples as well. However, we don't always have as clear a notion of what is actually \texttt{True} and what is \texttt{False}, depending on the semantics of the sentence space that the model is trained on. 
% What we end up with in the end is then not a probability distribution, which is one at some point and zero everywhere else, as in the example above. 
% All wirings are possible, while some are significantly more likely than others. In the above example, the \texttt{dog} technically could be \texttt{fragile} as well, it is just significantly less likely. 

% After explaining how to reason with the quantum probability distribution, we try to delve deeper and explain the ambiguity in the resulting sentence as a result of ambiguities of individual words interacting. We do this in section \ref{ch:SyntaxDistribution-oldmanship}, after explaining the mapping to quantum circuits in the following chapter.  
% Consider the simple example in which we want to compare the density matrix arising from the ambiguity above with how \texttt{TRUE} one or the other reading is. 
% One can take the trace inner product with the density matrix: 
% \begin{equation*}
%     \Tr \big( \rho_{\texttt{it is fast}} \cdot \rho_{\texttt{TRUE}}\big)
% \end{equation*}
% where only $\rho_2$  




\jurek{clearly, in the presentation above, the question has to be asked about how the sources of ambiguity can be identified in text. 
Again, things like these might be recovered from boundary entropy, e.g., when the entropy rises after encountering the word it, this might be due to the word it introducing ambiguity to the sentence. }

\jurek{add also that we propose the source word to be made up of only wires (refer to coecke) but in addition, we propose that it is a morphism that entails copying either of the other words.}


% %*************************
% \subsection{Mapping to Quantum Circuits}
% \label{ch:SyntaxDistribution-mappingtoQC}
% %*************************

% In this section, we explain how we map the concept of having a probability distribution over diagrams onto quantum circuits using maximally entangled states. 
% In order to map the density matrices representing diagrams to quantum circuits, we use a particular trick presented in the following.
% This trick is a particular quantum circuit architecture and is displayed in diagram \ref{diag:mappingToQC}.
% \begin{figure}[h]
%     \centering
%     \ctikzfig{simpleExample}
%     \caption{Ansatz for creating a quantum probability distribution over carrying out two operations $O_1$, $O_2$}
%     \label{diag:mappingToQC}
% \end{figure}
% Generally there are two operations on qubits $q_1$ and $q_2$ termed $O_1$ and $O_2$, respectively. 
% The idea behind this circuit is that, due to the $X$-gate in between the two controlled gates on qubit $q_3$, only one of the operations $O_1$ or $O_2$ is executed. 
% What this circuit thus does is, it entangles the qubits $q_3$ and $q_2$ with probability \num{0.5}, and if it does not entangle qubits $q_3$ and $q_2$, it entangles qubits $q_3$ and $q_1$. 
% We verify this using the explicit matrix representations for the qubits: 
% \begin{equation*}
%     \big(\ket{0} \otimes \ket{0} \otimes \ket{0} \big) \circ \big( \texttt{H} \otimes 1 \otimes 1 \big) \circ \big( \ket{0} \bra{0} \otimes 1 \otimes 1 + \ket{1}\bra{1} \otimes O_1 \otimes 1 \big) \circ \big( \texttt{X} \otimes 1 \otimes 1 \big) \circ \big( \ket{0} \bra{0} \otimes 1 \otimes 1 + \ket{1}\bra{1} \otimes 1 \otimes O_2 \big)
% \end{equation*}
% where $1$ is the two dimensional identity matrix.
% % We will apply the gates step by step and explain the result. 
% Firstly, from the initial state $\ket{000}$, applying the Hadamard gate yields: 
% \begin{equation*}
%     \frac{1}{\sqrt{2}} \big( \ket{0} + \ket{1} \big) \otimes \ket{0} \otimes \ket{0} 
% \end{equation*}
% Now, applying the first controlled operation, we have: 
% \begin{equation*}
%     \frac{1}{\sqrt{2}} \big( \ket{0} \otimes \ket{0} \otimes \ket{0} + \ket{1} \otimes \ket{0} \otimes \ket{0} \big) \circ \big( \ket{0} \bra{0} \otimes 1 \otimes 1 + \ket{1}\bra{1} \otimes O_1 \otimes 1 \big) = \frac{1}{\sqrt{2}} \big( \ket{0} \otimes \ket{0} \otimes \ket{0} + \ket{1} \otimes O_1 \ket{0} \otimes \ket{0} \big)
% \end{equation*}
% which we then, after applying the $X$-gate to the first qubit, which flips the state for the first qubit, apply the second control operation to: 
% \begin{equation*}
%     \frac{1}{\sqrt{2}} \big( \ket{1} \otimes \ket{0} \otimes \ket{0} + \ket{0} \otimes O_1 \ket{0} \otimes \ket{0} \big) \circ \big( \ket{0} \bra{0} \otimes 1 \otimes 1 + \ket{1}\bra{1} \otimes 1 \otimes O_2 \big) = \frac{1}{\sqrt{2}} \big( \ket{1} \otimes \ket{0} \otimes O_2 \ket{0} + \ket{0} \otimes O_1 \ket{0} \otimes \ket{0} \big)
% \end{equation*}
% This is the resulting state after executing the circuit. 
% We see that, if the first operation $O_1$ is applied, the first and third qubit will be measured to $\ket{0}$, whereas if the second operation $O_2$ is applied, the first qubit will be measured to $\ket{1}$ and the second qubit will be measured to $\ket{0}$. We see that, if one operation is applied, the other is not. 
% This is what we need to model the above density matrices on quantum circuits, as will become evident shortly. 
% Now, by discarding qubit $q_3$, we obtain a maximally mixed state, which represents a probability distribution over which of the operations are executed. 

% The motivation behind this idea is that we can now connect these operations $O_1$ and $O_2$ to connecting diagrams in a certain way. 
% For example, as we will see shortly, the operations could be connected to copying different words in the sentence. Consider again: 
% \begin{displayquote}
%     \texttt{The dog hunts the cat and it is fast.}
% \end{displayquote}
% Operation $O_1$ would be to copy the qubit encoding the word \texttt{dog} and operation $O_2$ to copy the qubit representing the word \texttt{cat}. 
% Note that if there were more possible readings, one can extend the number of readings that can be displayed by adding qubits to the quantum circuit in diagram \ref{diag:mappingToQC} (adding $n$ qubits to the diagram will allow us to model $2^n$ times the ambiguity). 
% Using the example sentence
% \[\texttt{Dog hunts cat. It is fast.}\] 
% As a quantum circuit, the whole sentence is: 

% \ctikzfig{catHuntsDogQC}
% where then the open noun wires will be composed according to the DisCoCat formalism. 
% This procedure can be applied to all the examples discussed in the upper part of this section, where the operations $O_1$ and $O_2$ in diagram \ref{diag:mappingToQC} have to be adjusted. 
% It is important to understand that for each of the possible wirings in the different examples above, there exists an equivalent quantum circuit, because there is a direct mapping from DisCoCat diagrams to quantum circuits that has been discussed in detail in section \ref{subsec:sentencesToQC}.
% % In the above diagram, the unitaries $U_{\texttt{it}^1}$ and $U_{\texttt{it}^2}$ have not yet been explained. We will do this in the following. As argued above, these two represent copying the \texttt{cat}, or the \texttt{dog}, respectively. 
% We explain, using this explicit example sentence, how the copying of the words \texttt{cat} and \texttt{dog} by the unitaries $U_{\texttt{it}^1}$ and $U_{\texttt{it}^2}$ look like as explicit quantum circuits in example \ref{expl:catDogCircuit} in the appendix. 
% We explain this using an explicit example of the training procedure, where we create an artificial dataset to showcase the function of the training process in detail. 

% In fact, one is not restricted to choosing both probabilities to \num{0.5}. And this is where this method can be explicitly verified using computer code. 
% By assigning probabilities $\alpha$ to the action of \texttt{cat} being copied and $\beta$ to the word \texttt{dog} being copied, after the sentence is finished, we end up with a probability distribution as: 
% \begin{equation}
%     \alpha \cdot \texttt{sentence one} + \beta \cdot \texttt{sentence two}
% \end{equation}
% This theory \textit{strongly} relies on the possibility to update the meaning of density matrices. 
% It is important to note that after one execution of the quantum circuit, 
% After having presented this particular example, we can generalise this idea to any sentence and any probability distribution. 
% By considering bigger datasets, the mechanisms stay the same. However, the model's predictions will not be as perfect as in the example above. 
% This will become evident in section \ref{ch:SyntaxDistribution-implementation}, where we develop a slightly bigger dataset to investigate the reasoning process developed in this chapter. 

% We briefly relate our findings to the work done by \citet{pronounResolution}. As reasoned in section \ref{sec:pronounResolution}, \citet{pronounResolution} train a model to predict if a sentence contains a subject relative, or an object relative pronoun, by explicitly training a model on this particular task. We claim that one can, with a model trained on semantics alone, recover if a relative pronoun is referring to the subject or the object in a sentence by creating a probability distribution over these two different sentences and projecting out the part that is more \texttt{True}. We will further discuss this in section \ref{ch:SyntaxDistribution-implementation}. 

% Note that, in practice, one would certainly keep this circuit more general, where the \texttt{cat} and \texttt{dog} unitaries as well as the explicit representations of the verb \texttt{hunts} and the phrase \texttt{is fast} are kept more general parametrised quantum (sub-)circuits. 
% Indeed, each of the sentences in the dataset used by \citet{pronounResolution}, shortly presented in section \ref{sec:pronounResolution}, can be modelled using this general circuit. 
% However, in order for this data to be actually implemented using the approach presented here, current quantum computers are too error prone and thus unable to process so much data. We have to note that, while indeed using our method, we can recover the internal wiring directly from syntax, we do have to teach the model the semantics in the first place. Using sentences as \citet{pronounResolution} do, this becomes very much data very fast, because the individual sentences are not related to each other semantically, only syntactically (same structure).
% In conclusion, what \citet{pronounResolution} do is probably the best approach to the particular task stated in their work. 


% If we now want to establish which of the two is the more likely, we can take the \textit{state inner product} introduced in section \ref{ch:background} with some other density matrix. 
% Consider e.g., the simple density matrix representing the pure state corresponding to \texttt{TRUE}: 
% \begin{equation*}
%     \rho_{\texttt{TRUE}} = \ket{1} \bra{1}
% \end{equation*}
% The trace inner product then yields: 
% \begin{equation*}
%     \Tr \big(  \rho_{\texttt{TRUE}} \cdot \rho_{\texttt{noun* is fast}}  \big) = 
%     \Tr \big(  0.5 \cdot \ket{1} \bra{1}  \big) = 0.5 \cdot \Tr \big(  
%     \begin{pmatrix}
%         0 & 0 \\
%         0 & 1 \\
%     \end{pmatrix}  \big) = 0.5
% \end{equation*}
% And the same for \texttt{FALSE}: 
% \begin{equation*}
%     \Tr \big(  \rho_{\texttt{FALSE}} \cdot \rho_{\texttt{noun* is fast}}  \big) = 
%     \Tr \big(  0.5 \cdot \ket{0} \bra{0}  \big) = 0.5 \cdot \Tr \big(  
%     \begin{pmatrix}
%         1 & 0 \\
%         0 & 0 \\
%     \end{pmatrix}  \big) = 0.5
% \end{equation*}
% So, the probability of this sentence being true is as likely as it being false. This makes sense, given the above discussed. 

% For this, one can furthermore use the fidelity as introduced in definition \ref{def:fidelity}: 
% \begin{equation*}
%     F(\rho_{\texttt{TRUE}}, \rho_{\texttt{noun* is fast}}) = \Tr \Big( \sqrt{ 
%     \begin{pmatrix}
%         0 & 0 \\
%         0 & 1 \\
%     \end{pmatrix}
%     \cdot 
%     \begin{pmatrix}
%         0.5 & 0 \\
%         0 & 0.5 \\
%     \end{pmatrix}
%     \cdot
%     \begin{pmatrix}
%         0 & 0 \\
%         0 & 1 \\
%     \end{pmatrix}
%     } \Big) 
% \end{equation*}
% which also returns \texttt{TRUE} and \texttt{FALSE} being equally likely. 

% What we want to do now is \textbf{update} the meaning of the density matrix. We can do this using the \texttt{FUZZ} or \texttt{PHASER} introduced in definition \ref{def:fuzz, def:phaser}, which, in this specific context, are the same: 

% \begin{equation*}
%     \rho_{\texttt{TRUE}} \, \sharp \, \rho_{\texttt{noun* is fast}} =     
%     \begin{pmatrix}
%         0 & 0 \\
%         0 & 1 \\
%     \end{pmatrix}
%     \cdot 
%     \begin{pmatrix}
%         0.5 & 0 \\
%         0 & 0.5 \\
%     \end{pmatrix}
%     \cdot
%     \begin{pmatrix}
%         0 & 0 \\
%         0 & 1 \\
%     \end{pmatrix}
%     = \begin{pmatrix}
%         0 & 0 \\
%         0 & 0.5 \\
%     \end{pmatrix}
% \end{equation*}
% As noted in definition \ref{def:fuzz}, these need to be renormalized, which amounts to dividing by the trace, which is $0.5$, so that composing the meaning \texttt{TRUE} with our resulting density matrix filters out the meaning \texttt{TRUE}, leaving us with the matrix: 
% \begin{equation*}
%     \begin{pmatrix}
%         0 & 0 \\
%         0 & 1 \\
%     \end{pmatrix}
% \end{equation*}
% where this part of the matrix arose from the word \texttt{cat} being copied. 
















%*************************
\subsection{Connection to DisCoCirc}
\label{ch:SyntaxDistribution-discocirc}
%*************************

\jurek{delete the introduction to discocirc and stess that the $\sigma$ is now a mixed state rather than a pure state}

In the proposed model, the words that are the sources of ambiguity are processes that alter the meaning of the rest of the words in the sentence. 
We give a connection to the DisCoCirc framework presented in section \ref{subsec:extensionsDisCoCat}. 
\citet{DisCoCirc} argues that a sentence is a \textit{process} that alters the meaning of the words that make it up. 
He argues that, in its most basic form, a sentence consists of nouns interacting and having properties imposed on them by verbs, adjectives, and other nouns.
\textit{Dynamic} nouns are such whose meaning evolve with the text. These nouns are modelled as density matrices whose meanings are updated using methods introduced above. 
\textit{Static} nouns are such whose meaning is static within the sentence. The corresponding density matrices are not updated with the evolution of the sentence. 

Consider the example \texttt{Man sees woman on mountain with telescope} from section \ref{ch:syntaxDistribution-multipleSources}. 
The dynamic nouns in this example are \texttt{man} and \texttt{woman}. 
This sentence can be split in three parts: 
\begin{enumerate}
    \item \texttt{Man saw woman}
    \item \texttt{on mountain}
    \item \texttt{with telescope}
\end{enumerate}
with a density matrix corresponding to each of them. 
% The process of sentences being processes acting on dynamic nouns has been explained in section \ref{subsec:extensionsDisCoCat} using the following diagram: 

% \ctikzfig{sentences}
% where $\sigma_1, \sigma_2, \ldots$ are sentences that update the meaning of the dynamic nouns. Applied to the above example, this yields: 

In DisCoCirc, the above example looks like:
\ctikzfig{manWomanDisCoCirc}
where now the meanings of the density matrices \texttt{man} and \texttt{woman} are updated by the different parts of the sentence. The initial states for \texttt{man} and \texttt{woman} can be understood as prior knowledge about these nouns. 
We can embed the theory developed above into the DisCoCirc framework in the following fashion: 

\ctikzfig{saw}
where the grey dot is either the \textit{fuzz} (definition \ref{def:fuzz}) or \textit{phaser} (definition \ref{def:phaser}). Note that one can use the \textit{Spider} as a composition method here, too. The reason is that the commutation, coming along with it, does not alter the meaning of the sentence: it does not matter in what order we update the meaning of the dynamic nouns \texttt{man} and \texttt{woman} in the example above. 
We will see next that, actually, one models the verb \texttt{saw} as a \textit{dynamic verb} as well, effectively eliminating commutativity. However, given the diagram above, one could use the spider. 

As discussed above, we want to also be able to update the meaning of the verb \texttt{saw} using either the density matrix \texttt{with telescope} or \texttt{on mountain}. 
Thus, one could interpret the verb as a \textit{dynamic verb} whose meaning is updated after interacting with the two phrases and afterwards applied to \texttt{man} and \texttt{woman}. 
We can model a dynamic verb, e.g., as: 

\ctikzfig{dynamicVerb}
where we see that the processes \texttt{with telescope} and \texttt{on mountain} will alter the meaning of the verb as well, which will only act on the nouns \texttt{man} and \texttt{woman} when the sentence is finished. 

% However, a question that arises is, how one knows if a verb is dynamic. For this, we propose all verbs be dynamic, where the dynamic nouns are composed with the dynamic nouns once all words in a sentence have been processed by the DisCoCirc framework. 

One can furthermore think about including the composition of verbs and nouns into the ambiguous phrases themselves as: 
% To answer the question of scope, one can end the scope of the dynamic verb by explicitly composing it with the dynamic nouns in the appropriate part of the sentence, so that: 
\begin{equation*}
% \hspace*{-3cm}
    \resizebox{\textwidth}{!}{\tikzfig{dynamicVerbScope}}
\end{equation*}
% \resizebox{3cm}{!}{%
% \begin{equation*}
% \tikzfig{dynamicVerbScope}
% \end{equation*}%
% }
where we see that in the rightmost of these options, the phrase \texttt{with telescope} is a verb modifier.
In this scenario, we would have to know exactly which of the phrases act on verbs as well. 

\jurek{I added this just now}


In DisCoCirc, the action of a sentence $\sigma$ on the two nouns \texttt{dog} and \texttt{vase} are captured as: 

\ctikzfig{ambiguityInDisCoCirc}

More conretely, the sentence $\sigma$ is now a probability distribution over the two different realisations of the circuit: 

\ctikzfig{dogBrokeVaseDisCoCirc}

which makes the sentence itself, as a density matrix updating the other density matrices, a mixed state. 
We see that, by introducing the theoretical framework above (in the DisCoCat framework), we are able to further the development of the DisCoCirc framework as well. 

\jurek{I would think that the connection to DisCoCirc might be better before the implementation of the theory. }








\subsection{Implementation}
\label{ch:SyntaxDistribution-implementation}

\jurek{one thing that we have to keep in mind and that we already emphasised above, is that certain processes can be generalised when using semantics rather than syntax. However, we have to keep in mind that the general training that we can do is very limited. So, in this section, we explain what such a limited training would look like, and how we can indeed recover the syntactic connection from the semantics. }

% We claim that a model that is trained on semantic relations is able to 
% As long as the semantics for every word are learned by the model, we can use the above methodology to determine which syntactic sentence structure makes semantically most sense. 
% Furthermore, we do not seek generalisation with this model. We want the model to learn the training set as well as possible, because we want a maximally good basis to reason with. 
In this section, we present a short experiment to illustrate how the proposed theory works. 
% A task could generally look like this: we teach the model some words, e.g., the word \texttt{cat} and \texttt{dog} and perhaps \texttt{duck} and associate these words to certain adjectives. 
% We then use the above constructed circuit to create a probability distribution as: 
% \begin{equation*}
%     \rho_{\texttt{sentence}} = \alpha \cdot \texttt{animal}_1 \texttt{ is adjective} + \beta \cdot \texttt{animal}_2 \texttt{ is adjective}
% \end{equation*}
% where we can then project out the \texttt{True} part of this density matrix
% Note that the object we are recovering is another density matrix. There is no way for us to get a diagram returned. However, we can choose $\alpha$ and $\beta$ to be different, which will then indicate which of the two sentences is more \texttt{True}. 
% We do not expect to receive one sentence in return. Rather we expect a probability distribution over the two sentences in return where the (semantically) more likely one has a higher probability associated to it.  
% For time reasons, we do not implement this. 
% \jurek{we may implement it, though ....}
We implement our idea using a simple dataset consisting of ten words (inspired by the dataset used by \citet{pronounResolution}, presented in section \ref{subsec:pronounResolution-implementation}): 
\begin{displayquote}
    \texttt{pancakes, pasta, women, men, tasty, delicious, hungry, starving, are, is}
\end{displayquote}
Using this vocabulary, we compose all possible meaningful combinations of words to sentences and assign the label \texttt{True}, and we compose the non-meaningful combinations of words and assign the label \texttt{False}\footnote{We want to explicitly mention here that the combinations resulting from the words \texttt{women}, \texttt{men} and \texttt{tasty} are labelled as \texttt{False}}. Example sentences in this dataset are: 
\begin{displayquote}
    \texttt{Pancakes are hungry} \qquad \texttt{False} \newline 
    \texttt{Women are starving} \qquad \, \texttt{True}
\end{displayquote}
In total, the dataset consists of \num{16} sentences, with eight sentences each labelled \texttt{False} and \texttt{True}. 
We train a \texttt{Tket} model (introduced in section \ref{ch:taskOne-binaryClassification}) on the task of matching the resulting quantum circuits to labels (where we choose $\texttt{True} = (1, 0)^T$ and $\texttt{False} = (0, 1)^T$). We use {one} qubit to encode the noun meanings on, and use the IQP-ansatz with the same parameters as used in the studies above. 
In this small study, we only use a training set, without a validation set. We saw in the chapters before that the training with the \texttt{Tket} model converges smoothly. Since this dataset is so small (\num{16} sentences in total), introducing a validation set would significantly lower the model's ability to optimise the parameters.  
The loss curve is shown in figure \ref{fig:syntaxAmbLoss}. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/tketAmbOverSyntax.png}
    \caption{The train loss and train accuracy curves for the \texttt{Tket} model, trained on the dataset introduced in the main text, noun-meaning encoded on one qubit, final accuracy on the training set: \num{1.0}, $\kappa$ = \num{1.0}, $f$1-score = \num{1.0}}
    \label{fig:syntaxAmbLoss}
\end{figure}
As we can see, the accuracy, Cohen's kappa, as well as the $f$1-score are \num{1.0}, indicating that the model makes perfect predictions. 
As a next step, in accordance with the discussion in section \ref{ch:SyntaxDistribution-mappingtoQC}, we now create a quantum circuit that creates a density matrix representing a probability distribution over two different predictions. The circuit is depicted in figure \ref{diag:implementationCircuit}. 
\begin{figure}[h]
    \centering
    \ctikzfig{appliedCircuit}
    \caption{The circuit used to create a probability distribution over the possible predictions of the model.}
    \label{diag:implementationCircuit}
\end{figure}
The sentence meaning is encoded on the uppermost qubit. Now, using this circuit, we create probability distributions over predictions of different categories and reason about this probability distribution. We do this in the following fashion. 
We create all possible combinations of \texttt{noun one} and \texttt{noun two}, where they have to belong to different categories (so \texttt{men} and \texttt{pancakes}, but not \texttt{pancakes}, \texttt{pasta}). 
We do this to obtain only probability distributions over {different} predictions of the model. 
We thus obtain one sentence that is to be predicted as \texttt{False} and one sentence that is to be predicted as \texttt{True}. We thus expect a probability distribution over the quantum states representing the label \texttt{True} and representing the label \texttt{False}. 
We then, for all of these combinations, capture the value of the {entropy} of the resulting density matrix (encoded on the upper qubit in the diagram above) and the values of the {fidelity}. The values of the fidelity are determined as comparison with the density matrices $\rho_{\texttt{True}}$ and $\rho_{\texttt{False}}$, where: 
\begin{equation}
\label{eq:trueFalseMatrix}
    \rho_{\texttt{True}} = \begin{pmatrix}
        1 & 0 \\ 0& 0
    \end{pmatrix} \qquad \rho_{\texttt{False}} = \begin{pmatrix}
        0& 0 \\ 0& 1
    \end{pmatrix} 
\end{equation}
as in chapter \ref{ch:densityMatrices}. So that, for each combination of words, we obtain one value for the entropy and two values for the fidelity. 
Note that, given the explicit matrix representations in equation \ref{eq:trueFalseMatrix}, the density matrix we observe would, in the optimal case be a probability distribution over these two {perfect} predictions, which is: 
\begin{equation*}
    \rho_{\texttt{optimal}} = \frac{1}{2}  \begin{pmatrix}
        1& 0 \\ 0& 1
    \end{pmatrix} 
\end{equation*}
The entropy for this optimal density matrix is one, and the fidelity, taken with respect to either of the pure matrices in equation \ref{eq:trueFalseMatrix}, is \num{0.5}. 
However, since the model does not make perfect predictions, as we will see further below, this result will not be achieved. 
As a last step to obtaining the resulting values for the entropy and fidelity, we {average} over the different combinations of words mentioned above and obtain the resulting average entropy and fidelity values that we discuss in the following. 

We report an average entropy of \num{0.642}. Keep in mind that the entropy we expect to see is \num{1}, because we considered only combinations of words that are of different kind, meaning that the resulting probability distribution is one over the model predicting \texttt{True} and the model predicting \texttt{False}. However, we would only be able to see this in the case of the two \textit{pure} states being perfectly separated. The density matrices overlap, as the training procedure is not optimal. 
We report an average fidelity (with the density matrix $\rho_{\texttt{True}}$) of \num{0.694}, and the fidelity with the density matrix $\rho_{\texttt{False}}$ is \num{0.306}. Note that the fidelities we would expect are \num{0.5} for both of these cases, as mentioned above.
Indeed, this suboptimal balance is due to the {pure states} representing the meanings of, e.g., \texttt{Pancakes are hungry} or \texttt{Men are hungry}, not being perfectly predicted by the model. 
Ultimately, as a prediction, we do not see a perfect probability distribution over the states $\rho_{\texttt{True}}$ and $\rho_{\texttt{False}}$. Rather, we see the probability distribution over the {predictions} of the model, which are imperfect. 

We want to quantify how imperfect these predictions are. Although we have measures like the accuracy in the training process, we now want to determine what the fidelity between the pure states representing the predictions of the model, and the density matrices $\rho_{\texttt{True}}$ and $\rho_{\texttt{False}}$ is. 
 
We record an average fidelity of \num{0.874} for the \texttt{True} sentences with the density matrix $\rho_{\texttt{True}}$, and an average fidelity of \num{0.719} for the \texttt{False} sentences with the density matrix $\rho_{\texttt{False}}$. 
It also makes sense to look at the fidelity of the predicted \texttt{False} states with the density matrix $\rho_{\texttt{True}}$, for which we find a value of \num{0.281}, and the predicted \texttt{True} states with the density matrix $\rho_{\texttt{False}}$, for which we find a value of \num{0.126}. 

\subsection{Discussion}

We see that the model's predictions, which yield \texttt{True}, have a bigger overlap with the correct density matrix than the predictions that yield \texttt{False}. 
This means that the model makes the predictions when it comes to \texttt{True} sentences more reliably. 
This, in turn, implies that what we see the model predicting as a probability distribution over two decisions, makes sense. All in all, given that the model predicts \texttt{True} labels more correctly, it makes sense that in the probability distribution over the two different predictions \texttt{True} and \texttt{False}, the model is more likely to predict the label \texttt{True} which explains the higher fidelity with the matrix $\rho_{\texttt{True}}$ and the entropy lower than 1 for the whole circuit. 
% In conclusion, 
% the minimal study conducted in this section reports our theoretically suggested model presented in this chapter. 
Our findings suggest that the probability distribution over different wirings in DisCoCat diagrams can be modelled on a quantum computer and furthermore one can reason with the density matrices that capture these probability distributions with the help of quantum circuits, as proposed in the theory in this chapter. 






==> dataset_table.tex <==
\begin{longtable}[t]{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline
woman prepares tasty dinner & woman cooks tasty sauce \\
\hline
skillful man prepares dinner & skillful woman cooks sauce \\
\hline
man prepares sauce & person cooks tasty sauce \\
\hline
man cooks sauce & woman bakes meal \\
\hline
skillful man bakes sauce & person bakes meal \\
\hline
skillful woman bakes dinner & skillful woman cooks dinner \\
\hline
man cooks meal & woman bakes sauce \\
\hline
woman prepares meal & skillful man prepares sauce \\
\hline
skillful man bakes dinner & woman cooks tasty meal \\
\hline
man prepares meal & woman prepares tasty meal \\
\hline
woman prepares sauce & woman prepares dinner \\
\hline
skillful person prepares meal & skillful person bakes dinner \\
\hline
skillful woman bakes meal & man bakes tasty meal \\
\hline
person prepares tasty meal & man bakes tasty dinner \\
\hline
skillful man cooks dinner & person cooks dinner \\
\hline
skillful woman prepares meal & skillful woman bakes sauce \\
\hline
skillful man bakes meal & woman cooks meal \\
\hline
woman bakes dinner & skillful man cooks meal \\
\hline
man cooks dinner & woman cooks tasty dinner \\
\hline
woman cooks dinner & man bakes tasty sauce \\
\hline
man prepares dinner & skillful person cooks sauce \\
\hline
person prepares tasty sauce & skillful person bakes sauce \\
\hline
skillful man cooks sauce & woman bakes tasty meal \\
\hline
person cooks meal & person bakes tasty sauce \\
\hline
person bakes dinner & man cooks tasty meal \\
\hline
skillful person cooks meal & person cooks sauce \\
\hline
man cooks tasty sauce & skillful person bakes meal \\
\hline
man prepares tasty meal & man prepares tasty sauce \\
\hline
person bakes tasty meal & person prepares dinner \\
\hline
man bakes sauce & person cooks tasty dinner \\
\hline
woman bakes tasty sauce & skillful person prepares sauce \\
\hline
person prepares tasty dinner & woman bakes tasty dinner \\
\hline
woman cooks sauce & skillful woman prepares software \\
\hline
woman runs useful program & skillful person runs software \\
\hline
skillful person prepares program & man prepares program \\
\hline
skillful person prepares software & man prepares useful software \\
\hline
woman debugs program & skillful woman runs application \\
\hline
man debugs software & skillful woman debugs application \\
\hline
person debugs software & woman runs useful software \\
\hline
person debugs program & skillful woman debugs software \\
\hline
skillful woman debugs program & person runs program \\
\hline
person runs useful application & woman runs useful application \\
\hline
woman runs application & man prepares software \\
\hline
person prepares useful program & man debugs useful application \\
\hline
person debugs useful application & woman prepares program \\
\hline
man prepares useful application & man debugs useful software \\
\hline
man prepares application & person debugs useful software \\
% \hline
% \end{tabular}
% \begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
\hline
person runs application & woman runs program \\
\hline
skillful man prepares program & woman runs software \\
\hline
skillful man debugs software & skillful man prepares software \\
\hline
person prepares software & person runs software \\
\hline
man debugs program & man runs software \\
\hline
person prepares useful application & woman debugs software \\
\hline
skillful man runs software & woman debugs application \\
\hline
woman debugs useful program & skillful woman runs program \\
\hline
person runs useful program & skillful person prepares application \\
\hline
man prepares useful program & man runs program \\
\hline
woman prepares software & person prepares useful software \\
\hline
skillful person debugs program & person debugs application \\
\hline
skillful person debugs software & skillful woman runs software \\
\hline
person debugs useful program & man runs application \\
\hline
woman debugs useful software & man runs useful application \\
\hline
person prepares program & woman debugs useful application \\
\hline
skillful woman prepares application & man debugs application \\
\hline
woman prepares useful application & man debugs useful program \\
\hline
\end{longtable}

==> figs/centrifugalpump.tex <==
\begin{tikzpicture}[scale=1]
        % define pump constants, using \def
        \def\rin{1.5}                                   % inner radius
        \def\rout{3.7}                                  % outer radius
        \def\bin{60}                                    % inner beta, degrees
        \def\bout{30}                                   % outer beta, degrees
        \def\bladepos{90}                               % blade position angle, degrees
        \def\bladecurve{60}                             % blade curve angle, degrees
        \def\uin{1.5}                                   % inner rotational velocity
        \def\cin{2.6}                                   % inner absolute velocity
        
        % calculate velocities and angles, using \pgfmathsetmacro for math operations
        \pgfmathsetmacro\uout{\uin*\rout/\rin}          % outer rotational velocity
        \pgfmathsetmacro\coutrad{\cin*\rin/\rout}       % outer absolute radial velocity
        \pgfmathsetmacro\wout{\coutrad/sin{\bout}}      % outer relative velocity
        \pgfmathsetmacro\couttan{\uout-\wout*cos(\bout)}% outer absolute tangential velocity
        \pgfmathsetmacro\tana{\coutrad/\couttan}        % outer absolute tangential velocity
        \pgfmathsetmacro\aout{atan(\tana)}              % outer alpha, degrees
        \pgfmathsetmacro\cout{\coutrad/sin(\aout)}      % outer absolute radial velocity
        
        % draw pump
        \drawcentrifugalpumpcircles{\rin}{\rout}; % draw pump circles
        
        % draw blade
        {\drawcentrifugalpumpblade{\rin}{\rout}{\bladepos}{\bladecurve}{\bin}{\bout}};
 
        % draw velocity triangle at inlet
        \draw [rotation,->] (root) -- +(0:\uin) node [right] {$u_1$};
        \draw [absolute,->] (root) -- +(90:\cin) node [right] {$c_1=c_\up{1r}$};
        \draw [relative,->] (root) -- +(-\uin,\cin) node [right] {$w_1$};
        
        % draw velocity triangle at outlet
        \draw [rotation,->] (tip) -- +(\bladecurve:\uout) coordinate (U2) node [left] {$u_2$};
        \draw [relative,->] (tip) -- +(180+\bladecurve-\bout:\wout) coordinate (W2) node [left] {$w_2$};
        \draw [absolute,->] (tip) -- +(90+\bladecurve:\coutrad) node [left] {$c_\up{2r}$};
        \coordinate (C2) at ($(U2)   +({180+\bladecurve-\bout}:{\wout})$);
        \draw [absolute,->] (tip) -- (C2) node [right] {$c_\up{2}$};
        \draw [axis] (W2) -- (C2);  % connect end of w2, c2r, c2
        
        % draw angles: location, angle1, angle2, label, arc radius, label pos, left/right
        \drawangle{root}{180}{180-\bin}{$\beta_1$}{0.4cm}{0.5}{left};                         % beta 1
        \drawangle{tip}{180+\bladecurve}{180+\bladecurve-\bout}{$\beta_2$}{1cm}{0.1}{left};   % beta 2
        \drawangle{root}{0}{90}{$\alpha_1$}{0.4cm}{0.5}{right};                               % alpha 1
        \drawangle{tip}{\bladecurve}{\bladecurve +\aout}{$\alpha_2$}{1cm}{0.4}{above}         % alpha 2
\end{tikzpicture}




==> figs/freebody.tex <==
% source: http://www.texample.net/tikz/examples/free-body-diagrams/

\def\iangle{45} % Angle of the inclined plane, was 30 in original code
\def\down{-90}
\def\arcr{0.8cm} % Radius of the arc used to indicate angles, was 0.5cm in original code

\begin{tikzpicture}[
    axis/.style={densely dashed,gray,font=\small},
    M/.style={rectangle,draw,fill=lightgray,minimum size=0.5cm,thin},
    m/.style={rectangle,draw=black,fill=lightgray,minimum size=0.3cm,thin},
    plane/.style={draw=black,fill=blue!10},
    string/.style={draw=red, thick},
    pulley/.style={thick},
]
    \matrix[column sep=1cm] {
        % Sketch
        \draw[plane] (0,-1) coordinate (base)
                         -- coordinate[pos=0.5] (mid) ++(\iangle:3) coordinate (top)
                         |- (base) -- cycle;
        \path (mid) node[M,rotate=\iangle,yshift=0.25cm] (M) {};
        \draw[pulley] (top) -- ++(\iangle:0.25) circle (0.25cm)
                       ++ (90-\iangle:0.5) coordinate (pulley);
        \draw[string] (M.east) -- ++(\iangle:1.5cm) arc (90+\iangle:0:0.25)
                      -- ++(0,-1) node[m] {};
    
        \draw[->] (base)++(\arcr,0) arc (0:\iangle:\arcr);
        \path (base)++(\iangle*0.5:\arcr+5pt) node {$\alpha$};
        %
    &
        % Free body diagram of M
        \begin{scope}[rotate=\iangle]
            \node[M,transform shape] (M) {};
            % Draw axes and help lines
            {[axis,->]
                \draw (0,-1) -- (0,2) node[right] {$+y$};
                \draw (M) -- ++(2,0) node[right] {$+x$};
                % Indicate angle. The code is a bit awkward.
                \draw[solid,shorten >=0.5pt] (\down-\iangle:\arcr)
                    arc(\down-\iangle:\down:\arcr);
                \node at (\down-0.5*\iangle:1.3*\arcr) {$\alpha$};
            }
            % Forces
            {[force,->]
                % Assuming that Mg = 1. The normal force will therefore be cos(alpha)
                \draw (M.center) -- ++(0,{cos(\iangle)}) node[above right] {$N$};
                \draw (M.west) -- ++(-1,0) node[left] {$f_\up{R}$};
                \draw (M.east) -- ++(1,0) node[above] {$T$};
            }
        \end{scope}
        % Draw gravity force. The code is put outside the rotated
        % scope for simplicity. No need to do any angle calculations. 
        \draw[force,->] (M.center) -- ++(0,-1) node[below] {$Mg$};
        %
    &
        %
        % Free body diagram of m
        \node[m] (m) {};
        \draw[axis,->] (m) -- ++(0,-2) node[left] {$+$};
        {[force,->]
            \draw (m.north) -- ++(0,1) node[above] {$T'$};
            \draw (m.south) -- ++(0,-1) node[right] {$mg$};
        }
    \\
    };
\end{tikzpicture}

==> figs/groupplot.tex <==
\begin{tikzpicture}\tinybeamer
	\begin{groupplot}[group style={group size=2 by 2,vertical sep=1em,horizontal sep=2ex,x descriptions at=edge bottom,y descriptions at=edge left},
	xmin=-2.7,xmax = 11.2,ymin=0,ymax=100,
	xlabel={$\qdot_\up{exchanged}\unitschart{kW}$},
	ylabel= {$T\unitschart{\SI{}{\celsius}}$},
	height=0.45\textheight,width=0.55\textwidth]
    	\nextgroupplot	\def\Q{1.3}; % Q in kW
    	\draw [blue,deco=0.5] (axis cs: 0,20) -- (axis cs: \Q,20+\Q/0.2/1) node [right] {\SI{26}{\celsius}};
    	\draw [red,deco=0.5](axis cs: \Q,90)  -- (axis cs: 0,90-\Q/0.03/4.18)  node [left] {\SI{80}{\celsius}};
    	\draw[helpline] (axis cs: 0,90-\Q/0.03/4.18) -- (0,0) (\Q,0) -- (\Q,90);
    	\draw[measure,<->] (axis cs: 0,10) -- (axis cs: \Q,10) node [right]{\Q~kW};
    	\node at (axis cs: 5,70) [right,align=left]{$A=\SI{0.68}{m^2}$};
    	\nextgroupplot \def\Q{2.5}; % Q in kW
    	\draw [blue,deco=0.5] (axis cs: 0,20) -- (axis cs: \Q,20+\Q/0.2/1) node [right] {\SI{33}{\celsius}};
    	\draw [red,deco=0.5](axis cs: \Q,90)  -- (axis cs: 0,90-\Q/0.03/4.18)  node [left] {\SI{70}{\celsius}};
    	\draw[helpline] (axis cs: 0,90-\Q/0.03/4.18) -- (0,0) (\Q,0) -- (\Q,90);
    	\draw[measure,<->] (axis cs: 0,10) -- (axis cs: \Q,10) node [right]{\Q~kW};
    	\node at (axis cs: 5,70) [right,align=left]{$A=\SI{1.6}{m^2}$};
    	\nextgroupplot \def\Q{3.8}; % Q in kW
    	\draw [blue,deco=0.5] (axis cs: 0,20) -- (axis cs: \Q,20+\Q/0.2/1) node [right] {\SI{39}{\celsius}};
    	\draw [red,deco=0.5](axis cs: \Q,90)  -- (axis cs: 0,90-\Q/0.03/4.18)  node [left] {\SI{60}{\celsius}};
    	\draw[helpline] (axis cs: 0,90-\Q/0.03/4.18) -- (0,0) (\Q,0) -- (\Q,90);
    	\draw[measure,<->] (axis cs: 0,10) -- node [above]{\Q~kW} (axis cs: \Q,10);
    	\node at (axis cs: 5,70) [right,align=left]{$A=\SI{2.8}{m^2}$};
    	\nextgroupplot \def\Q{8.8}; % Q in kW
    	\draw [blue,deco=0.5] (axis cs: 0,20) -- (axis cs: \Q,20+\Q/0.2/1)  node [right] {\SI{64}{\celsius}};
    	\draw [red,deco=0.5](axis cs: \Q,90) -- (axis cs: 0,90-\Q/0.03/4.18) node [left] {\SI{20}{\celsius}};
    	\draw[helpline] (axis cs: 0,90-\Q/0.03/4.18) -- (0,0) (\Q,0) -- (\Q,90);  
    	\draw[measure,<->] (axis cs: 0,10) -- node [above]{\Q~kW $=\qdot_\up{max}$} (axis cs: \Q,10); 
    	\node at (axis cs: -2,70) [right,align=left]{$A=\infty~\up{m^2}$};
	\end{groupplot}
\end{tikzpicture}
